ATLAS Run 1 searches for direct pair production of third-generation squarks at the Large Hadron Collider

This paper reviews and extends searches for the direct pair production of the scalar supersymmetric partners of the top and bottom quarks in proton-proton collisions collected by the ATLAS collaboration during the LHC Run 1. Most of the analyses use 20 fb$^{-1}$ of collisions at a centre-of-mass energy of $\sqrt{s}$ = 8 TeV, although in some case an additional 4.7 fb$^{-1}$ of collision data at $\sqrt{s}$ = 7 TeV are used. New analyses are introduced to improve the sensitivity to specific regions of the model parameter space. Since no evidence of third-generation squarks is found, exclusion limits are derived by combining several analyses and are presented in both a simplified model framework, assuming simple decay chains, as well as within the context of more elaborate phenomenological supersymmetric models.

==> SRtable.tex <==

\begin{table}[hp]
\begin{center}
\caption{Event yields, SM predictions, expected and observed visible cross section limits for all signal regions considered.  \label{tab:SRyields}}
\vspace{0.5cm}
\begin{tabular}{cc|c|c|c|c} \hline\hline
\multicolumn{2}{c|}{\multirow{2}{*}{Region}} & \multirow{2}{*}{$N_{\mathrm{obs}}$} & \multirow{2}{*}{$N_{\mathrm{exp}}$} & \multicolumn{2}{c}{$\sigma_{\mathrm{vis}}$ [fb]} \\
&  & & & Obs. & Exp. \\
 \hline
 \hline
 \multicolumn{2}{c|}{\stopZeroLep-SRA1} & 11 & $15.8\pm 1.9$ & 0.33 & 0.48\\
 \multicolumn{2}{c|}{\stopZeroLep-SRA2} & 4 & $4.1\pm 0.8$ & 0.29 & 0.29\\
 \multicolumn{2}{c|}{\stopZeroLep-SRA3} & 5 & $4.1\pm 0.9$ & 0.33 & 0.29\\
 \multicolumn{2}{c|}{\stopZeroLep-SRA4} & 4 & $2.4\pm 0.7$ & 0.32 & 0.25\\
 \multicolumn{2}{c|}{\stopZeroLep-SRB} & 2 & $2.4\pm 0.7$ & 0.21 & 0.24\\
 \multicolumn{2}{c|}{\stopZeroLep-SRC1} & 59 & $68\pm 7$ & 0.78 & 1.03\\
 \multicolumn{2}{c|}{\stopZeroLep-SRC2} & 30 & $34\pm 5$ & 0.62 & 0.73\\
 \multicolumn{2}{c|}{\stopZeroLep-SRC3} & 15 & $20.3\pm 3.0$ & 0.40 & 0.55\\
 \hline
 \hline
 \multicolumn{2}{c|}{\stopOneLep-tN\_med} & 12 & $13.0 \pm 2.2$ & 0.4 & 0.5\\
 \multicolumn{2}{c|}{\stopOneLep-tN\_high} & 5 & $5.0 \pm 1.0$ & 0.3 & 0.3\\
 \multicolumn{2}{c|}{\stopOneLep-tN\_boost} & 5 & $3.3 \pm 0.7$ & 0.3 & 0.3\\	
 \multicolumn{2}{c|}{\stopOneLep-bCa\_low} & 11 & $6.5 \pm 1.4$ & 0.61 & 0.92\\	
 \multicolumn{2}{c|}{\stopOneLep-bCa\_med} & 20 & $17 \pm 4$ & 0.72 & 0.68\\	
 \multicolumn{2}{c|}{\stopOneLep-bCb\_med1} & 41 & $32 \pm 5$ & 1.17 & 0.88\\	
 \multicolumn{2}{c|}{\stopOneLep-bCb\_high} & 7 & $9.8 \pm 1.6$ & 0.32 & 0.22\\	
 \multicolumn{2}{c|}{\stopOneLep-bCc\_diag} & 493 & $470 \pm 50$ & 5.4 & 4.7\\	
 \multicolumn{2}{c|}{\stopOneLep-bCd\_high1} & 16 & $11.0 \pm 1.5$ & 0.7 & 0.4\\	
 \multicolumn{2}{c|}{\stopOneLep-bCd\_high2} & 5 & $4.4 \pm 0.8$ & $0.3$ & $0.3$ \\
 \multicolumn{2}{c|}{\stopOneLep-tNbC\_mix}& 10 & $7.2 \pm 1.0$ & $0.5$ & $0.3$ \\
 \hline
 \multicolumn{2}{l|}{\stopOneLep-tN\_diag} & & & &  \\
$125 < \met  < 150$\ \GeV, & $120 < \mt < 140$\, \GeV  & 117 & $136 \pm 22$& $2.1$ & $2.7$ \\
$125 < \met  < 150$\ \GeV, & $\mt > 140$\ \GeV  & 163 & $152 \pm 20$ & $2.7$ & $2.4$ \\
$\met > 150$\ \GeV, & $120 < \mt < 140$\ \GeV  & 101 & $98 \pm 13$& $1.8$ & $1.7$ \\
$\met > 150$\ \GeV, & $\mt > 140$\ \GeV  & 217 & $236 \pm 29$& $2.9$ & $3.5$ \\
\hline
\multicolumn{2}{l|}{\stopOneLep-bCb\_med2} & & & & \\
$175 < \amtTwo < 250$\ \GeV, & $90 < \mt < 120$\ \GeV & 10 & $12.1 \pm 2.0$& $0.4$ & $0.4$ \\
$175 < \amtTwo < 250$\ \GeV, & $\mt > 120$\ \GeV  & 10 & $7.4 \pm 1.4$& $0.5$ & $0.4$ \\
$\amtTwo > 250$\ \GeV, & $90 < \mt < 120$\ \GeV  & 16 & $21 \pm 4$& $0.5$ & $0.6$ \\
$\amtTwo > 250$\ \GeV, & $\mt > 120$\ \GeV  & 9 & $9.1 \pm 1.6$& $0.4$ & $0.4$ \\
\hline
\multicolumn{2}{l|}{\stopOneLep-bCd\_bulk} & & & & \\
$175 < \amtTwo < 250$\ \GeV, & $90 < \mt < 120$\,\GeV & 144 & $133 \pm 22$& $1.8$ & $1.7$ \\
$175 < \amtTwo < 250$\ \GeV, & $\mt > 120$\,\GeV   & 78 & $73 \pm 8$& $2.9$ & $3.5$ \\
$\amtTwo > 250$\,\GeV, & $90 < \mt < 120$\,\GeV   & 61 & $66 \pm 6$& $0.9$ & $1.0$ \\
$\amtTwo > 250$\,\GeV, & $\mt > 120$\,\GeV  & 29 & $26.5 \pm 2.6$& $0.7$ & $0.6$ \\
\hline
\multicolumn{2}{l|}{\stopOneLep-3body} & & & & \\
$80 < \amtTwo < 90$\ \GeV, &  $90 < \mt < 120$\,\GeV & 12 & $16.9 \pm 2.8$ & $0.4$ & $0.5$ \\
$80 < \amtTwo < 90$\ \GeV, & $\mt > 120$\,\GeV    & 8 & $8.4 \pm 2.2$ & $0.4$ & $0.4$ \\
$90 < \amtTwo < 100$\ \GeV, & $90 < \mt < 120$\,\GeV   & 29 & $35 \pm 4$ & $0.6$ & $0.7$ \\
$90 < \amtTwo < 100$\ \GeV, & $\mt > 120$\ \GeV  & 22 & $29 \pm 5$ & $2.7$ & $2.4$ \\
\hline
\hline
\end{tabular}
\end{center}
\end{table}
\begin{table}
\begin{center}
\begin{tabular}{cc|c|c|c|c}
\hline
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{Region}} & \multirow{2}{*}{$N_{\mathrm{obs}}$} & \multirow{2}{*}{$N_{\mathrm{exp}}$} & \multicolumn{2}{c}{$\sigma_{\mathrm{vis}}$ [fb]} \\
&  & & & Obs. & Exp. \\
\hline
\multicolumn{2}{c|}{\stopTwoLep-L90} & 274 & $300 \pm 50$ & 3.6 & 4.2 \\
\multicolumn{2}{c|}{\stopTwoLep-L100} & 3 & $5.2 \pm 2.2$ & 0.28 & 0.32 \\
\multicolumn{2}{c|}{\stopTwoLep-L110} & 8 & $9.3 \pm 3.5$ & 0.44 & 0.46 \\
\multicolumn{2}{c|}{\stopTwoLep-L120} & 18 & $19 \pm 9$ & 0.86 & 0.89 \\
\hline
\multicolumn{2}{c|}{\stopCharm-M1} & 33054 & $33450 \pm 960$ & 96.2 &  96.6\\
\multicolumn{2}{c|}{\stopCharm-M2} & 8606 & $8620 \pm 270$ & 28.4 & 29.1\\
\multicolumn{2}{c|}{\stopCharm-M3} & 1776 & $1770 \pm 81$ & 9.6 & 9.4\\
\multicolumn{2}{c|}{\stopCharm-C1} & 208& $208 \pm 21$ & 1.76 & 1.81\\
\multicolumn{2}{c|}{\stopCharm-C2} & 71 & $75 \pm 11$ & 0.95 & 1.08\\
\hline
\multicolumn{2}{c|}{\stopTwo-SR2A} & 10 & $10.8 \pm 1.7$ & 0.40 & 0.46\\
\multicolumn{2}{c|}{\stopTwo-SR2B} & 1 & $2.4 \pm 0.9$ & 0.19 & 0.24\\
\multicolumn{2}{c|}{\stopTwo-SR2C} & 2 & $3.5 \pm 0.5$ & 0.20 & 0.27\\
\multicolumn{2}{c|}{\stopTwo-SR3A} & 4 & $4.5 \pm 1.4$ & 0.30 & 0.31\\
\multicolumn{2}{c|}{\stopTwo-SR3B} & 2 & $1.3 \pm 0.4$ & 0.20 & 0.26\\
\hline
\multicolumn{2}{c|}{\WWlike-SR1} & 40 & $48 \pm 14$ & 1.12 & 1.25\\
\multicolumn{2}{c|}{\WWlike-SR2} & 71 & $81 \pm 13$ & 1.24 & 1.45\\
\multicolumn{2}{c|}{\WWlike-SR3} & 215 & $203 \pm 27$ & 2.38 & 2.29\\
\multicolumn{2}{c|}{\WWlike-SR4} & 88 & $81 \pm 12$ & 1.73 & 1.34\\
\multicolumn{2}{c|}{\WWlike-SR5} & 4 & $3.39 \pm 0.91$ & 0.30 & 0.28\\
\multicolumn{2}{c|}{\WWlike-SR6} & 160 & $154 \pm 19$ & 2.25 & 2.16\\
\multicolumn{2}{c|}{\WWlike-SR7} & 21 & $23.1 \pm 4.4$ & 0.61 & 0.68\\
\hline
\end{tabular}
\end{center}
\end{table}


==> bChi_diagrams.tex <==
% !TEX root = ../stopsbottom_summary.tex

\begin{figure}
\setlength{\unitlength}{0.20mm}
\subfloat[\label{fig:bCdecay_DM520}]{
\begin{picture}(200,250)
\color{red}
\linethickness{0.7mm}
\put(50,30){\line(1,0){100}}
\put(50,70){\line(1,0){100}}
\put(50,220){\line(1,0){100}}
\color{black}
\linethickness{0.2mm}
\put(100,220){\vector(0,-1){150}}
\put(100,70){\vector(0,1){150}}
\put(100,70){\vector(0,-1){40}}
\put(100,30){\vector(0,1){40}}
%\put(40,120){$\alpha$}
%\put(15,230){$\dmCN = 5, 20\ \mathrm{GeV}$}
\put(170,215){$\tone$}
\put(170,65){$\chipm$}
\put(170,25){$\neut$}
\end{picture}
}
\subfloat[\label{fig:bCdecay_fixedC}]{
\begin{picture}(200,250)
\color{red}
\linethickness{0.7mm}
\put(50,30){\line(1,0){100}}
\linethickness{1.2mm}
\put(50,100){\line(1,0){100}}
\linethickness{0.7mm}
\put(50,220){\line(1,0){100}}
\color{black}
\linethickness{0.2mm}
\put(100,220){\vector(0,-1){120}}
\put(100,100){\vector(0,1){120}}
\put(100,100){\vector(0,-1){70}}
\put(100,30){\vector(0,1){70}}
%\put(40,120){$\alpha$}
%\put(15,230){Fixed chargino mass}
\put(170,215){$\tone$}
\put(170,95){$\chipm$}
\put(170,25){$\neut$}
\end{picture}
}
\subfloat[\label{fig:bCdecay_gaugeUni}]{
\begin{picture}(200,250)
\color{red}
\linethickness{0.7mm}
\put(50,30){\line(1,0){100}}
\put(50,135){\line(1,0){100}}
\put(50,220){\line(1,0){100}}
\color{black}
\linethickness{0.2mm}
\put(100,220){\vector(0,-1){85}}
\put(100,135){\vector(0,1){85}}
\put(100,135){\vector(0,-1){105}}
\put(100,30){\vector(0,1){105}}
%\put(40,120){$\alpha$}
%\put(55,230){$m_{\chipm} = 2 m_{\neut}$}
\put(170,215){$\tone$}
\put(170,125){$\chipm$}
\put(170,25){$\neut$}
\end{picture}
}
\subfloat[\label{fig:bCdecay_tCcompressed}]{
\begin{picture}(200,250)
\color{red}
\linethickness{0.7mm}
\put(50,30){\line(1,0){100}}
\put(50,195){\line(1,0){100}}
\put(50,220){\line(1,0){100}}
\color{black}
\linethickness{0.2mm}
\put(100,220){\vector(0,-1){25}}
\put(100,195){\vector(0,1){25}}
\put(100,195){\vector(0,-1){165}}
\put(100,30){\vector(0,1){165}}
%\put(40,120){$\alpha$}
%\put(15,230){$\Delta m \left(\tone, \chipm \right) = 10\ \mathrm{GeV}$}
\put(170,215){$\tone$}
\put(170,190){$\chipm$}
\put(170,25){$\neut$}
\end{picture}
}


\caption{Scenarios considered for the $\tone \rightarrow b \chipm$ decay: (a) $\dmCN = 5, 20\ \mathrm{GeV}$; (b) Fixed chargino mass; (c) $m_{\chipm} = 2 m_{\neut}$; (d) $\Delta m \left(\tone, \chipm \right) = 10\ \mathrm{GeV}$. A thicker red line indicates that the particle mass is kept fixed in the corresponding model}
\label{fig:TC1}
\end{figure}


==> other_decays.tex <==

Besides the decays of the stop discussed earlier in this section, other possible scenarios have been considered. One of these scenarios is inspired by natural gauge-mediated SUSY breaking~\cite{Dine:1981gu,AlvarezGaume:1981wy,Nappi:1982hm,Dine:1993yw, Dine:1994vc,Dine:1995ag} (GMSB) models. In GMSB models, the lightest neutralino is typically the NLSP, and the supersymmetric partner of the graviton (the gravitino $\tilde{G}$) is the LSP, with mass of the order of a \keV. The scenario considered, which assumes direct $\tone$ pair production and decays mostly through $\tone \rightarrow t \neut \rightarrow t Z \tilde{G}$, gives final states similar to those in the \stopTwo\ scenario and  is described in detail in Ref.~\cite{Aad:2014mha}. The derived 95\% CL limits are obtained in the plane defined by the stop and neutralino (assumed to be the NLSP) mass: they exclude the existence of stops with masses  up to  540 GeV for a neutralino mass of 100 GeV.





==> pippo <==
01lep_combine.tex:The statistical combination of the two analyses is performed by running the combined fit simultaneously on the control and signal regions of the two analyses. The detector systematic uncertainties are treated as correlated by using, for each of the uncertainties considered, a single nuisance parameter. The supersymmetric signal parameter strength used is the same for the two analyses, while the normalisation parameters for the background processes are kept independent in each analysis.\footnote{The choice is motivated by the fact that the phase-space regions in which the two analyses determine the normalisation parameters of the \ttbar, \Zjets\ and \Wjets\ (for \stopZeroLep) and \ttbar\ and \Wjets\ (for \stopOneLep) are characterised by different kinematic selections and jet multiplicities.} The nuisance parameters associated with modelling uncertainties of the various processes are also kept independent.
01lep_combine.tex:For each combination performed, the fit setup is validated by checking that the background normalisation parameters obtained are compatible with those obtained separately by the two analyses, by verifying that no additional constraint on the nuisance parameters is introduced with respect to the individual fits, and by checking that no artificial correlation is introduced between any of the fit parameters.
01lep_combine_summary.tex:To maximise the sensitivity to the $\tone \rightarrow t \neut$ decays a statistical combination of the  \stopZeroLep\ and \stopOneLep\ signal regions is performed. The details of the combination are given in Appendix~\ref{sec:01lepCombine} and the final limit is shown in Figure~\ref{fig:tNsummary} by the largest shaded region (yellow). The expected limit on the stop mass is about 50 GeV higher at low $m_{\neut}$ than in the individual analyses. The observed limit is increased by roughly the same amount and stop masses between 200~GeV and 700~GeV are excluded for small neutralino masses.\footnote{This result holds if the top quark produced in the $\tone$ decay has a right-handed chirality. The dependence of the individual limits on the top quark chirality is discussed in Refs.~\cite{Aad:2014bva} and \cite{Aad:2014kra}.}
01lep_combine_summary.tex:A similar combination is performed to target a scenario where the stop can decay as $\tone \rightarrow t \neut$ with branching ratio $x$ and as $\tone \rightarrow b \chipm$ with branching ratio $1-x$. Assuming gauge universality, the mass of the chargino is set to be twice that of the neutralino. Neutralino masses below 50 GeV are not considered, to take into account limits on the lightest chargino mass obtained at LEP~\cite{lep2, Heister:2003zk, Abdallah:2003xe, Acciarri:1999km, Abbiendi:2003sc}.  The exclusion limits are derived for $x= 75\%, 50\%, 25\%$ and 0\%.\footnote{A value of $x = 0\%$ is in fact not achievable in a  real supersymmetric model. Nevertheless, this value has been considered as the limiting case of a simplified model.} Regardless of the branching ratio considered, it is always assumed that $m_{\tone} > \mtop + m_{\neut}$ and $m_{\tone} > m_b + m_{\chipm}$, such that the two decays $\stop \rightarrow t \neut$ and $\stop \rightarrow b \chipm$ are both kinematically allowed. A statistical combination, identical to the one described above, is used for $x = 75\%$. For smaller values of $x$, no combined fit is performed, as the sensitivity is dominated by the \stopOneLep\ analysis almost everywhere: rather either the \stopZeroLep\ or the \stopOneLep\ analysis is used, depending which one gives the smaller expected \cls\ value. 
0lepton.tex:Finally, a third set of signal regions, named \stopZeroLep-SRC, is designed to increase the analysis sensitivity to the decay $\tone \rightarrow b \chipm$. The presence of the intermediate chargino state tends to decrease the jet multiplicity: these signal regions require five \antikt\ jets with $R=0.4$, and base the signal selection on a set of transverse mass variables aimed at  rejecting the dominant SM \ttbar\ production process.
1lepton.tex:The large number of signal regions defined in this analysis stems from the variety and complexity of the possible stop final states considered~\cite{Aad:2014kra}. All signal regions are characterised by the presence of one lepton, a second-lepton veto, a minimum of two jets and large \etmiss. A first set of four signal regions (t1L-tN) were optimised assuming a branching ratio of 100\% for the decay $\stop \rightarrow t \neut$. These signal regions aim at having sensitivity to different $\Delta m(\stop, \neut)$, in particular \stopOneLep-tN\_diag targets scenarios with small $\dmTN$ and makes use of the shape information of the \etmiss and \mt distributions.\footnote{The transverse mass $\mt$ of the lepton  with transverse momentum $\vec{p}_{\mathrm{T}}$ and the missing transverse momentum vector \ptmiss with magnitude \etmiss is defined as 
1lepton.tex:\mt = \sqrt{2\left(|\vec{p}_{\mathrm{T}}| \etmiss - \vec{p}_{\mathrm{T}} \cdot \ptmiss\right)}
1lepton.tex:The last two signal regions listed in Table~\ref{tab:SRname},  \stopOneLep-3body and \stopOneLep-tNbC\_mix, were optimised for two additional possible scenarios. If $\Delta m(\stop, \neut) < \mtop$ and the mass hierarchy or the model parameters suppress the decay through a chargino, then the dominant stop decay is $\stop \rightarrow bW\neut$, through an off-shell top quark (three-body decay). The dedicated signal region relies on the shape information from the \mt\ and \amtTwo\ variable distributions. Finally,  \stopOneLep-tNbC\_mix is designed to recover sensitivity in scenarios where the stop is assumed to decay with similar probabilities to $t\neut$ and $b\chipm$: the selection aims to reject the dominant dileptonic \ttbar\ background by making use of the topness~\cite{Graesser:2012qy} variable.
Acknowledgements.tex:We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC,
Acknowledgements.tex:Foundation, Germany; GSRT and NSRF, Greece; RGC, Hong Kong SAR, China; ISF, MINERVA, GIF, I-CORE and Benoziyo Center, Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; FOM and NWO, Netherlands; BRF and RCN, Norway; MNiSW and NCN, Poland; GRICES and FCT, Portugal; MNE/IFA, Romania; MES of Russia and NRC KI, Russian Federation; JINR; MSTD,
Acknowledgements.tex:KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain),
SRtable.tex:\multicolumn{2}{c|}{\multirow{2}{*}{Region}} & \multirow{2}{*}{$N_{\mathrm{obs}}$} & \multirow{2}{*}{$N_{\mathrm{exp}}$} & \multicolumn{2}{c}{$\sigma_{\mathrm{vis}}$ [fb]} \\
SRtable.tex:\multicolumn{2}{c|}{\multirow{2}{*}{Region}} & \multirow{2}{*}{$N_{\mathrm{obs}}$} & \multirow{2}{*}{$N_{\mathrm{exp}}$} & \multicolumn{2}{c}{$\sigma_{\mathrm{vis}}$ [fb]} \\
SRtable.tex:\multicolumn{2}{c|}{\stopCharm-M1} & 33054 & $33450 \pm 960$ & 96.2 &  96.6\\
SRtable.tex:\multicolumn{2}{c|}{\stopCharm-M2} & 8606 & $8620 \pm 270$ & 28.4 & 29.1\\
SRtable.tex:\multicolumn{2}{c|}{\stopCharm-M3} & 1776 & $1770 \pm 81$ & 9.6 & 9.4\\
SRtable.tex:\multicolumn{2}{c|}{\stopCharm-C1} & 208& $208 \pm 21$ & 1.76 & 1.81\\
SRtable.tex:\multicolumn{2}{c|}{\stopCharm-C2} & 71 & $75 \pm 11$ & 0.95 & 1.08\\
WWlike.tex:MC simulated events are used to model the signal and to describe all backgrounds that produce two prompt leptons from $W$, $Z$ or $h$ decay. For processes whose predicted yield in the signal regions is small, or whose topology resembles very closely that of the signal, making it hard to define a proper control region, the background estimate is fully based on MC simulation. For \ttbar, \Zjets\ and $WW$ production processes, which are the dominant backgrounds, the acceptance of the signal regions selection is estimated with MC simulation, while the normalisation is estimated in dedicated control regions. The MC samples used are the same as in Ref.~\cite{Aad:2014qaa}.
WWlike.tex:{\color{red}{Finally, the variable $\cos \theta_\mathrm{b}$, the cosine of the angle between the direction of motion of the one of the two leptons and the beam axis in the centre-of-mass frame of the two visible leptons~\cite{Melia:2011cu}, is sensitive to the spin of the produced particles, hence it provides additional rejection power against the $WW$ production process.}}
WWlike.tex:$|\cos\theta_\mathrm{b}|$ & $<0.8$ & $<0.8$ & $<0.8$ & - & - & $<0.8$ & - \\
WWlike.tex:  Specific control regions, whose event yield is expected to be dominated by each of these production processes, are defined and included in the fit to constrain the normalisation parameters. The control region CRT for \ttbar production is defined by changing the following selections with respect to the signal regions: $\mtTwoll > 35$ GeV, $R_1 < 0.3$. Its purity is 92\%. The CR for $WW$ production (CRW) is defined by $\mtTwoll > 35$ GeV, $\Delta X > 0.04$, and has a purity of 72\%. Finally, the CR for \Zjets\  (CRZ) is defined by $\mtTwoll < 20$ GeV, $30\ \mathrm{GeV} < m_{\ell \ell} < 80$ GeV, with a purity of 86\%. The normalisation factors of the $WW$, \ttbar, \Zjets\ production processes ($\mu_{WW}, \mu_{\ttbar}$ and $\mu_Z$ respectively) are determined by a combined profile likelihood fit. When testing the signal-plus-background hypothesis for rejection, the fit takes automatically into account the signal contamination in the control regions. For signal scenarios considering light ($m_{\tone} < 150$ GeV) stops decaying through $\tone \rightarrow bW^{(*)}\neut$, the signal contamination becomes so large that $\mu_{WW}$ becomes unrealistically low. For such cases the fit is performed excluding CRW and taking the normalisation of the $WW$ background from MC simulation.
WWlike.tex: Systematic uncertainties, affecting both the modelling of the detector response (detector-related systematic uncertainties) and the theoretical prediction of the cross sections and acceptances of the background processes (theory-related systematic uncertainties) affect the predicted rates in the signal regions. Their classification and estimation follows closely those defined in Ref.~\cite{Aad:2014qaa}. A few differences, discussed in the following, exist on the estimation of the theory-related uncertainties. The total uncertainty on the yield of the $WW$ production process is composed of three terms: the  uncertainty on the NLO hard-scattering calculation is taken to be the difference between the prediction of \powheg and aMC@NLO both using \pythia for the parton shower; the uncertainty addressing the  choice of the parton-shower model is estimated as the difference of the aMC@NLO predictions showered either with \herwig or \pythia; the uncertainty due to the choice of the renormalisation and factorisation scale is evaluated by changing the scales independently by a factor of two or one-half and taking the maximum difference. The estimated relative uncertainties on the signal region yields are about 6\% in SR1--SR4 and SR6; 11\% in SR7 and 29\% in SR5. Similar comparisons performed on the $WZ$  and $ZZ$ process yield uncertainties ranging from 30\% to 45\% depending on the signal region considered. Additional systematic uncertainties are assigned to the small expected yields from \Zjets\ production (80\%), $Wt$ (50\% to 100\% depending on the SR considered), and non-prompt lepton background.
WWlike.tex:The values of the normalisation factors obtained when performing the fit to the control regions only are shown in Table~\ref{tab:WWNorm}. 
WWlike.tex:\caption{ Normalisation factors for the $\ttbar$, $WW$ and \Zjets\ background processes obtained by the combined fit to the control region yields. The uncertainties include systematic and statistical uncertainties.\label{tab:WWNorm}} 
WWlike.tex:Normalisation factor  & Value \\
WWlike.tex:$|\cos\theta_\mathrm{b}|<0.8$ & $|\cos\theta_b|<0.8$ & $|\cos\theta_b|<0.8$  \\
WWlike.tex:  \caption{Observed (Obs) and predicted (Exp) numbers of events in the signal regions of the \WWlike\ analysis, together with the 95\% CL upper limits on the observed and expected number of signal events ($S_{\rm obs}^{95}$ and $S_{\rm exp}^{95}$, respectively), and on the visible cross section ($\langle\epsilon{\rm \sigma}\rangle_{\rm obs}^{95}$).
WWlike.tex:{\bf Signal channel}                        & Obs & Exp &  $S_{\rm obs}^{95}$  & $S_{\rm exp}^{95}$ &  $\langle\epsilon{\rm \sigma}\rangle_{\rm obs}^{95}$[fb]  \\
WWlike.tex:Table~\ref{tab:WWresults} compares the predicted and observed numbers of events in each of the signal regions. No excess above the SM prediction is observed, hence the results are first used to derive model-independent 95\% CL exclusion limits on the minimum number of events beyond the Standard Model in the signal region assuming no signal contamination in the control regions, and then to extract limits on $\sigma_{\mathrm{vis}} = \sigma \times \epsilon \times \mathcal{A}$, where $\sigma$ is the cross section for non-SM processes, $\epsilon$ is the selection efficiency and $\mathcal{A}$ is the selection acceptance. These limits are also reported in Table~\ref{tab:WWresults}. Finally, 95\% CL exclusion limits are derived in specific supersymmetric models of direct pair production of stops. The first exclusion limit (Figure~\ref{fig:WW_stop_10}) is derived in a model where the stop is assumed to decay as $\tone \rightarrow b \chipm$ with a branching ratio of 100\%, followed by the decay of the chargino into the neutralino, assumed to be the stable LSP, through $\chipm \rightarrow W^{(*)} \neut$. The chargino mass is assumed to satisfy the relation $m_{\chipm} = m_{\tone} - 10\ \GeV$, and the limit is derived in the $m_{\tone}$--$m_{\neut}$ plane. Stop masses up to about 250 GeV are excluded, almost independently of the neutralino mass. The second limit is derived in a model where the $\tone$ decays through its three-body or four-body decay (depending on its mass and on that of the neutralino) into $\tone \rightarrow b \ell\nu \neut$ with a branching ratio of 100\%, under the assumption that the decay happens through an off-shell top quark and an on- or off-shell $W$ boson. The limit is shown in Figure~\ref{fig:WW_threebody} and fills a gap between the exclusions of the \stopTwoLep\ and \stopOneLep\ analyses. 
atlas_authlist.tex:G.~Aad$^{\rm 85}$,
atlas_authlist.tex:B.~Abbott$^{\rm 113}$,
atlas_authlist.tex:J.~Abdallah$^{\rm 151}$,
atlas_authlist.tex:O.~Abdinov$^{\rm 11}$,
atlas_authlist.tex:R.~Aben$^{\rm 107}$,
atlas_authlist.tex:M.~Abolins$^{\rm 90}$,
atlas_authlist.tex:O.S.~AbouZeid$^{\rm 158}$,
atlas_authlist.tex:H.~Abramowicz$^{\rm 153}$,
atlas_authlist.tex:H.~Abreu$^{\rm 152}$,
atlas_authlist.tex:R.~Abreu$^{\rm 116}$,
atlas_authlist.tex:Y.~Abulaiti$^{\rm 146a,146b}$,
atlas_authlist.tex:B.S.~Acharya$^{\rm 164a,164b}$$^{,a}$,
atlas_authlist.tex:L.~Adamczyk$^{\rm 38a}$,
atlas_authlist.tex:D.L.~Adams$^{\rm 25}$,
atlas_authlist.tex:J.~Adelman$^{\rm 108}$,
atlas_authlist.tex:S.~Adomeit$^{\rm 100}$,
atlas_authlist.tex:T.~Adye$^{\rm 131}$,
atlas_authlist.tex:A.A.~Affolder$^{\rm 74}$,
atlas_authlist.tex:T.~Agatonovic-Jovin$^{\rm 13}$,
atlas_authlist.tex:J.~Agricola$^{\rm 54}$,
atlas_authlist.tex:J.A.~Aguilar-Saavedra$^{\rm 126a,126f}$,
atlas_authlist.tex:S.P.~Ahlen$^{\rm 22}$,
atlas_authlist.tex:F.~Ahmadov$^{\rm 65}$$^{,b}$,
atlas_authlist.tex:G.~Aielli$^{\rm 133a,133b}$,
atlas_authlist.tex:H.~Akerstedt$^{\rm 146a,146b}$,
atlas_authlist.tex:T.P.A.~{\AA}kesson$^{\rm 81}$,
atlas_authlist.tex:A.V.~Akimov$^{\rm 96}$,
atlas_authlist.tex:G.L.~Alberghi$^{\rm 20a,20b}$,
atlas_authlist.tex:J.~Albert$^{\rm 169}$,
atlas_authlist.tex:S.~Albrand$^{\rm 55}$,
atlas_authlist.tex:M.J.~Alconada~Verzini$^{\rm 71}$,
atlas_authlist.tex:M.~Aleksa$^{\rm 30}$,
atlas_authlist.tex:I.N.~Aleksandrov$^{\rm 65}$,
atlas_authlist.tex:C.~Alexa$^{\rm 26a}$,
atlas_authlist.tex:G.~Alexander$^{\rm 153}$,
atlas_authlist.tex:T.~Alexopoulos$^{\rm 10}$,
atlas_authlist.tex:M.~Alhroob$^{\rm 113}$,
atlas_authlist.tex:G.~Alimonti$^{\rm 91a}$,
atlas_authlist.tex:L.~Alio$^{\rm 85}$,
atlas_authlist.tex:J.~Alison$^{\rm 31}$,
atlas_authlist.tex:S.P.~Alkire$^{\rm 35}$,
atlas_authlist.tex:B.M.M.~Allbrooke$^{\rm 149}$,
atlas_authlist.tex:P.P.~Allport$^{\rm 74}$,
atlas_authlist.tex:A.~Aloisio$^{\rm 104a,104b}$,
atlas_authlist.tex:A.~Alonso$^{\rm 36}$,
atlas_authlist.tex:F.~Alonso$^{\rm 71}$,
atlas_authlist.tex:C.~Alpigiani$^{\rm 76}$,
atlas_authlist.tex:A.~Altheimer$^{\rm 35}$,
atlas_authlist.tex:B.~Alvarez~Gonzalez$^{\rm 30}$,
atlas_authlist.tex:D.~\'{A}lvarez~Piqueras$^{\rm 167}$,
atlas_authlist.tex:M.G.~Alviggi$^{\rm 104a,104b}$,
atlas_authlist.tex:B.T.~Amadio$^{\rm 15}$,
atlas_authlist.tex:K.~Amako$^{\rm 66}$,
atlas_authlist.tex:Y.~Amaral~Coutinho$^{\rm 24a}$,
atlas_authlist.tex:C.~Amelung$^{\rm 23}$,
atlas_authlist.tex:D.~Amidei$^{\rm 89}$,
atlas_authlist.tex:S.P.~Amor~Dos~Santos$^{\rm 126a,126c}$,
atlas_authlist.tex:A.~Amorim$^{\rm 126a,126b}$,
atlas_authlist.tex:S.~Amoroso$^{\rm 48}$,
atlas_authlist.tex:N.~Amram$^{\rm 153}$,
atlas_authlist.tex:G.~Amundsen$^{\rm 23}$,
atlas_authlist.tex:C.~Anastopoulos$^{\rm 139}$,
atlas_authlist.tex:L.S.~Ancu$^{\rm 49}$,
atlas_authlist.tex:N.~Andari$^{\rm 108}$,
atlas_authlist.tex:T.~Andeen$^{\rm 35}$,
atlas_authlist.tex:C.F.~Anders$^{\rm 58b}$,
atlas_authlist.tex:G.~Anders$^{\rm 30}$,
atlas_authlist.tex:J.K.~Anders$^{\rm 74}$,
atlas_authlist.tex:K.J.~Anderson$^{\rm 31}$,
atlas_authlist.tex:A.~Andreazza$^{\rm 91a,91b}$,
atlas_authlist.tex:V.~Andrei$^{\rm 58a}$,
atlas_authlist.tex:S.~Angelidakis$^{\rm 9}$,
atlas_authlist.tex:I.~Angelozzi$^{\rm 107}$,
atlas_authlist.tex:P.~Anger$^{\rm 44}$,
atlas_authlist.tex:A.~Angerami$^{\rm 35}$,
atlas_authlist.tex:F.~Anghinolfi$^{\rm 30}$,
atlas_authlist.tex:A.V.~Anisenkov$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:N.~Anjos$^{\rm 12}$,
atlas_authlist.tex:A.~Annovi$^{\rm 124a,124b}$,
atlas_authlist.tex:M.~Antonelli$^{\rm 47}$,
atlas_authlist.tex:A.~Antonov$^{\rm 98}$,
atlas_authlist.tex:J.~Antos$^{\rm 144b}$,
atlas_authlist.tex:F.~Anulli$^{\rm 132a}$,
atlas_authlist.tex:M.~Aoki$^{\rm 66}$,
atlas_authlist.tex:L.~Aperio~Bella$^{\rm 18}$,
atlas_authlist.tex:G.~Arabidze$^{\rm 90}$,
atlas_authlist.tex:Y.~Arai$^{\rm 66}$,
atlas_authlist.tex:J.P.~Araque$^{\rm 126a}$,
atlas_authlist.tex:A.T.H.~Arce$^{\rm 45}$,
atlas_authlist.tex:F.A.~Arduh$^{\rm 71}$,
atlas_authlist.tex:J-F.~Arguin$^{\rm 95}$,
atlas_authlist.tex:S.~Argyropoulos$^{\rm 42}$,
atlas_authlist.tex:M.~Arik$^{\rm 19a}$,
atlas_authlist.tex:A.J.~Armbruster$^{\rm 30}$,
atlas_authlist.tex:O.~Arnaez$^{\rm 30}$,
atlas_authlist.tex:V.~Arnal$^{\rm 82}$,
atlas_authlist.tex:H.~Arnold$^{\rm 48}$,
atlas_authlist.tex:M.~Arratia$^{\rm 28}$,
atlas_authlist.tex:O.~Arslan$^{\rm 21}$,
atlas_authlist.tex:A.~Artamonov$^{\rm 97}$,
atlas_authlist.tex:G.~Artoni$^{\rm 23}$,
atlas_authlist.tex:S.~Asai$^{\rm 155}$,
atlas_authlist.tex:N.~Asbah$^{\rm 42}$,
atlas_authlist.tex:A.~Ashkenazi$^{\rm 153}$,
atlas_authlist.tex:B.~{\AA}sman$^{\rm 146a,146b}$,
atlas_authlist.tex:L.~Asquith$^{\rm 149}$,
atlas_authlist.tex:K.~Assamagan$^{\rm 25}$,
atlas_authlist.tex:R.~Astalos$^{\rm 144a}$,
atlas_authlist.tex:M.~Atkinson$^{\rm 165}$,
atlas_authlist.tex:N.B.~Atlay$^{\rm 141}$,
atlas_authlist.tex:B.~Auerbach$^{\rm 6}$,
atlas_authlist.tex:K.~Augsten$^{\rm 128}$,
atlas_authlist.tex:M.~Aurousseau$^{\rm 145b}$,
atlas_authlist.tex:G.~Avolio$^{\rm 30}$,
atlas_authlist.tex:B.~Axen$^{\rm 15}$,
atlas_authlist.tex:M.K.~Ayoub$^{\rm 117}$,
atlas_authlist.tex:G.~Azuelos$^{\rm 95}$$^{,d}$,
atlas_authlist.tex:M.A.~Baak$^{\rm 30}$,
atlas_authlist.tex:A.E.~Baas$^{\rm 58a}$,
atlas_authlist.tex:M.J.~Baca$^{\rm 18}$,
atlas_authlist.tex:C.~Bacci$^{\rm 134a,134b}$,
atlas_authlist.tex:H.~Bachacou$^{\rm 136}$,
atlas_authlist.tex:K.~Bachas$^{\rm 154}$,
atlas_authlist.tex:M.~Backes$^{\rm 30}$,
atlas_authlist.tex:M.~Backhaus$^{\rm 30}$,
atlas_authlist.tex:P.~Bagiacchi$^{\rm 132a,132b}$,
atlas_authlist.tex:P.~Bagnaia$^{\rm 132a,132b}$,
atlas_authlist.tex:Y.~Bai$^{\rm 33a}$,
atlas_authlist.tex:T.~Bain$^{\rm 35}$,
atlas_authlist.tex:J.T.~Baines$^{\rm 131}$,
atlas_authlist.tex:O.K.~Baker$^{\rm 176}$,
atlas_authlist.tex:E.M.~Baldin$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:P.~Balek$^{\rm 129}$,
atlas_authlist.tex:T.~Balestri$^{\rm 148}$,
atlas_authlist.tex:F.~Balli$^{\rm 84}$,
atlas_authlist.tex:E.~Banas$^{\rm 39}$,
atlas_authlist.tex:Sw.~Banerjee$^{\rm 173}$,
atlas_authlist.tex:A.A.E.~Bannoura$^{\rm 175}$,
atlas_authlist.tex:H.S.~Bansil$^{\rm 18}$,
atlas_authlist.tex:L.~Barak$^{\rm 30}$,
atlas_authlist.tex:E.L.~Barberio$^{\rm 88}$,
atlas_authlist.tex:D.~Barberis$^{\rm 50a,50b}$,
atlas_authlist.tex:M.~Barbero$^{\rm 85}$,
atlas_authlist.tex:T.~Barillari$^{\rm 101}$,
atlas_authlist.tex:M.~Barisonzi$^{\rm 164a,164b}$,
atlas_authlist.tex:T.~Barklow$^{\rm 143}$,
atlas_authlist.tex:N.~Barlow$^{\rm 28}$,
atlas_authlist.tex:S.L.~Barnes$^{\rm 84}$,
atlas_authlist.tex:B.M.~Barnett$^{\rm 131}$,
atlas_authlist.tex:R.M.~Barnett$^{\rm 15}$,
atlas_authlist.tex:Z.~Barnovska$^{\rm 5}$,
atlas_authlist.tex:A.~Baroncelli$^{\rm 134a}$,
atlas_authlist.tex:G.~Barone$^{\rm 23}$,
atlas_authlist.tex:A.J.~Barr$^{\rm 120}$,
atlas_authlist.tex:F.~Barreiro$^{\rm 82}$,
atlas_authlist.tex:J.~Barreiro~Guimar\~{a}es~da~Costa$^{\rm 57}$,
atlas_authlist.tex:R.~Bartoldus$^{\rm 143}$,
atlas_authlist.tex:A.E.~Barton$^{\rm 72}$,
atlas_authlist.tex:P.~Bartos$^{\rm 144a}$,
atlas_authlist.tex:A.~Basalaev$^{\rm 123}$,
atlas_authlist.tex:A.~Bassalat$^{\rm 117}$,
atlas_authlist.tex:A.~Basye$^{\rm 165}$,
atlas_authlist.tex:R.L.~Bates$^{\rm 53}$,
atlas_authlist.tex:S.J.~Batista$^{\rm 158}$,
atlas_authlist.tex:J.R.~Batley$^{\rm 28}$,
atlas_authlist.tex:M.~Battaglia$^{\rm 137}$,
atlas_authlist.tex:M.~Bauce$^{\rm 132a,132b}$,
atlas_authlist.tex:F.~Bauer$^{\rm 136}$,
atlas_authlist.tex:H.S.~Bawa$^{\rm 143}$$^{,e}$,
atlas_authlist.tex:J.B.~Beacham$^{\rm 111}$,
atlas_authlist.tex:M.D.~Beattie$^{\rm 72}$,
atlas_authlist.tex:T.~Beau$^{\rm 80}$,
atlas_authlist.tex:P.H.~Beauchemin$^{\rm 161}$,
atlas_authlist.tex:R.~Beccherle$^{\rm 124a,124b}$,
atlas_authlist.tex:P.~Bechtle$^{\rm 21}$,
atlas_authlist.tex:H.P.~Beck$^{\rm 17}$$^{,f}$,
atlas_authlist.tex:K.~Becker$^{\rm 120}$,
atlas_authlist.tex:M.~Becker$^{\rm 83}$,
atlas_authlist.tex:S.~Becker$^{\rm 100}$,
atlas_authlist.tex:M.~Beckingham$^{\rm 170}$,
atlas_authlist.tex:C.~Becot$^{\rm 117}$,
atlas_authlist.tex:A.J.~Beddall$^{\rm 19b}$,
atlas_authlist.tex:A.~Beddall$^{\rm 19b}$,
atlas_authlist.tex:V.A.~Bednyakov$^{\rm 65}$,
atlas_authlist.tex:C.P.~Bee$^{\rm 148}$,
atlas_authlist.tex:L.J.~Beemster$^{\rm 107}$,
atlas_authlist.tex:T.A.~Beermann$^{\rm 175}$,
atlas_authlist.tex:M.~Begel$^{\rm 25}$,
atlas_authlist.tex:J.K.~Behr$^{\rm 120}$,
atlas_authlist.tex:C.~Belanger-Champagne$^{\rm 87}$,
atlas_authlist.tex:W.H.~Bell$^{\rm 49}$,
atlas_authlist.tex:G.~Bella$^{\rm 153}$,
atlas_authlist.tex:L.~Bellagamba$^{\rm 20a}$,
atlas_authlist.tex:A.~Bellerive$^{\rm 29}$,
atlas_authlist.tex:M.~Bellomo$^{\rm 86}$,
atlas_authlist.tex:K.~Belotskiy$^{\rm 98}$,
atlas_authlist.tex:O.~Beltramello$^{\rm 30}$,
atlas_authlist.tex:O.~Benary$^{\rm 153}$,
atlas_authlist.tex:D.~Benchekroun$^{\rm 135a}$,
atlas_authlist.tex:M.~Bender$^{\rm 100}$,
atlas_authlist.tex:K.~Bendtz$^{\rm 146a,146b}$,
atlas_authlist.tex:N.~Benekos$^{\rm 10}$,
atlas_authlist.tex:Y.~Benhammou$^{\rm 153}$,
atlas_authlist.tex:E.~Benhar~Noccioli$^{\rm 49}$,
atlas_authlist.tex:J.A.~Benitez~Garcia$^{\rm 159b}$,
atlas_authlist.tex:D.P.~Benjamin$^{\rm 45}$,
atlas_authlist.tex:J.R.~Bensinger$^{\rm 23}$,
atlas_authlist.tex:S.~Bentvelsen$^{\rm 107}$,
atlas_authlist.tex:L.~Beresford$^{\rm 120}$,
atlas_authlist.tex:M.~Beretta$^{\rm 47}$,
atlas_authlist.tex:D.~Berge$^{\rm 107}$,
atlas_authlist.tex:E.~Bergeaas~Kuutmann$^{\rm 166}$,
atlas_authlist.tex:N.~Berger$^{\rm 5}$,
atlas_authlist.tex:F.~Berghaus$^{\rm -290}$,
atlas_authlist.tex:J.~Beringer$^{\rm 15}$,
atlas_authlist.tex:C.~Bernard$^{\rm 22}$,
atlas_authlist.tex:N.R.~Bernard$^{\rm 86}$,
atlas_authlist.tex:C.~Bernius$^{\rm 110}$,
atlas_authlist.tex:F.U.~Bernlochner$^{\rm 21}$,
atlas_authlist.tex:T.~Berry$^{\rm 77}$,
atlas_authlist.tex:P.~Berta$^{\rm 129}$,
atlas_authlist.tex:C.~Bertella$^{\rm 83}$,
atlas_authlist.tex:G.~Bertoli$^{\rm 146a,146b}$,
atlas_authlist.tex:F.~Bertolucci$^{\rm 124a,124b}$,
atlas_authlist.tex:C.~Bertsche$^{\rm 113}$,
atlas_authlist.tex:D.~Bertsche$^{\rm 113}$,
atlas_authlist.tex:M.I.~Besana$^{\rm 91a}$,
atlas_authlist.tex:G.J.~Besjes$^{\rm 36}$,
atlas_authlist.tex:O.~Bessidskaia~Bylund$^{\rm 146a,146b}$,
atlas_authlist.tex:M.~Bessner$^{\rm 42}$,
atlas_authlist.tex:N.~Besson$^{\rm 136}$,
atlas_authlist.tex:C.~Betancourt$^{\rm 48}$,
atlas_authlist.tex:S.~Bethke$^{\rm 101}$,
atlas_authlist.tex:A.J.~Bevan$^{\rm 76}$,
atlas_authlist.tex:W.~Bhimji$^{\rm 15}$,
atlas_authlist.tex:R.M.~Bianchi$^{\rm 125}$,
atlas_authlist.tex:L.~Bianchini$^{\rm 23}$,
atlas_authlist.tex:M.~Bianco$^{\rm 30}$,
atlas_authlist.tex:O.~Biebel$^{\rm 100}$,
atlas_authlist.tex:D.~Biedermann$^{\rm 16}$,
atlas_authlist.tex:S.P.~Bieniek$^{\rm 78}$,
atlas_authlist.tex:M.~Biglietti$^{\rm 134a}$,
atlas_authlist.tex:J.~Bilbao~De~Mendizabal$^{\rm 49}$,
atlas_authlist.tex:H.~Bilokon$^{\rm 47}$,
atlas_authlist.tex:M.~Bindi$^{\rm 54}$,
atlas_authlist.tex:S.~Binet$^{\rm 117}$,
atlas_authlist.tex:A.~Bingul$^{\rm 19b}$,
atlas_authlist.tex:C.~Bini$^{\rm 132a,132b}$,
atlas_authlist.tex:S.~Biondi$^{\rm 20a,20b}$,
atlas_authlist.tex:C.W.~Black$^{\rm 150}$,
atlas_authlist.tex:J.E.~Black$^{\rm 143}$,
atlas_authlist.tex:K.M.~Black$^{\rm 22}$,
atlas_authlist.tex:D.~Blackburn$^{\rm 138}$,
atlas_authlist.tex:R.E.~Blair$^{\rm 6}$,
atlas_authlist.tex:J.-B.~Blanchard$^{\rm 136}$,
atlas_authlist.tex:J.E.~Blanco$^{\rm 77}$,
atlas_authlist.tex:T.~Blazek$^{\rm 144a}$,
atlas_authlist.tex:I.~Bloch$^{\rm 42}$,
atlas_authlist.tex:C.~Blocker$^{\rm 23}$,
atlas_authlist.tex:W.~Blum$^{\rm 83}$$^{,*}$,
atlas_authlist.tex:U.~Blumenschein$^{\rm 54}$,
atlas_authlist.tex:G.J.~Bobbink$^{\rm 107}$,
atlas_authlist.tex:V.S.~Bobrovnikov$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:S.S.~Bocchetta$^{\rm 81}$,
atlas_authlist.tex:A.~Bocci$^{\rm 45}$,
atlas_authlist.tex:C.~Bock$^{\rm 100}$,
atlas_authlist.tex:M.~Boehler$^{\rm 48}$,
atlas_authlist.tex:J.A.~Bogaerts$^{\rm 30}$,
atlas_authlist.tex:D.~Bogavac$^{\rm 13}$,
atlas_authlist.tex:A.G.~Bogdanchikov$^{\rm 109}$,
atlas_authlist.tex:C.~Bohm$^{\rm 146a}$,
atlas_authlist.tex:V.~Boisvert$^{\rm 77}$,
atlas_authlist.tex:T.~Bold$^{\rm 38a}$,
atlas_authlist.tex:V.~Boldea$^{\rm 26a}$,
atlas_authlist.tex:A.S.~Boldyrev$^{\rm 99}$,
atlas_authlist.tex:M.~Bomben$^{\rm 80}$,
atlas_authlist.tex:M.~Bona$^{\rm 76}$,
atlas_authlist.tex:M.~Boonekamp$^{\rm 136}$,
atlas_authlist.tex:A.~Borisov$^{\rm 130}$,
atlas_authlist.tex:G.~Borissov$^{\rm 72}$,
atlas_authlist.tex:S.~Borroni$^{\rm 42}$,
atlas_authlist.tex:J.~Bortfeldt$^{\rm 100}$,
atlas_authlist.tex:V.~Bortolotto$^{\rm 60a,60b,60c}$,
atlas_authlist.tex:K.~Bos$^{\rm 107}$,
atlas_authlist.tex:D.~Boscherini$^{\rm 20a}$,
atlas_authlist.tex:M.~Bosman$^{\rm 12}$,
atlas_authlist.tex:J.~Boudreau$^{\rm 125}$,
atlas_authlist.tex:J.~Bouffard$^{\rm 2}$,
atlas_authlist.tex:E.V.~Bouhova-Thacker$^{\rm 72}$,
atlas_authlist.tex:D.~Boumediene$^{\rm 34}$,
atlas_authlist.tex:C.~Bourdarios$^{\rm 117}$,
atlas_authlist.tex:N.~Bousson$^{\rm 114}$,
atlas_authlist.tex:A.~Boveia$^{\rm 30}$,
atlas_authlist.tex:J.~Boyd$^{\rm 30}$,
atlas_authlist.tex:I.R.~Boyko$^{\rm 65}$,
atlas_authlist.tex:I.~Bozic$^{\rm 13}$,
atlas_authlist.tex:J.~Bracinik$^{\rm 18}$,
atlas_authlist.tex:A.~Brandt$^{\rm 8}$,
atlas_authlist.tex:G.~Brandt$^{\rm 54}$,
atlas_authlist.tex:O.~Brandt$^{\rm 58a}$,
atlas_authlist.tex:U.~Bratzler$^{\rm 156}$,
atlas_authlist.tex:B.~Brau$^{\rm 86}$,
atlas_authlist.tex:J.E.~Brau$^{\rm 116}$,
atlas_authlist.tex:H.M.~Braun$^{\rm 175}$$^{,*}$,
atlas_authlist.tex:S.F.~Brazzale$^{\rm 164a,164c}$,
atlas_authlist.tex:W.D.~Breaden~Madden$^{\rm 53}$,
atlas_authlist.tex:K.~Brendlinger$^{\rm 122}$,
atlas_authlist.tex:A.J.~Brennan$^{\rm 88}$,
atlas_authlist.tex:L.~Brenner$^{\rm 107}$,
atlas_authlist.tex:R.~Brenner$^{\rm 166}$,
atlas_authlist.tex:S.~Bressler$^{\rm 172}$,
atlas_authlist.tex:K.~Bristow$^{\rm 145c}$,
atlas_authlist.tex:T.M.~Bristow$^{\rm 46}$,
atlas_authlist.tex:D.~Britton$^{\rm 53}$,
atlas_authlist.tex:D.~Britzger$^{\rm 42}$,
atlas_authlist.tex:F.M.~Brochu$^{\rm 28}$,
atlas_authlist.tex:I.~Brock$^{\rm 21}$,
atlas_authlist.tex:R.~Brock$^{\rm 90}$,
atlas_authlist.tex:J.~Bronner$^{\rm 101}$,
atlas_authlist.tex:G.~Brooijmans$^{\rm 35}$,
atlas_authlist.tex:T.~Brooks$^{\rm 77}$,
atlas_authlist.tex:W.K.~Brooks$^{\rm 32b}$,
atlas_authlist.tex:J.~Brosamer$^{\rm 15}$,
atlas_authlist.tex:E.~Brost$^{\rm 116}$,
atlas_authlist.tex:J.~Brown$^{\rm 55}$,
atlas_authlist.tex:P.A.~Bruckman~de~Renstrom$^{\rm 39}$,
atlas_authlist.tex:D.~Bruncko$^{\rm 144b}$,
atlas_authlist.tex:R.~Bruneliere$^{\rm 48}$,
atlas_authlist.tex:A.~Bruni$^{\rm 20a}$,
atlas_authlist.tex:G.~Bruni$^{\rm 20a}$,
atlas_authlist.tex:M.~Bruschi$^{\rm 20a}$,
atlas_authlist.tex:N.~Bruscino$^{\rm 21}$,
atlas_authlist.tex:L.~Bryngemark$^{\rm 81}$,
atlas_authlist.tex:T.~Buanes$^{\rm 14}$,
atlas_authlist.tex:Q.~Buat$^{\rm 142}$,
atlas_authlist.tex:P.~Buchholz$^{\rm 141}$,
atlas_authlist.tex:A.G.~Buckley$^{\rm 53}$,
atlas_authlist.tex:S.I.~Buda$^{\rm 26a}$,
atlas_authlist.tex:I.A.~Budagov$^{\rm 65}$,
atlas_authlist.tex:F.~Buehrer$^{\rm 48}$,
atlas_authlist.tex:L.~Bugge$^{\rm 119}$,
atlas_authlist.tex:M.K.~Bugge$^{\rm 119}$,
atlas_authlist.tex:O.~Bulekov$^{\rm 98}$,
atlas_authlist.tex:D.~Bullock$^{\rm 8}$,
atlas_authlist.tex:H.~Burckhart$^{\rm 30}$,
atlas_authlist.tex:S.~Burdin$^{\rm 74}$,
atlas_authlist.tex:B.~Burghgrave$^{\rm 108}$,
atlas_authlist.tex:S.~Burke$^{\rm 131}$,
atlas_authlist.tex:I.~Burmeister$^{\rm 43}$,
atlas_authlist.tex:E.~Busato$^{\rm 34}$,
atlas_authlist.tex:D.~B\"uscher$^{\rm 48}$,
atlas_authlist.tex:V.~B\"uscher$^{\rm 83}$,
atlas_authlist.tex:P.~Bussey$^{\rm 53}$,
atlas_authlist.tex:J.M.~Butler$^{\rm 22}$,
atlas_authlist.tex:A.I.~Butt$^{\rm 3}$,
atlas_authlist.tex:C.M.~Buttar$^{\rm 53}$,
atlas_authlist.tex:J.M.~Butterworth$^{\rm 78}$,
atlas_authlist.tex:P.~Butti$^{\rm 107}$,
atlas_authlist.tex:W.~Buttinger$^{\rm 25}$,
atlas_authlist.tex:A.~Buzatu$^{\rm 53}$,
atlas_authlist.tex:A.R.~Buzykaev$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:S.~Cabrera~Urb\'an$^{\rm 167}$,
atlas_authlist.tex:D.~Caforio$^{\rm 128}$,
atlas_authlist.tex:V.M.~Cairo$^{\rm 37a,37b}$,
atlas_authlist.tex:O.~Cakir$^{\rm 4a}$,
atlas_authlist.tex:N.~Calace$^{\rm 49}$,
atlas_authlist.tex:P.~Calafiura$^{\rm 15}$,
atlas_authlist.tex:A.~Calandri$^{\rm 136}$,
atlas_authlist.tex:G.~Calderini$^{\rm 80}$,
atlas_authlist.tex:P.~Calfayan$^{\rm 100}$,
atlas_authlist.tex:L.P.~Caloba$^{\rm 24a}$,
atlas_authlist.tex:D.~Calvet$^{\rm 34}$,
atlas_authlist.tex:S.~Calvet$^{\rm 34}$,
atlas_authlist.tex:R.~Camacho~Toro$^{\rm 31}$,
atlas_authlist.tex:S.~Camarda$^{\rm 42}$,
atlas_authlist.tex:P.~Camarri$^{\rm 133a,133b}$,
atlas_authlist.tex:D.~Cameron$^{\rm 119}$,
atlas_authlist.tex:R.~Caminal~Armadans$^{\rm 165}$,
atlas_authlist.tex:S.~Campana$^{\rm 30}$,
atlas_authlist.tex:M.~Campanelli$^{\rm 78}$,
atlas_authlist.tex:A.~Campoverde$^{\rm 148}$,
atlas_authlist.tex:V.~Canale$^{\rm 104a,104b}$,
atlas_authlist.tex:A.~Canepa$^{\rm 159a}$,
atlas_authlist.tex:M.~Cano~Bret$^{\rm 33e}$,
atlas_authlist.tex:J.~Cantero$^{\rm 82}$,
atlas_authlist.tex:R.~Cantrill$^{\rm 126a}$,
atlas_authlist.tex:T.~Cao$^{\rm 40}$,
atlas_authlist.tex:M.D.M.~Capeans~Garrido$^{\rm 30}$,
atlas_authlist.tex:I.~Caprini$^{\rm 26a}$,
atlas_authlist.tex:M.~Caprini$^{\rm 26a}$,
atlas_authlist.tex:M.~Capua$^{\rm 37a,37b}$,
atlas_authlist.tex:R.~Caputo$^{\rm 83}$,
atlas_authlist.tex:R.~Cardarelli$^{\rm 133a}$,
atlas_authlist.tex:F.~Cardillo$^{\rm 48}$,
atlas_authlist.tex:T.~Carli$^{\rm 30}$,
atlas_authlist.tex:G.~Carlino$^{\rm 104a}$,
atlas_authlist.tex:L.~Carminati$^{\rm 91a,91b}$,
atlas_authlist.tex:S.~Caron$^{\rm 106}$,
atlas_authlist.tex:E.~Carquin$^{\rm 32a}$,
atlas_authlist.tex:G.D.~Carrillo-Montoya$^{\rm 8}$,
atlas_authlist.tex:J.R.~Carter$^{\rm 28}$,
atlas_authlist.tex:J.~Carvalho$^{\rm 126a,126c}$,
atlas_authlist.tex:D.~Casadei$^{\rm 78}$,
atlas_authlist.tex:M.P.~Casado$^{\rm 12}$,
atlas_authlist.tex:M.~Casolino$^{\rm 12}$,
atlas_authlist.tex:E.~Castaneda-Miranda$^{\rm 145b}$,
atlas_authlist.tex:A.~Castelli$^{\rm 107}$,
atlas_authlist.tex:V.~Castillo~Gimenez$^{\rm 167}$,
atlas_authlist.tex:N.F.~Castro$^{\rm 126a}$$^{,g}$,
atlas_authlist.tex:P.~Catastini$^{\rm 57}$,
atlas_authlist.tex:A.~Catinaccio$^{\rm 30}$,
atlas_authlist.tex:J.R.~Catmore$^{\rm 119}$,
atlas_authlist.tex:A.~Cattai$^{\rm 30}$,
atlas_authlist.tex:J.~Caudron$^{\rm 83}$,
atlas_authlist.tex:V.~Cavaliere$^{\rm 165}$,
atlas_authlist.tex:D.~Cavalli$^{\rm 91a}$,
atlas_authlist.tex:M.~Cavalli-Sforza$^{\rm 12}$,
atlas_authlist.tex:V.~Cavasinni$^{\rm 124a,124b}$,
atlas_authlist.tex:F.~Ceradini$^{\rm 134a,134b}$,
atlas_authlist.tex:B.C.~Cerio$^{\rm 45}$,
atlas_authlist.tex:K.~Cerny$^{\rm 129}$,
atlas_authlist.tex:A.S.~Cerqueira$^{\rm 24b}$,
atlas_authlist.tex:A.~Cerri$^{\rm 149}$,
atlas_authlist.tex:L.~Cerrito$^{\rm 76}$,
atlas_authlist.tex:F.~Cerutti$^{\rm 15}$,
atlas_authlist.tex:M.~Cerv$^{\rm 30}$,
atlas_authlist.tex:A.~Cervelli$^{\rm 17}$,
atlas_authlist.tex:S.A.~Cetin$^{\rm 19c}$,
atlas_authlist.tex:A.~Chafaq$^{\rm 135a}$,
atlas_authlist.tex:D.~Chakraborty$^{\rm 108}$,
atlas_authlist.tex:I.~Chalupkova$^{\rm 129}$,
atlas_authlist.tex:P.~Chang$^{\rm 165}$,
atlas_authlist.tex:J.D.~Chapman$^{\rm 28}$,
atlas_authlist.tex:D.G.~Charlton$^{\rm 18}$,
atlas_authlist.tex:C.C.~Chau$^{\rm 158}$,
atlas_authlist.tex:C.A.~Chavez~Barajas$^{\rm 149}$,
atlas_authlist.tex:S.~Cheatham$^{\rm 152}$,
atlas_authlist.tex:A.~Chegwidden$^{\rm 90}$,
atlas_authlist.tex:S.~Chekanov$^{\rm 6}$,
atlas_authlist.tex:S.V.~Chekulaev$^{\rm 159a}$,
atlas_authlist.tex:G.A.~Chelkov$^{\rm 65}$$^{,h}$,
atlas_authlist.tex:M.A.~Chelstowska$^{\rm 89}$,
atlas_authlist.tex:C.~Chen$^{\rm 64}$,
atlas_authlist.tex:H.~Chen$^{\rm 25}$,
atlas_authlist.tex:K.~Chen$^{\rm 148}$,
atlas_authlist.tex:L.~Chen$^{\rm 33d}$$^{,i}$,
atlas_authlist.tex:S.~Chen$^{\rm 33c}$,
atlas_authlist.tex:X.~Chen$^{\rm 33f}$,
atlas_authlist.tex:Y.~Chen$^{\rm 67}$,
atlas_authlist.tex:H.C.~Cheng$^{\rm 89}$,
atlas_authlist.tex:Y.~Cheng$^{\rm 31}$,
atlas_authlist.tex:A.~Cheplakov$^{\rm 65}$,
atlas_authlist.tex:E.~Cheremushkina$^{\rm 130}$,
atlas_authlist.tex:R.~Cherkaoui~El~Moursli$^{\rm 135e}$,
atlas_authlist.tex:V.~Chernyatin$^{\rm 25}$$^{,*}$,
atlas_authlist.tex:E.~Cheu$^{\rm 7}$,
atlas_authlist.tex:L.~Chevalier$^{\rm 136}$,
atlas_authlist.tex:V.~Chiarella$^{\rm 47}$,
atlas_authlist.tex:G.~Chiarelli$^{\rm 124a,124b}$,
atlas_authlist.tex:J.T.~Childers$^{\rm 6}$,
atlas_authlist.tex:G.~Chiodini$^{\rm 73a}$,
atlas_authlist.tex:A.S.~Chisholm$^{\rm 18}$,
atlas_authlist.tex:R.T.~Chislett$^{\rm 78}$,
atlas_authlist.tex:A.~Chitan$^{\rm 26a}$,
atlas_authlist.tex:M.V.~Chizhov$^{\rm 65}$,
atlas_authlist.tex:K.~Choi$^{\rm 61}$,
atlas_authlist.tex:S.~Chouridou$^{\rm 9}$,
atlas_authlist.tex:B.K.B.~Chow$^{\rm 100}$,
atlas_authlist.tex:V.~Christodoulou$^{\rm 78}$,
atlas_authlist.tex:D.~Chromek-Burckhart$^{\rm 30}$,
atlas_authlist.tex:J.~Chudoba$^{\rm 127}$,
atlas_authlist.tex:A.J.~Chuinard$^{\rm 87}$,
atlas_authlist.tex:J.J.~Chwastowski$^{\rm 39}$,
atlas_authlist.tex:L.~Chytka$^{\rm 115}$,
atlas_authlist.tex:G.~Ciapetti$^{\rm 132a,132b}$,
atlas_authlist.tex:A.K.~Ciftci$^{\rm 4a}$,
atlas_authlist.tex:D.~Cinca$^{\rm 53}$,
atlas_authlist.tex:V.~Cindro$^{\rm 75}$,
atlas_authlist.tex:I.A.~Cioara$^{\rm 21}$,
atlas_authlist.tex:A.~Ciocio$^{\rm 15}$,
atlas_authlist.tex:Z.H.~Citron$^{\rm 172}$,
atlas_authlist.tex:M.~Ciubancan$^{\rm 26a}$,
atlas_authlist.tex:A.~Clark$^{\rm 49}$,
atlas_authlist.tex:B.L.~Clark$^{\rm 57}$,
atlas_authlist.tex:P.J.~Clark$^{\rm 46}$,
atlas_authlist.tex:R.N.~Clarke$^{\rm 15}$,
atlas_authlist.tex:W.~Cleland$^{\rm 125}$,
atlas_authlist.tex:C.~Clement$^{\rm 146a,146b}$,
atlas_authlist.tex:Y.~Coadou$^{\rm 85}$,
atlas_authlist.tex:M.~Cobal$^{\rm 164a,164c}$,
atlas_authlist.tex:A.~Coccaro$^{\rm 138}$,
atlas_authlist.tex:J.~Cochran$^{\rm 64}$,
atlas_authlist.tex:L.~Coffey$^{\rm 23}$,
atlas_authlist.tex:J.G.~Cogan$^{\rm 143}$,
atlas_authlist.tex:L.~Colasurdo$^{\rm 106}$,
atlas_authlist.tex:B.~Cole$^{\rm 35}$,
atlas_authlist.tex:S.~Cole$^{\rm 108}$,
atlas_authlist.tex:A.P.~Colijn$^{\rm 107}$,
atlas_authlist.tex:J.~Collot$^{\rm 55}$,
atlas_authlist.tex:T.~Colombo$^{\rm 58c}$,
atlas_authlist.tex:G.~Compostella$^{\rm 101}$,
atlas_authlist.tex:P.~Conde~Mui\~no$^{\rm 126a,126b}$,
atlas_authlist.tex:E.~Coniavitis$^{\rm 48}$,
atlas_authlist.tex:S.H.~Connell$^{\rm 145b}$,
atlas_authlist.tex:I.A.~Connelly$^{\rm 77}$,
atlas_authlist.tex:S.M.~Consonni$^{\rm 91a,91b}$,
atlas_authlist.tex:V.~Consorti$^{\rm 48}$,
atlas_authlist.tex:S.~Constantinescu$^{\rm 26a}$,
atlas_authlist.tex:C.~Conta$^{\rm 121a,121b}$,
atlas_authlist.tex:G.~Conti$^{\rm 30}$,
atlas_authlist.tex:F.~Conventi$^{\rm 104a}$$^{,j}$,
atlas_authlist.tex:M.~Cooke$^{\rm 15}$,
atlas_authlist.tex:B.D.~Cooper$^{\rm 78}$,
atlas_authlist.tex:A.M.~Cooper-Sarkar$^{\rm 120}$,
atlas_authlist.tex:T.~Cornelissen$^{\rm 175}$,
atlas_authlist.tex:M.~Corradi$^{\rm 20a}$,
atlas_authlist.tex:F.~Corriveau$^{\rm 87}$$^{,k}$,
atlas_authlist.tex:A.~Corso-Radu$^{\rm 163}$,
atlas_authlist.tex:A.~Cortes-Gonzalez$^{\rm 12}$,
atlas_authlist.tex:G.~Cortiana$^{\rm 101}$,
atlas_authlist.tex:G.~Costa$^{\rm 91a}$,
atlas_authlist.tex:M.J.~Costa$^{\rm 167}$,
atlas_authlist.tex:D.~Costanzo$^{\rm 139}$,
atlas_authlist.tex:D.~C\^ot\'e$^{\rm 8}$,
atlas_authlist.tex:G.~Cottin$^{\rm 28}$,
atlas_authlist.tex:G.~Cowan$^{\rm 77}$,
atlas_authlist.tex:B.E.~Cox$^{\rm 84}$,
atlas_authlist.tex:K.~Cranmer$^{\rm 110}$,
atlas_authlist.tex:G.~Cree$^{\rm 29}$,
atlas_authlist.tex:S.~Cr\'ep\'e-Renaudin$^{\rm 55}$,
atlas_authlist.tex:F.~Crescioli$^{\rm 80}$,
atlas_authlist.tex:W.A.~Cribbs$^{\rm 146a,146b}$,
atlas_authlist.tex:M.~Crispin~Ortuzar$^{\rm 120}$,
atlas_authlist.tex:M.~Cristinziani$^{\rm 21}$,
atlas_authlist.tex:V.~Croft$^{\rm 106}$,
atlas_authlist.tex:G.~Crosetti$^{\rm 37a,37b}$,
atlas_authlist.tex:T.~Cuhadar~Donszelmann$^{\rm 139}$,
atlas_authlist.tex:J.~Cummings$^{\rm 176}$,
atlas_authlist.tex:M.~Curatolo$^{\rm 47}$,
atlas_authlist.tex:C.~Cuthbert$^{\rm 150}$,
atlas_authlist.tex:H.~Czirr$^{\rm 141}$,
atlas_authlist.tex:P.~Czodrowski$^{\rm 3}$,
atlas_authlist.tex:S.~D'Auria$^{\rm 53}$,
atlas_authlist.tex:M.~D'Onofrio$^{\rm 74}$,
atlas_authlist.tex:M.J.~Da~Cunha~Sargedas~De~Sousa$^{\rm 126a,126b}$,
atlas_authlist.tex:C.~Da~Via$^{\rm 84}$,
atlas_authlist.tex:W.~Dabrowski$^{\rm 38a}$,
atlas_authlist.tex:A.~Dafinca$^{\rm 120}$,
atlas_authlist.tex:T.~Dai$^{\rm 89}$,
atlas_authlist.tex:O.~Dale$^{\rm 14}$,
atlas_authlist.tex:F.~Dallaire$^{\rm 95}$,
atlas_authlist.tex:C.~Dallapiccola$^{\rm 86}$,
atlas_authlist.tex:M.~Dam$^{\rm 36}$,
atlas_authlist.tex:J.R.~Dandoy$^{\rm 31}$,
atlas_authlist.tex:N.P.~Dang$^{\rm 48}$,
atlas_authlist.tex:A.C.~Daniells$^{\rm 18}$,
atlas_authlist.tex:M.~Danninger$^{\rm 168}$,
atlas_authlist.tex:M.~Dano~Hoffmann$^{\rm 136}$,
atlas_authlist.tex:V.~Dao$^{\rm 48}$,
atlas_authlist.tex:G.~Darbo$^{\rm 50a}$,
atlas_authlist.tex:S.~Darmora$^{\rm 8}$,
atlas_authlist.tex:J.~Dassoulas$^{\rm 3}$,
atlas_authlist.tex:A.~Dattagupta$^{\rm 61}$,
atlas_authlist.tex:W.~Davey$^{\rm 21}$,
atlas_authlist.tex:C.~David$^{\rm 169}$,
atlas_authlist.tex:T.~Davidek$^{\rm 129}$,
atlas_authlist.tex:E.~Davies$^{\rm 120}$$^{,l}$,
atlas_authlist.tex:M.~Davies$^{\rm 153}$,
atlas_authlist.tex:P.~Davison$^{\rm 78}$,
atlas_authlist.tex:Y.~Davygora$^{\rm 58a}$,
atlas_authlist.tex:E.~Dawe$^{\rm 88}$,
atlas_authlist.tex:I.~Dawson$^{\rm 139}$,
atlas_authlist.tex:R.K.~Daya-Ishmukhametova$^{\rm 86}$,
atlas_authlist.tex:K.~De$^{\rm 8}$,
atlas_authlist.tex:R.~de~Asmundis$^{\rm 104a}$,
atlas_authlist.tex:A.~De~Benedetti$^{\rm 113}$,
atlas_authlist.tex:S.~De~Castro$^{\rm 20a,20b}$,
atlas_authlist.tex:S.~De~Cecco$^{\rm 80}$,
atlas_authlist.tex:N.~De~Groot$^{\rm 106}$,
atlas_authlist.tex:P.~de~Jong$^{\rm 107}$,
atlas_authlist.tex:H.~De~la~Torre$^{\rm 82}$,
atlas_authlist.tex:F.~De~Lorenzi$^{\rm 64}$,
atlas_authlist.tex:L.~De~Nooij$^{\rm 107}$,
atlas_authlist.tex:D.~De~Pedis$^{\rm 132a}$,
atlas_authlist.tex:A.~De~Salvo$^{\rm 132a}$,
atlas_authlist.tex:U.~De~Sanctis$^{\rm 149}$,
atlas_authlist.tex:A.~De~Santo$^{\rm 149}$,
atlas_authlist.tex:J.B.~De~Vivie~De~Regie$^{\rm 117}$,
atlas_authlist.tex:W.J.~Dearnaley$^{\rm 72}$,
atlas_authlist.tex:R.~Debbe$^{\rm 25}$,
atlas_authlist.tex:C.~Debenedetti$^{\rm 137}$,
atlas_authlist.tex:D.V.~Dedovich$^{\rm 65}$,
atlas_authlist.tex:I.~Deigaard$^{\rm 107}$,
atlas_authlist.tex:J.~Del~Peso$^{\rm 82}$,
atlas_authlist.tex:T.~Del~Prete$^{\rm 124a,124b}$,
atlas_authlist.tex:D.~Delgove$^{\rm 117}$,
atlas_authlist.tex:F.~Deliot$^{\rm 136}$,
atlas_authlist.tex:C.M.~Delitzsch$^{\rm 49}$,
atlas_authlist.tex:M.~Deliyergiyev$^{\rm 75}$,
atlas_authlist.tex:A.~Dell'Acqua$^{\rm 30}$,
atlas_authlist.tex:L.~Dell'Asta$^{\rm 22}$,
atlas_authlist.tex:M.~Dell'Orso$^{\rm 124a,124b}$,
atlas_authlist.tex:M.~Della~Pietra$^{\rm 104a}$$^{,j}$,
atlas_authlist.tex:D.~della~Volpe$^{\rm 49}$,
atlas_authlist.tex:M.~Delmastro$^{\rm 5}$,
atlas_authlist.tex:P.A.~Delsart$^{\rm 55}$,
atlas_authlist.tex:C.~Deluca$^{\rm 107}$,
atlas_authlist.tex:D.A.~DeMarco$^{\rm 158}$,
atlas_authlist.tex:S.~Demers$^{\rm 176}$,
atlas_authlist.tex:M.~Demichev$^{\rm 65}$,
atlas_authlist.tex:A.~Demilly$^{\rm 80}$,
atlas_authlist.tex:S.P.~Denisov$^{\rm 130}$,
atlas_authlist.tex:D.~Derendarz$^{\rm 39}$,
atlas_authlist.tex:J.E.~Derkaoui$^{\rm 135d}$,
atlas_authlist.tex:F.~Derue$^{\rm 80}$,
atlas_authlist.tex:P.~Dervan$^{\rm 74}$,
atlas_authlist.tex:K.~Desch$^{\rm 21}$,
atlas_authlist.tex:C.~Deterre$^{\rm 42}$,
atlas_authlist.tex:P.O.~Deviveiros$^{\rm 30}$,
atlas_authlist.tex:A.~Dewhurst$^{\rm 131}$,
atlas_authlist.tex:S.~Dhaliwal$^{\rm 23}$,
atlas_authlist.tex:A.~Di~Ciaccio$^{\rm 133a,133b}$,
atlas_authlist.tex:L.~Di~Ciaccio$^{\rm 5}$,
atlas_authlist.tex:A.~Di~Domenico$^{\rm 132a,132b}$,
atlas_authlist.tex:C.~Di~Donato$^{\rm 104a,104b}$,
atlas_authlist.tex:A.~Di~Girolamo$^{\rm 30}$,
atlas_authlist.tex:B.~Di~Girolamo$^{\rm 30}$,
atlas_authlist.tex:A.~Di~Mattia$^{\rm 152}$,
atlas_authlist.tex:B.~Di~Micco$^{\rm 134a,134b}$,
atlas_authlist.tex:R.~Di~Nardo$^{\rm 47}$,
atlas_authlist.tex:A.~Di~Simone$^{\rm 48}$,
atlas_authlist.tex:R.~Di~Sipio$^{\rm 158}$,
atlas_authlist.tex:D.~Di~Valentino$^{\rm 29}$,
atlas_authlist.tex:C.~Diaconu$^{\rm 85}$,
atlas_authlist.tex:M.~Diamond$^{\rm 158}$,
atlas_authlist.tex:F.A.~Dias$^{\rm 46}$,
atlas_authlist.tex:M.A.~Diaz$^{\rm 32a}$,
atlas_authlist.tex:E.B.~Diehl$^{\rm 89}$,
atlas_authlist.tex:J.~Dietrich$^{\rm 16}$,
atlas_authlist.tex:S.~Diglio$^{\rm 85}$,
atlas_authlist.tex:A.~Dimitrievska$^{\rm 13}$,
atlas_authlist.tex:J.~Dingfelder$^{\rm 21}$,
atlas_authlist.tex:P.~Dita$^{\rm 26a}$,
atlas_authlist.tex:S.~Dita$^{\rm 26a}$,
atlas_authlist.tex:F.~Dittus$^{\rm 30}$,
atlas_authlist.tex:F.~Djama$^{\rm 85}$,
atlas_authlist.tex:T.~Djobava$^{\rm 51b}$,
atlas_authlist.tex:J.I.~Djuvsland$^{\rm 58a}$,
atlas_authlist.tex:M.A.B.~do~Vale$^{\rm 24c}$,
atlas_authlist.tex:D.~Dobos$^{\rm 30}$,
atlas_authlist.tex:M.~Dobre$^{\rm 26a}$,
atlas_authlist.tex:C.~Doglioni$^{\rm 81}$,
atlas_authlist.tex:T.~Dohmae$^{\rm 155}$,
atlas_authlist.tex:J.~Dolejsi$^{\rm 129}$,
atlas_authlist.tex:Z.~Dolezal$^{\rm 129}$,
atlas_authlist.tex:B.A.~Dolgoshein$^{\rm 98}$$^{,*}$,
atlas_authlist.tex:M.~Donadelli$^{\rm 24d}$,
atlas_authlist.tex:S.~Donati$^{\rm 124a,124b}$,
atlas_authlist.tex:P.~Dondero$^{\rm 121a,121b}$,
atlas_authlist.tex:J.~Donini$^{\rm 34}$,
atlas_authlist.tex:J.~Dopke$^{\rm 131}$,
atlas_authlist.tex:A.~Doria$^{\rm 104a}$,
atlas_authlist.tex:M.T.~Dova$^{\rm 71}$,
atlas_authlist.tex:A.T.~Doyle$^{\rm 53}$,
atlas_authlist.tex:E.~Drechsler$^{\rm 54}$,
atlas_authlist.tex:M.~Dris$^{\rm 10}$,
atlas_authlist.tex:E.~Dubreuil$^{\rm 34}$,
atlas_authlist.tex:E.~Duchovni$^{\rm 172}$,
atlas_authlist.tex:G.~Duckeck$^{\rm 100}$,
atlas_authlist.tex:O.A.~Ducu$^{\rm 26a,85}$,
atlas_authlist.tex:D.~Duda$^{\rm 107}$,
atlas_authlist.tex:A.~Dudarev$^{\rm 30}$,
atlas_authlist.tex:L.~Duflot$^{\rm 117}$,
atlas_authlist.tex:L.~Duguid$^{\rm 77}$,
atlas_authlist.tex:M.~D\"uhrssen$^{\rm 30}$,
atlas_authlist.tex:M.~Dunford$^{\rm 58a}$,
atlas_authlist.tex:H.~Duran~Yildiz$^{\rm 4a}$,
atlas_authlist.tex:M.~D\"uren$^{\rm 52}$,
atlas_authlist.tex:A.~Durglishvili$^{\rm 51b}$,
atlas_authlist.tex:D.~Duschinger$^{\rm 44}$,
atlas_authlist.tex:M.~Dyndal$^{\rm 38a}$,
atlas_authlist.tex:C.~Eckardt$^{\rm 42}$,
atlas_authlist.tex:K.M.~Ecker$^{\rm 101}$,
atlas_authlist.tex:R.C.~Edgar$^{\rm 89}$,
atlas_authlist.tex:W.~Edson$^{\rm 2}$,
atlas_authlist.tex:N.C.~Edwards$^{\rm 46}$,
atlas_authlist.tex:W.~Ehrenfeld$^{\rm 21}$,
atlas_authlist.tex:T.~Eifert$^{\rm 30}$,
atlas_authlist.tex:G.~Eigen$^{\rm 14}$,
atlas_authlist.tex:K.~Einsweiler$^{\rm 15}$,
atlas_authlist.tex:T.~Ekelof$^{\rm 166}$,
atlas_authlist.tex:M.~El~Kacimi$^{\rm 135c}$,
atlas_authlist.tex:M.~Ellert$^{\rm 166}$,
atlas_authlist.tex:S.~Elles$^{\rm 5}$,
atlas_authlist.tex:F.~Ellinghaus$^{\rm 175}$,
atlas_authlist.tex:A.A.~Elliot$^{\rm 169}$,
atlas_authlist.tex:N.~Ellis$^{\rm 30}$,
atlas_authlist.tex:J.~Elmsheuser$^{\rm 100}$,
atlas_authlist.tex:M.~Elsing$^{\rm 30}$,
atlas_authlist.tex:D.~Emeliyanov$^{\rm 131}$,
atlas_authlist.tex:Y.~Enari$^{\rm 155}$,
atlas_authlist.tex:O.C.~Endner$^{\rm 83}$,
atlas_authlist.tex:M.~Endo$^{\rm 118}$,
atlas_authlist.tex:J.~Erdmann$^{\rm 43}$,
atlas_authlist.tex:A.~Ereditato$^{\rm 17}$,
atlas_authlist.tex:G.~Ernis$^{\rm 175}$,
atlas_authlist.tex:J.~Ernst$^{\rm 2}$,
atlas_authlist.tex:M.~Ernst$^{\rm 25}$,
atlas_authlist.tex:S.~Errede$^{\rm 165}$,
atlas_authlist.tex:E.~Ertel$^{\rm 83}$,
atlas_authlist.tex:M.~Escalier$^{\rm 117}$,
atlas_authlist.tex:H.~Esch$^{\rm 43}$,
atlas_authlist.tex:C.~Escobar$^{\rm 125}$,
atlas_authlist.tex:B.~Esposito$^{\rm 47}$,
atlas_authlist.tex:A.I.~Etienvre$^{\rm 136}$,
atlas_authlist.tex:E.~Etzion$^{\rm 153}$,
atlas_authlist.tex:H.~Evans$^{\rm 61}$,
atlas_authlist.tex:A.~Ezhilov$^{\rm 123}$,
atlas_authlist.tex:L.~Fabbri$^{\rm 20a,20b}$,
atlas_authlist.tex:G.~Facini$^{\rm 31}$,
atlas_authlist.tex:R.M.~Fakhrutdinov$^{\rm 130}$,
atlas_authlist.tex:S.~Falciano$^{\rm 132a}$,
atlas_authlist.tex:R.J.~Falla$^{\rm 78}$,
atlas_authlist.tex:J.~Faltova$^{\rm 129}$,
atlas_authlist.tex:Y.~Fang$^{\rm 33a}$,
atlas_authlist.tex:M.~Fanti$^{\rm 91a,91b}$,
atlas_authlist.tex:A.~Farbin$^{\rm 8}$,
atlas_authlist.tex:A.~Farilla$^{\rm 134a}$,
atlas_authlist.tex:T.~Farooque$^{\rm 12}$,
atlas_authlist.tex:S.~Farrell$^{\rm 15}$,
atlas_authlist.tex:S.M.~Farrington$^{\rm 170}$,
atlas_authlist.tex:P.~Farthouat$^{\rm 30}$,
atlas_authlist.tex:F.~Fassi$^{\rm 135e}$,
atlas_authlist.tex:P.~Fassnacht$^{\rm 30}$,
atlas_authlist.tex:D.~Fassouliotis$^{\rm 9}$,
atlas_authlist.tex:M.~Faucci~Giannelli$^{\rm 77}$,
atlas_authlist.tex:A.~Favareto$^{\rm 50a,50b}$,
atlas_authlist.tex:L.~Fayard$^{\rm 117}$,
atlas_authlist.tex:P.~Federic$^{\rm 144a}$,
atlas_authlist.tex:O.L.~Fedin$^{\rm 123}$$^{,m}$,
atlas_authlist.tex:W.~Fedorko$^{\rm 168}$,
atlas_authlist.tex:S.~Feigl$^{\rm 30}$,
atlas_authlist.tex:L.~Feligioni$^{\rm 85}$,
atlas_authlist.tex:C.~Feng$^{\rm 33d}$,
atlas_authlist.tex:E.J.~Feng$^{\rm 6}$,
atlas_authlist.tex:H.~Feng$^{\rm 89}$,
atlas_authlist.tex:A.B.~Fenyuk$^{\rm 130}$,
atlas_authlist.tex:L.~Feremenga$^{\rm 8}$,
atlas_authlist.tex:P.~Fernandez~Martinez$^{\rm 167}$,
atlas_authlist.tex:S.~Fernandez~Perez$^{\rm 30}$,
atlas_authlist.tex:J.~Ferrando$^{\rm 53}$,
atlas_authlist.tex:A.~Ferrari$^{\rm 166}$,
atlas_authlist.tex:P.~Ferrari$^{\rm 107}$,
atlas_authlist.tex:R.~Ferrari$^{\rm 121a}$,
atlas_authlist.tex:D.E.~Ferreira~de~Lima$^{\rm 53}$,
atlas_authlist.tex:A.~Ferrer$^{\rm 167}$,
atlas_authlist.tex:D.~Ferrere$^{\rm 49}$,
atlas_authlist.tex:C.~Ferretti$^{\rm 89}$,
atlas_authlist.tex:A.~Ferretto~Parodi$^{\rm 50a,50b}$,
atlas_authlist.tex:M.~Fiascaris$^{\rm 31}$,
atlas_authlist.tex:F.~Fiedler$^{\rm 83}$,
atlas_authlist.tex:A.~Filip\v{c}i\v{c}$^{\rm 75}$,
atlas_authlist.tex:M.~Filipuzzi$^{\rm 42}$,
atlas_authlist.tex:F.~Filthaut$^{\rm 106}$,
atlas_authlist.tex:M.~Fincke-Keeler$^{\rm 169}$,
atlas_authlist.tex:K.D.~Finelli$^{\rm 150}$,
atlas_authlist.tex:M.C.N.~Fiolhais$^{\rm 126a,126c}$,
atlas_authlist.tex:L.~Fiorini$^{\rm 167}$,
atlas_authlist.tex:A.~Firan$^{\rm 40}$,
atlas_authlist.tex:A.~Fischer$^{\rm 2}$,
atlas_authlist.tex:C.~Fischer$^{\rm 12}$,
atlas_authlist.tex:J.~Fischer$^{\rm 175}$,
atlas_authlist.tex:W.C.~Fisher$^{\rm 90}$,
atlas_authlist.tex:E.A.~Fitzgerald$^{\rm 23}$,
atlas_authlist.tex:N.~Flaschel$^{\rm 42}$,
atlas_authlist.tex:I.~Fleck$^{\rm 141}$,
atlas_authlist.tex:P.~Fleischmann$^{\rm 89}$,
atlas_authlist.tex:S.~Fleischmann$^{\rm 175}$,
atlas_authlist.tex:G.T.~Fletcher$^{\rm 139}$,
atlas_authlist.tex:G.~Fletcher$^{\rm 76}$,
atlas_authlist.tex:R.R.M.~Fletcher$^{\rm 122}$,
atlas_authlist.tex:T.~Flick$^{\rm 175}$,
atlas_authlist.tex:A.~Floderus$^{\rm 81}$,
atlas_authlist.tex:L.R.~Flores~Castillo$^{\rm 60a}$,
atlas_authlist.tex:M.J.~Flowerdew$^{\rm 101}$,
atlas_authlist.tex:A.~Formica$^{\rm 136}$,
atlas_authlist.tex:A.~Forti$^{\rm 84}$,
atlas_authlist.tex:D.~Fournier$^{\rm 117}$,
atlas_authlist.tex:H.~Fox$^{\rm 72}$,
atlas_authlist.tex:S.~Fracchia$^{\rm 12}$,
atlas_authlist.tex:P.~Francavilla$^{\rm 80}$,
atlas_authlist.tex:M.~Franchini$^{\rm 20a,20b}$,
atlas_authlist.tex:D.~Francis$^{\rm 30}$,
atlas_authlist.tex:L.~Franconi$^{\rm 119}$,
atlas_authlist.tex:M.~Franklin$^{\rm 57}$,
atlas_authlist.tex:M.~Frate$^{\rm 163}$,
atlas_authlist.tex:M.~Fraternali$^{\rm 121a,121b}$,
atlas_authlist.tex:D.~Freeborn$^{\rm 78}$,
atlas_authlist.tex:S.T.~French$^{\rm 28}$,
atlas_authlist.tex:F.~Friedrich$^{\rm 44}$,
atlas_authlist.tex:D.~Froidevaux$^{\rm 30}$,
atlas_authlist.tex:J.A.~Frost$^{\rm 120}$,
atlas_authlist.tex:C.~Fukunaga$^{\rm 156}$,
atlas_authlist.tex:E.~Fullana~Torregrosa$^{\rm 83}$,
atlas_authlist.tex:B.G.~Fulsom$^{\rm 143}$,
atlas_authlist.tex:T.~Fusayasu$^{\rm 102}$,
atlas_authlist.tex:J.~Fuster$^{\rm 167}$,
atlas_authlist.tex:C.~Gabaldon$^{\rm 55}$,
atlas_authlist.tex:O.~Gabizon$^{\rm 175}$,
atlas_authlist.tex:A.~Gabrielli$^{\rm 20a,20b}$,
atlas_authlist.tex:A.~Gabrielli$^{\rm 132a,132b}$,
atlas_authlist.tex:G.P.~Gach$^{\rm 38a}$,
atlas_authlist.tex:S.~Gadatsch$^{\rm 107}$,
atlas_authlist.tex:S.~Gadomski$^{\rm 49}$,
atlas_authlist.tex:G.~Gagliardi$^{\rm 50a,50b}$,
atlas_authlist.tex:P.~Gagnon$^{\rm 61}$,
atlas_authlist.tex:C.~Galea$^{\rm 106}$,
atlas_authlist.tex:B.~Galhardo$^{\rm 126a,126c}$,
atlas_authlist.tex:E.J.~Gallas$^{\rm 120}$,
atlas_authlist.tex:B.J.~Gallop$^{\rm 131}$,
atlas_authlist.tex:P.~Gallus$^{\rm 128}$,
atlas_authlist.tex:G.~Galster$^{\rm 36}$,
atlas_authlist.tex:K.K.~Gan$^{\rm 111}$,
atlas_authlist.tex:J.~Gao$^{\rm 33b,85}$,
atlas_authlist.tex:Y.~Gao$^{\rm 46}$,
atlas_authlist.tex:Y.S.~Gao$^{\rm 143}$$^{,e}$,
atlas_authlist.tex:F.M.~Garay~Walls$^{\rm 46}$,
atlas_authlist.tex:F.~Garberson$^{\rm 176}$,
atlas_authlist.tex:C.~Garc\'ia$^{\rm 167}$,
atlas_authlist.tex:J.E.~Garc\'ia~Navarro$^{\rm 167}$,
atlas_authlist.tex:M.~Garcia-Sciveres$^{\rm 15}$,
atlas_authlist.tex:R.W.~Gardner$^{\rm 31}$,
atlas_authlist.tex:N.~Garelli$^{\rm 143}$,
atlas_authlist.tex:V.~Garonne$^{\rm 119}$,
atlas_authlist.tex:C.~Gatti$^{\rm 47}$,
atlas_authlist.tex:A.~Gaudiello$^{\rm 50a,50b}$,
atlas_authlist.tex:G.~Gaudio$^{\rm 121a}$,
atlas_authlist.tex:B.~Gaur$^{\rm 141}$,
atlas_authlist.tex:L.~Gauthier$^{\rm 95}$,
atlas_authlist.tex:P.~Gauzzi$^{\rm 132a,132b}$,
atlas_authlist.tex:I.L.~Gavrilenko$^{\rm 96}$,
atlas_authlist.tex:C.~Gay$^{\rm 168}$,
atlas_authlist.tex:G.~Gaycken$^{\rm 21}$,
atlas_authlist.tex:E.N.~Gazis$^{\rm 10}$,
atlas_authlist.tex:P.~Ge$^{\rm 33d}$,
atlas_authlist.tex:Z.~Gecse$^{\rm 168}$,
atlas_authlist.tex:C.N.P.~Gee$^{\rm 131}$,
atlas_authlist.tex:D.A.A.~Geerts$^{\rm 107}$,
atlas_authlist.tex:Ch.~Geich-Gimbel$^{\rm 21}$,
atlas_authlist.tex:M.P.~Geisler$^{\rm 58a}$,
atlas_authlist.tex:C.~Gemme$^{\rm 50a}$,
atlas_authlist.tex:M.H.~Genest$^{\rm 55}$,
atlas_authlist.tex:S.~Gentile$^{\rm 132a,132b}$,
atlas_authlist.tex:M.~George$^{\rm 54}$,
atlas_authlist.tex:S.~George$^{\rm 77}$,
atlas_authlist.tex:D.~Gerbaudo$^{\rm 163}$,
atlas_authlist.tex:A.~Gershon$^{\rm 153}$,
atlas_authlist.tex:S.~Ghasemi$^{\rm 141}$,
atlas_authlist.tex:H.~Ghazlane$^{\rm 135b}$,
atlas_authlist.tex:B.~Giacobbe$^{\rm 20a}$,
atlas_authlist.tex:S.~Giagu$^{\rm 132a,132b}$,
atlas_authlist.tex:V.~Giangiobbe$^{\rm 12}$,
atlas_authlist.tex:P.~Giannetti$^{\rm 124a,124b}$,
atlas_authlist.tex:B.~Gibbard$^{\rm 25}$,
atlas_authlist.tex:S.M.~Gibson$^{\rm 77}$,
atlas_authlist.tex:M.~Gilchriese$^{\rm 15}$,
atlas_authlist.tex:T.P.S.~Gillam$^{\rm 28}$,
atlas_authlist.tex:D.~Gillberg$^{\rm 30}$,
atlas_authlist.tex:G.~Gilles$^{\rm 34}$,
atlas_authlist.tex:D.M.~Gingrich$^{\rm 3}$$^{,d}$,
atlas_authlist.tex:N.~Giokaris$^{\rm 9}$,
atlas_authlist.tex:M.P.~Giordani$^{\rm 164a,164c}$,
atlas_authlist.tex:F.M.~Giorgi$^{\rm 20a}$,
atlas_authlist.tex:F.M.~Giorgi$^{\rm 16}$,
atlas_authlist.tex:P.F.~Giraud$^{\rm 136}$,
atlas_authlist.tex:P.~Giromini$^{\rm 47}$,
atlas_authlist.tex:D.~Giugni$^{\rm 91a}$,
atlas_authlist.tex:C.~Giuliani$^{\rm 48}$,
atlas_authlist.tex:M.~Giulini$^{\rm 58b}$,
atlas_authlist.tex:B.K.~Gjelsten$^{\rm 119}$,
atlas_authlist.tex:S.~Gkaitatzis$^{\rm 154}$,
atlas_authlist.tex:I.~Gkialas$^{\rm 154}$,
atlas_authlist.tex:E.L.~Gkougkousis$^{\rm 117}$,
atlas_authlist.tex:L.K.~Gladilin$^{\rm 99}$,
atlas_authlist.tex:C.~Glasman$^{\rm 82}$,
atlas_authlist.tex:J.~Glatzer$^{\rm 30}$,
atlas_authlist.tex:P.C.F.~Glaysher$^{\rm 46}$,
atlas_authlist.tex:A.~Glazov$^{\rm 42}$,
atlas_authlist.tex:M.~Goblirsch-Kolb$^{\rm 101}$,
atlas_authlist.tex:J.R.~Goddard$^{\rm 76}$,
atlas_authlist.tex:J.~Godlewski$^{\rm 39}$,
atlas_authlist.tex:S.~Goldfarb$^{\rm 89}$,
atlas_authlist.tex:T.~Golling$^{\rm 49}$,
atlas_authlist.tex:D.~Golubkov$^{\rm 130}$,
atlas_authlist.tex:A.~Gomes$^{\rm 126a,126b,126d}$,
atlas_authlist.tex:R.~Gon\c{c}alo$^{\rm 126a}$,
atlas_authlist.tex:J.~Goncalves~Pinto~Firmino~Da~Costa$^{\rm 136}$,
atlas_authlist.tex:L.~Gonella$^{\rm 21}$,
atlas_authlist.tex:S.~Gonz\'alez~de~la~Hoz$^{\rm 167}$,
atlas_authlist.tex:G.~Gonzalez~Parra$^{\rm 12}$,
atlas_authlist.tex:S.~Gonzalez-Sevilla$^{\rm 49}$,
atlas_authlist.tex:L.~Goossens$^{\rm 30}$,
atlas_authlist.tex:P.A.~Gorbounov$^{\rm 97}$,
atlas_authlist.tex:H.A.~Gordon$^{\rm 25}$,
atlas_authlist.tex:I.~Gorelov$^{\rm 105}$,
atlas_authlist.tex:B.~Gorini$^{\rm 30}$,
atlas_authlist.tex:E.~Gorini$^{\rm 73a,73b}$,
atlas_authlist.tex:A.~Gori\v{s}ek$^{\rm 75}$,
atlas_authlist.tex:E.~Gornicki$^{\rm 39}$,
atlas_authlist.tex:A.T.~Goshaw$^{\rm 45}$,
atlas_authlist.tex:C.~G\"ossling$^{\rm 43}$,
atlas_authlist.tex:M.I.~Gostkin$^{\rm 65}$,
atlas_authlist.tex:D.~Goujdami$^{\rm 135c}$,
atlas_authlist.tex:A.G.~Goussiou$^{\rm 138}$,
atlas_authlist.tex:N.~Govender$^{\rm 145b}$,
atlas_authlist.tex:E.~Gozani$^{\rm 152}$,
atlas_authlist.tex:H.M.X.~Grabas$^{\rm 137}$,
atlas_authlist.tex:L.~Graber$^{\rm 54}$,
atlas_authlist.tex:I.~Grabowska-Bold$^{\rm 38a}$,
atlas_authlist.tex:P.O.J.~Gradin$^{\rm 166}$,
atlas_authlist.tex:P.~Grafstr\"om$^{\rm 20a,20b}$,
atlas_authlist.tex:K-J.~Grahn$^{\rm 42}$,
atlas_authlist.tex:J.~Gramling$^{\rm 49}$,
atlas_authlist.tex:E.~Gramstad$^{\rm 119}$,
atlas_authlist.tex:S.~Grancagnolo$^{\rm 16}$,
atlas_authlist.tex:V.~Grassi$^{\rm 148}$,
atlas_authlist.tex:V.~Gratchev$^{\rm 123}$,
atlas_authlist.tex:H.M.~Gray$^{\rm 30}$,
atlas_authlist.tex:E.~Graziani$^{\rm 134a}$,
atlas_authlist.tex:Z.D.~Greenwood$^{\rm 79}$$^{,n}$,
atlas_authlist.tex:K.~Gregersen$^{\rm 78}$,
atlas_authlist.tex:I.M.~Gregor$^{\rm 42}$,
atlas_authlist.tex:P.~Grenier$^{\rm 143}$,
atlas_authlist.tex:J.~Griffiths$^{\rm 8}$,
atlas_authlist.tex:A.A.~Grillo$^{\rm 137}$,
atlas_authlist.tex:K.~Grimm$^{\rm 72}$,
atlas_authlist.tex:S.~Grinstein$^{\rm 12}$$^{,o}$,
atlas_authlist.tex:Ph.~Gris$^{\rm 34}$,
atlas_authlist.tex:J.-F.~Grivaz$^{\rm 117}$,
atlas_authlist.tex:J.P.~Grohs$^{\rm 44}$,
atlas_authlist.tex:A.~Grohsjean$^{\rm 42}$,
atlas_authlist.tex:E.~Gross$^{\rm 172}$,
atlas_authlist.tex:J.~Grosse-Knetter$^{\rm 54}$,
atlas_authlist.tex:G.C.~Grossi$^{\rm 79}$,
atlas_authlist.tex:Z.J.~Grout$^{\rm 149}$,
atlas_authlist.tex:L.~Guan$^{\rm 89}$,
atlas_authlist.tex:J.~Guenther$^{\rm 128}$,
atlas_authlist.tex:F.~Guescini$^{\rm 49}$,
atlas_authlist.tex:D.~Guest$^{\rm 176}$,
atlas_authlist.tex:O.~Gueta$^{\rm 153}$,
atlas_authlist.tex:E.~Guido$^{\rm 50a,50b}$,
atlas_authlist.tex:T.~Guillemin$^{\rm 117}$,
atlas_authlist.tex:S.~Guindon$^{\rm 2}$,
atlas_authlist.tex:U.~Gul$^{\rm 53}$,
atlas_authlist.tex:C.~Gumpert$^{\rm 44}$,
atlas_authlist.tex:J.~Guo$^{\rm 33e}$,
atlas_authlist.tex:Y.~Guo$^{\rm 33b}$,
atlas_authlist.tex:S.~Gupta$^{\rm 120}$,
atlas_authlist.tex:G.~Gustavino$^{\rm 132a,132b}$,
atlas_authlist.tex:P.~Gutierrez$^{\rm 113}$,
atlas_authlist.tex:N.G.~Gutierrez~Ortiz$^{\rm 78}$,
atlas_authlist.tex:C.~Gutschow$^{\rm 44}$,
atlas_authlist.tex:C.~Guyot$^{\rm 136}$,
atlas_authlist.tex:C.~Gwenlan$^{\rm 120}$,
atlas_authlist.tex:C.B.~Gwilliam$^{\rm 74}$,
atlas_authlist.tex:A.~Haas$^{\rm 110}$,
atlas_authlist.tex:C.~Haber$^{\rm 15}$,
atlas_authlist.tex:H.K.~Hadavand$^{\rm 8}$,
atlas_authlist.tex:N.~Haddad$^{\rm 135e}$,
atlas_authlist.tex:P.~Haefner$^{\rm 21}$,
atlas_authlist.tex:S.~Hageb\"ock$^{\rm 21}$,
atlas_authlist.tex:Z.~Hajduk$^{\rm 39}$,
atlas_authlist.tex:H.~Hakobyan$^{\rm 177}$,
atlas_authlist.tex:M.~Haleem$^{\rm 42}$,
atlas_authlist.tex:J.~Haley$^{\rm 114}$,
atlas_authlist.tex:D.~Hall$^{\rm 120}$,
atlas_authlist.tex:G.~Halladjian$^{\rm 90}$,
atlas_authlist.tex:G.D.~Hallewell$^{\rm 85}$,
atlas_authlist.tex:K.~Hamacher$^{\rm 175}$,
atlas_authlist.tex:P.~Hamal$^{\rm 115}$,
atlas_authlist.tex:K.~Hamano$^{\rm 169}$,
atlas_authlist.tex:M.~Hamer$^{\rm 54}$,
atlas_authlist.tex:A.~Hamilton$^{\rm 145a}$,
atlas_authlist.tex:G.N.~Hamity$^{\rm 145c}$,
atlas_authlist.tex:P.G.~Hamnett$^{\rm 42}$,
atlas_authlist.tex:L.~Han$^{\rm 33b}$,
atlas_authlist.tex:K.~Hanagaki$^{\rm 66}$$^{,p}$,
atlas_authlist.tex:K.~Hanawa$^{\rm 155}$,
atlas_authlist.tex:M.~Hance$^{\rm 15}$,
atlas_authlist.tex:P.~Hanke$^{\rm 58a}$,
atlas_authlist.tex:R.~Hanna$^{\rm 136}$,
atlas_authlist.tex:J.B.~Hansen$^{\rm 36}$,
atlas_authlist.tex:J.D.~Hansen$^{\rm 36}$,
atlas_authlist.tex:M.C.~Hansen$^{\rm 21}$,
atlas_authlist.tex:P.H.~Hansen$^{\rm 36}$,
atlas_authlist.tex:K.~Hara$^{\rm 160}$,
atlas_authlist.tex:A.S.~Hard$^{\rm 173}$,
atlas_authlist.tex:T.~Harenberg$^{\rm 175}$,
atlas_authlist.tex:F.~Hariri$^{\rm 117}$,
atlas_authlist.tex:S.~Harkusha$^{\rm 92}$,
atlas_authlist.tex:R.D.~Harrington$^{\rm 46}$,
atlas_authlist.tex:P.F.~Harrison$^{\rm 170}$,
atlas_authlist.tex:F.~Hartjes$^{\rm 107}$,
atlas_authlist.tex:M.~Hasegawa$^{\rm 67}$,
atlas_authlist.tex:S.~Hasegawa$^{\rm 103}$,
atlas_authlist.tex:Y.~Hasegawa$^{\rm 140}$,
atlas_authlist.tex:A.~Hasib$^{\rm 113}$,
atlas_authlist.tex:S.~Hassani$^{\rm 136}$,
atlas_authlist.tex:S.~Haug$^{\rm 17}$,
atlas_authlist.tex:R.~Hauser$^{\rm 90}$,
atlas_authlist.tex:L.~Hauswald$^{\rm 44}$,
atlas_authlist.tex:M.~Havranek$^{\rm 127}$,
atlas_authlist.tex:C.M.~Hawkes$^{\rm 18}$,
atlas_authlist.tex:R.J.~Hawkings$^{\rm 30}$,
atlas_authlist.tex:A.D.~Hawkins$^{\rm 81}$,
atlas_authlist.tex:T.~Hayashi$^{\rm 160}$,
atlas_authlist.tex:D.~Hayden$^{\rm 90}$,
atlas_authlist.tex:C.P.~Hays$^{\rm 120}$,
atlas_authlist.tex:J.M.~Hays$^{\rm 76}$,
atlas_authlist.tex:H.S.~Hayward$^{\rm 74}$,
atlas_authlist.tex:S.J.~Haywood$^{\rm 131}$,
atlas_authlist.tex:S.J.~Head$^{\rm 18}$,
atlas_authlist.tex:T.~Heck$^{\rm 83}$,
atlas_authlist.tex:V.~Hedberg$^{\rm 81}$,
atlas_authlist.tex:L.~Heelan$^{\rm 8}$,
atlas_authlist.tex:S.~Heim$^{\rm 122}$,
atlas_authlist.tex:T.~Heim$^{\rm 175}$,
atlas_authlist.tex:B.~Heinemann$^{\rm 15}$,
atlas_authlist.tex:L.~Heinrich$^{\rm 110}$,
atlas_authlist.tex:J.~Hejbal$^{\rm 127}$,
atlas_authlist.tex:L.~Helary$^{\rm 22}$,
atlas_authlist.tex:S.~Hellman$^{\rm 146a,146b}$,
atlas_authlist.tex:D.~Hellmich$^{\rm 21}$,
atlas_authlist.tex:C.~Helsens$^{\rm 12}$,
atlas_authlist.tex:J.~Henderson$^{\rm 120}$,
atlas_authlist.tex:R.C.W.~Henderson$^{\rm 72}$,
atlas_authlist.tex:Y.~Heng$^{\rm 173}$,
atlas_authlist.tex:C.~Hengler$^{\rm 42}$,
atlas_authlist.tex:A.~Henrichs$^{\rm 176}$,
atlas_authlist.tex:A.M.~Henriques~Correia$^{\rm 30}$,
atlas_authlist.tex:S.~Henrot-Versille$^{\rm 117}$,
atlas_authlist.tex:G.H.~Herbert$^{\rm 16}$,
atlas_authlist.tex:Y.~Hern\'andez~Jim\'enez$^{\rm 167}$,
atlas_authlist.tex:R.~Herrberg-Schubert$^{\rm 16}$,
atlas_authlist.tex:G.~Herten$^{\rm 48}$,
atlas_authlist.tex:R.~Hertenberger$^{\rm 100}$,
atlas_authlist.tex:L.~Hervas$^{\rm 30}$,
atlas_authlist.tex:G.G.~Hesketh$^{\rm 78}$,
atlas_authlist.tex:N.P.~Hessey$^{\rm 107}$,
atlas_authlist.tex:J.W.~Hetherly$^{\rm 40}$,
atlas_authlist.tex:R.~Hickling$^{\rm 76}$,
atlas_authlist.tex:E.~Hig\'on-Rodriguez$^{\rm 167}$,
atlas_authlist.tex:E.~Hill$^{\rm 169}$,
atlas_authlist.tex:J.C.~Hill$^{\rm 28}$,
atlas_authlist.tex:K.H.~Hiller$^{\rm 42}$,
atlas_authlist.tex:S.J.~Hillier$^{\rm 18}$,
atlas_authlist.tex:I.~Hinchliffe$^{\rm 15}$,
atlas_authlist.tex:E.~Hines$^{\rm 122}$,
atlas_authlist.tex:R.R.~Hinman$^{\rm 15}$,
atlas_authlist.tex:M.~Hirose$^{\rm 157}$,
atlas_authlist.tex:D.~Hirschbuehl$^{\rm 175}$,
atlas_authlist.tex:J.~Hobbs$^{\rm 148}$,
atlas_authlist.tex:N.~Hod$^{\rm 107}$,
atlas_authlist.tex:M.C.~Hodgkinson$^{\rm 139}$,
atlas_authlist.tex:P.~Hodgson$^{\rm 139}$,
atlas_authlist.tex:A.~Hoecker$^{\rm 30}$,
atlas_authlist.tex:M.R.~Hoeferkamp$^{\rm 105}$,
atlas_authlist.tex:F.~Hoenig$^{\rm 100}$,
atlas_authlist.tex:M.~Hohlfeld$^{\rm 83}$,
atlas_authlist.tex:D.~Hohn$^{\rm 21}$,
atlas_authlist.tex:T.R.~Holmes$^{\rm 15}$,
atlas_authlist.tex:M.~Homann$^{\rm 43}$,
atlas_authlist.tex:T.M.~Hong$^{\rm 125}$,
atlas_authlist.tex:L.~Hooft~van~Huysduynen$^{\rm 110}$,
atlas_authlist.tex:W.H.~Hopkins$^{\rm 116}$,
atlas_authlist.tex:Y.~Horii$^{\rm 103}$,
atlas_authlist.tex:A.J.~Horton$^{\rm 142}$,
atlas_authlist.tex:J-Y.~Hostachy$^{\rm 55}$,
atlas_authlist.tex:S.~Hou$^{\rm 151}$,
atlas_authlist.tex:A.~Hoummada$^{\rm 135a}$,
atlas_authlist.tex:J.~Howard$^{\rm 120}$,
atlas_authlist.tex:J.~Howarth$^{\rm 42}$,
atlas_authlist.tex:M.~Hrabovsky$^{\rm 115}$,
atlas_authlist.tex:I.~Hristova$^{\rm 16}$,
atlas_authlist.tex:J.~Hrivnac$^{\rm 117}$,
atlas_authlist.tex:T.~Hryn'ova$^{\rm 5}$,
atlas_authlist.tex:A.~Hrynevich$^{\rm 93}$,
atlas_authlist.tex:C.~Hsu$^{\rm 145c}$,
atlas_authlist.tex:P.J.~Hsu$^{\rm 151}$$^{,q}$,
atlas_authlist.tex:S.-C.~Hsu$^{\rm 138}$,
atlas_authlist.tex:D.~Hu$^{\rm 35}$,
atlas_authlist.tex:Q.~Hu$^{\rm 33b}$,
atlas_authlist.tex:X.~Hu$^{\rm 89}$,
atlas_authlist.tex:Y.~Huang$^{\rm 42}$,
atlas_authlist.tex:Z.~Hubacek$^{\rm 128}$,
atlas_authlist.tex:F.~Hubaut$^{\rm 85}$,
atlas_authlist.tex:F.~Huegging$^{\rm 21}$,
atlas_authlist.tex:T.B.~Huffman$^{\rm 120}$,
atlas_authlist.tex:E.W.~Hughes$^{\rm 35}$,
atlas_authlist.tex:G.~Hughes$^{\rm 72}$,
atlas_authlist.tex:M.~Huhtinen$^{\rm 30}$,
atlas_authlist.tex:T.A.~H\"ulsing$^{\rm 83}$,
atlas_authlist.tex:N.~Huseynov$^{\rm 65}$$^{,b}$,
atlas_authlist.tex:J.~Huston$^{\rm 90}$,
atlas_authlist.tex:J.~Huth$^{\rm 57}$,
atlas_authlist.tex:G.~Iacobucci$^{\rm 49}$,
atlas_authlist.tex:G.~Iakovidis$^{\rm 25}$,
atlas_authlist.tex:I.~Ibragimov$^{\rm 141}$,
atlas_authlist.tex:L.~Iconomidou-Fayard$^{\rm 117}$,
atlas_authlist.tex:E.~Ideal$^{\rm 176}$,
atlas_authlist.tex:Z.~Idrissi$^{\rm 135e}$,
atlas_authlist.tex:P.~Iengo$^{\rm 30}$,
atlas_authlist.tex:O.~Igonkina$^{\rm 107}$,
atlas_authlist.tex:T.~Iizawa$^{\rm 171}$,
atlas_authlist.tex:Y.~Ikegami$^{\rm 66}$,
atlas_authlist.tex:K.~Ikematsu$^{\rm 141}$,
atlas_authlist.tex:M.~Ikeno$^{\rm 66}$,
atlas_authlist.tex:Y.~Ilchenko$^{\rm 31}$$^{,r}$,
atlas_authlist.tex:D.~Iliadis$^{\rm 154}$,
atlas_authlist.tex:N.~Ilic$^{\rm 143}$,
atlas_authlist.tex:T.~Ince$^{\rm 101}$,
atlas_authlist.tex:G.~Introzzi$^{\rm 121a,121b}$,
atlas_authlist.tex:P.~Ioannou$^{\rm 9}$,
atlas_authlist.tex:M.~Iodice$^{\rm 134a}$,
atlas_authlist.tex:K.~Iordanidou$^{\rm 35}$,
atlas_authlist.tex:V.~Ippolito$^{\rm 57}$,
atlas_authlist.tex:A.~Irles~Quiles$^{\rm 167}$,
atlas_authlist.tex:C.~Isaksson$^{\rm 166}$,
atlas_authlist.tex:M.~Ishino$^{\rm 68}$,
atlas_authlist.tex:M.~Ishitsuka$^{\rm 157}$,
atlas_authlist.tex:R.~Ishmukhametov$^{\rm 111}$,
atlas_authlist.tex:C.~Issever$^{\rm 120}$,
atlas_authlist.tex:S.~Istin$^{\rm 19a}$,
atlas_authlist.tex:J.M.~Iturbe~Ponce$^{\rm 84}$,
atlas_authlist.tex:R.~Iuppa$^{\rm 133a,133b}$,
atlas_authlist.tex:J.~Ivarsson$^{\rm 81}$,
atlas_authlist.tex:W.~Iwanski$^{\rm 39}$,
atlas_authlist.tex:H.~Iwasaki$^{\rm 66}$,
atlas_authlist.tex:J.M.~Izen$^{\rm 41}$,
atlas_authlist.tex:V.~Izzo$^{\rm 104a}$,
atlas_authlist.tex:S.~Jabbar$^{\rm 3}$,
atlas_authlist.tex:B.~Jackson$^{\rm 122}$,
atlas_authlist.tex:M.~Jackson$^{\rm 74}$,
atlas_authlist.tex:P.~Jackson$^{\rm 1}$,
atlas_authlist.tex:M.R.~Jaekel$^{\rm 30}$,
atlas_authlist.tex:V.~Jain$^{\rm 2}$,
atlas_authlist.tex:K.~Jakobs$^{\rm 48}$,
atlas_authlist.tex:S.~Jakobsen$^{\rm 30}$,
atlas_authlist.tex:T.~Jakoubek$^{\rm 127}$,
atlas_authlist.tex:J.~Jakubek$^{\rm 128}$,
atlas_authlist.tex:D.O.~Jamin$^{\rm 114}$,
atlas_authlist.tex:D.K.~Jana$^{\rm 79}$,
atlas_authlist.tex:E.~Jansen$^{\rm 78}$,
atlas_authlist.tex:R.~Jansky$^{\rm 62}$,
atlas_authlist.tex:J.~Janssen$^{\rm 21}$,
atlas_authlist.tex:M.~Janus$^{\rm 170}$,
atlas_authlist.tex:G.~Jarlskog$^{\rm 81}$,
atlas_authlist.tex:N.~Javadov$^{\rm 65}$$^{,b}$,
atlas_authlist.tex:T.~Jav\r{u}rek$^{\rm 48}$,
atlas_authlist.tex:L.~Jeanty$^{\rm 15}$,
atlas_authlist.tex:J.~Jejelava$^{\rm 51a}$$^{,s}$,
atlas_authlist.tex:G.-Y.~Jeng$^{\rm 150}$,
atlas_authlist.tex:D.~Jennens$^{\rm 88}$,
atlas_authlist.tex:P.~Jenni$^{\rm 48}$$^{,t}$,
atlas_authlist.tex:J.~Jentzsch$^{\rm 43}$,
atlas_authlist.tex:C.~Jeske$^{\rm 170}$,
atlas_authlist.tex:S.~J\'ez\'equel$^{\rm 5}$,
atlas_authlist.tex:H.~Ji$^{\rm 173}$,
atlas_authlist.tex:J.~Jia$^{\rm 148}$,
atlas_authlist.tex:Y.~Jiang$^{\rm 33b}$,
atlas_authlist.tex:S.~Jiggins$^{\rm 78}$,
atlas_authlist.tex:J.~Jimenez~Pena$^{\rm 167}$,
atlas_authlist.tex:S.~Jin$^{\rm 33a}$,
atlas_authlist.tex:A.~Jinaru$^{\rm 26a}$,
atlas_authlist.tex:O.~Jinnouchi$^{\rm 157}$,
atlas_authlist.tex:M.D.~Joergensen$^{\rm 36}$,
atlas_authlist.tex:P.~Johansson$^{\rm 139}$,
atlas_authlist.tex:K.A.~Johns$^{\rm 7}$,
atlas_authlist.tex:K.~Jon-And$^{\rm 146a,146b}$,
atlas_authlist.tex:G.~Jones$^{\rm 170}$,
atlas_authlist.tex:R.W.L.~Jones$^{\rm 72}$,
atlas_authlist.tex:T.J.~Jones$^{\rm 74}$,
atlas_authlist.tex:J.~Jongmanns$^{\rm 58a}$,
atlas_authlist.tex:P.M.~Jorge$^{\rm 126a,126b}$,
atlas_authlist.tex:K.D.~Joshi$^{\rm 84}$,
atlas_authlist.tex:J.~Jovicevic$^{\rm 159a}$,
atlas_authlist.tex:X.~Ju$^{\rm 173}$,
atlas_authlist.tex:C.A.~Jung$^{\rm 43}$,
atlas_authlist.tex:P.~Jussel$^{\rm 62}$,
atlas_authlist.tex:A.~Juste~Rozas$^{\rm 12}$$^{,o}$,
atlas_authlist.tex:M.~Kaci$^{\rm 167}$,
atlas_authlist.tex:A.~Kaczmarska$^{\rm 39}$,
atlas_authlist.tex:M.~Kado$^{\rm 117}$,
atlas_authlist.tex:H.~Kagan$^{\rm 111}$,
atlas_authlist.tex:M.~Kagan$^{\rm 143}$,
atlas_authlist.tex:S.J.~Kahn$^{\rm 85}$,
atlas_authlist.tex:E.~Kajomovitz$^{\rm 45}$,
atlas_authlist.tex:C.W.~Kalderon$^{\rm 120}$,
atlas_authlist.tex:S.~Kama$^{\rm 40}$,
atlas_authlist.tex:A.~Kamenshchikov$^{\rm 130}$,
atlas_authlist.tex:N.~Kanaya$^{\rm 155}$,
atlas_authlist.tex:S.~Kaneti$^{\rm 28}$,
atlas_authlist.tex:V.A.~Kantserov$^{\rm 98}$,
atlas_authlist.tex:J.~Kanzaki$^{\rm 66}$,
atlas_authlist.tex:B.~Kaplan$^{\rm 110}$,
atlas_authlist.tex:L.S.~Kaplan$^{\rm 173}$,
atlas_authlist.tex:A.~Kapliy$^{\rm 31}$,
atlas_authlist.tex:D.~Kar$^{\rm 53}$,
atlas_authlist.tex:K.~Karakostas$^{\rm 10}$,
atlas_authlist.tex:A.~Karamaoun$^{\rm 3}$,
atlas_authlist.tex:N.~Karastathis$^{\rm 10,107}$,
atlas_authlist.tex:M.J.~Kareem$^{\rm 54}$,
atlas_authlist.tex:E.~Karentzos$^{\rm 10}$,
atlas_authlist.tex:M.~Karnevskiy$^{\rm 83}$,
atlas_authlist.tex:S.N.~Karpov$^{\rm 65}$,
atlas_authlist.tex:Z.M.~Karpova$^{\rm 65}$,
atlas_authlist.tex:K.~Karthik$^{\rm 110}$,
atlas_authlist.tex:V.~Kartvelishvili$^{\rm 72}$,
atlas_authlist.tex:A.N.~Karyukhin$^{\rm 130}$,
atlas_authlist.tex:L.~Kashif$^{\rm 173}$,
atlas_authlist.tex:R.D.~Kass$^{\rm 111}$,
atlas_authlist.tex:A.~Kastanas$^{\rm 14}$,
atlas_authlist.tex:Y.~Kataoka$^{\rm 155}$,
atlas_authlist.tex:A.~Katre$^{\rm 49}$,
atlas_authlist.tex:J.~Katzy$^{\rm 42}$,
atlas_authlist.tex:K.~Kawagoe$^{\rm 70}$,
atlas_authlist.tex:T.~Kawamoto$^{\rm 155}$,
atlas_authlist.tex:G.~Kawamura$^{\rm 54}$,
atlas_authlist.tex:S.~Kazama$^{\rm 155}$,
atlas_authlist.tex:V.F.~Kazanin$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:R.~Keeler$^{\rm 169}$,
atlas_authlist.tex:R.~Kehoe$^{\rm 40}$,
atlas_authlist.tex:J.S.~Keller$^{\rm 42}$,
atlas_authlist.tex:J.J.~Kempster$^{\rm 77}$,
atlas_authlist.tex:H.~Keoshkerian$^{\rm 84}$,
atlas_authlist.tex:O.~Kepka$^{\rm 127}$,
atlas_authlist.tex:B.P.~Ker\v{s}evan$^{\rm 75}$,
atlas_authlist.tex:S.~Kersten$^{\rm 175}$,
atlas_authlist.tex:R.A.~Keyes$^{\rm 87}$,
atlas_authlist.tex:F.~Khalil-zada$^{\rm 11}$,
atlas_authlist.tex:H.~Khandanyan$^{\rm 146a,146b}$,
atlas_authlist.tex:A.~Khanov$^{\rm 114}$,
atlas_authlist.tex:A.G.~Kharlamov$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:T.J.~Khoo$^{\rm 28}$,
atlas_authlist.tex:V.~Khovanskiy$^{\rm 97}$,
atlas_authlist.tex:E.~Khramov$^{\rm 65}$,
atlas_authlist.tex:J.~Khubua$^{\rm 51b}$$^{,u}$,
atlas_authlist.tex:H.Y.~Kim$^{\rm 8}$,
atlas_authlist.tex:H.~Kim$^{\rm 146a,146b}$,
atlas_authlist.tex:S.H.~Kim$^{\rm 160}$,
atlas_authlist.tex:Y.~Kim$^{\rm 31}$,
atlas_authlist.tex:N.~Kimura$^{\rm 154}$,
atlas_authlist.tex:O.M.~Kind$^{\rm 16}$,
atlas_authlist.tex:B.T.~King$^{\rm 74}$,
atlas_authlist.tex:M.~King$^{\rm 167}$,
atlas_authlist.tex:S.B.~King$^{\rm 168}$,
atlas_authlist.tex:J.~Kirk$^{\rm 131}$,
atlas_authlist.tex:A.E.~Kiryunin$^{\rm 101}$,
atlas_authlist.tex:T.~Kishimoto$^{\rm 67}$,
atlas_authlist.tex:D.~Kisielewska$^{\rm 38a}$,
atlas_authlist.tex:F.~Kiss$^{\rm 48}$,
atlas_authlist.tex:K.~Kiuchi$^{\rm 160}$,
atlas_authlist.tex:O.~Kivernyk$^{\rm 136}$,
atlas_authlist.tex:E.~Kladiva$^{\rm 144b}$,
atlas_authlist.tex:M.H.~Klein$^{\rm 35}$,
atlas_authlist.tex:M.~Klein$^{\rm 74}$,
atlas_authlist.tex:U.~Klein$^{\rm 74}$,
atlas_authlist.tex:K.~Kleinknecht$^{\rm 83}$,
atlas_authlist.tex:P.~Klimek$^{\rm 146a,146b}$,
atlas_authlist.tex:A.~Klimentov$^{\rm 25}$,
atlas_authlist.tex:R.~Klingenberg$^{\rm 43}$,
atlas_authlist.tex:J.A.~Klinger$^{\rm 139}$,
atlas_authlist.tex:T.~Klioutchnikova$^{\rm 30}$,
atlas_authlist.tex:E.-E.~Kluge$^{\rm 58a}$,
atlas_authlist.tex:P.~Kluit$^{\rm 107}$,
atlas_authlist.tex:S.~Kluth$^{\rm 101}$,
atlas_authlist.tex:J.~Knapik$^{\rm 39}$,
atlas_authlist.tex:E.~Kneringer$^{\rm 62}$,
atlas_authlist.tex:E.B.F.G.~Knoops$^{\rm 85}$,
atlas_authlist.tex:A.~Knue$^{\rm 53}$,
atlas_authlist.tex:A.~Kobayashi$^{\rm 155}$,
atlas_authlist.tex:D.~Kobayashi$^{\rm 157}$,
atlas_authlist.tex:T.~Kobayashi$^{\rm 155}$,
atlas_authlist.tex:M.~Kobel$^{\rm 44}$,
atlas_authlist.tex:M.~Kocian$^{\rm 143}$,
atlas_authlist.tex:P.~Kodys$^{\rm 129}$,
atlas_authlist.tex:T.~Koffas$^{\rm 29}$,
atlas_authlist.tex:E.~Koffeman$^{\rm 107}$,
atlas_authlist.tex:L.A.~Kogan$^{\rm 120}$,
atlas_authlist.tex:S.~Kohlmann$^{\rm 175}$,
atlas_authlist.tex:Z.~Kohout$^{\rm 128}$,
atlas_authlist.tex:T.~Kohriki$^{\rm 66}$,
atlas_authlist.tex:T.~Koi$^{\rm 143}$,
atlas_authlist.tex:H.~Kolanoski$^{\rm 16}$,
atlas_authlist.tex:I.~Koletsou$^{\rm 5}$,
atlas_authlist.tex:A.A.~Komar$^{\rm 96}$$^{,*}$,
atlas_authlist.tex:Y.~Komori$^{\rm 155}$,
atlas_authlist.tex:T.~Kondo$^{\rm 66}$,
atlas_authlist.tex:N.~Kondrashova$^{\rm 42}$,
atlas_authlist.tex:K.~K\"oneke$^{\rm 48}$,
atlas_authlist.tex:A.C.~K\"onig$^{\rm 106}$,
atlas_authlist.tex:T.~Kono$^{\rm 66}$,
atlas_authlist.tex:R.~Konoplich$^{\rm 110}$$^{,v}$,
atlas_authlist.tex:N.~Konstantinidis$^{\rm 78}$,
atlas_authlist.tex:R.~Kopeliansky$^{\rm 152}$,
atlas_authlist.tex:S.~Koperny$^{\rm 38a}$,
atlas_authlist.tex:L.~K\"opke$^{\rm 83}$,
atlas_authlist.tex:A.K.~Kopp$^{\rm 48}$,
atlas_authlist.tex:K.~Korcyl$^{\rm 39}$,
atlas_authlist.tex:K.~Kordas$^{\rm 154}$,
atlas_authlist.tex:A.~Korn$^{\rm 78}$,
atlas_authlist.tex:A.A.~Korol$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:I.~Korolkov$^{\rm 12}$,
atlas_authlist.tex:E.V.~Korolkova$^{\rm 139}$,
atlas_authlist.tex:O.~Kortner$^{\rm 101}$,
atlas_authlist.tex:S.~Kortner$^{\rm 101}$,
atlas_authlist.tex:T.~Kosek$^{\rm 129}$,
atlas_authlist.tex:V.V.~Kostyukhin$^{\rm 21}$,
atlas_authlist.tex:V.M.~Kotov$^{\rm 65}$,
atlas_authlist.tex:A.~Kotwal$^{\rm 45}$,
atlas_authlist.tex:A.~Kourkoumeli-Charalampidi$^{\rm 154}$,
atlas_authlist.tex:C.~Kourkoumelis$^{\rm 9}$,
atlas_authlist.tex:V.~Kouskoura$^{\rm 25}$,
atlas_authlist.tex:A.~Koutsman$^{\rm 159a}$,
atlas_authlist.tex:R.~Kowalewski$^{\rm 169}$,
atlas_authlist.tex:T.Z.~Kowalski$^{\rm 38a}$,
atlas_authlist.tex:W.~Kozanecki$^{\rm 136}$,
atlas_authlist.tex:A.S.~Kozhin$^{\rm 130}$,
atlas_authlist.tex:V.A.~Kramarenko$^{\rm 99}$,
atlas_authlist.tex:G.~Kramberger$^{\rm 75}$,
atlas_authlist.tex:D.~Krasnopevtsev$^{\rm 98}$,
atlas_authlist.tex:M.W.~Krasny$^{\rm 80}$,
atlas_authlist.tex:A.~Krasznahorkay$^{\rm 30}$,
atlas_authlist.tex:J.K.~Kraus$^{\rm 21}$,
atlas_authlist.tex:A.~Kravchenko$^{\rm 25}$,
atlas_authlist.tex:S.~Kreiss$^{\rm 110}$,
atlas_authlist.tex:M.~Kretz$^{\rm 58c}$,
atlas_authlist.tex:J.~Kretzschmar$^{\rm 74}$,
atlas_authlist.tex:K.~Kreutzfeldt$^{\rm 52}$,
atlas_authlist.tex:P.~Krieger$^{\rm 158}$,
atlas_authlist.tex:K.~Krizka$^{\rm 31}$,
atlas_authlist.tex:K.~Kroeninger$^{\rm 43}$,
atlas_authlist.tex:H.~Kroha$^{\rm 101}$,
atlas_authlist.tex:J.~Kroll$^{\rm 122}$,
atlas_authlist.tex:J.~Kroseberg$^{\rm 21}$,
atlas_authlist.tex:J.~Krstic$^{\rm 13}$,
atlas_authlist.tex:U.~Kruchonak$^{\rm 65}$,
atlas_authlist.tex:H.~Kr\"uger$^{\rm 21}$,
atlas_authlist.tex:N.~Krumnack$^{\rm 64}$,
atlas_authlist.tex:A.~Kruse$^{\rm 173}$,
atlas_authlist.tex:M.C.~Kruse$^{\rm 45}$,
atlas_authlist.tex:M.~Kruskal$^{\rm 22}$,
atlas_authlist.tex:T.~Kubota$^{\rm 88}$,
atlas_authlist.tex:H.~Kucuk$^{\rm 78}$,
atlas_authlist.tex:S.~Kuday$^{\rm 4b}$,
atlas_authlist.tex:S.~Kuehn$^{\rm 48}$,
atlas_authlist.tex:A.~Kugel$^{\rm 58c}$,
atlas_authlist.tex:F.~Kuger$^{\rm 174}$,
atlas_authlist.tex:A.~Kuhl$^{\rm 137}$,
atlas_authlist.tex:T.~Kuhl$^{\rm 42}$,
atlas_authlist.tex:V.~Kukhtin$^{\rm 65}$,
atlas_authlist.tex:Y.~Kulchitsky$^{\rm 92}$,
atlas_authlist.tex:S.~Kuleshov$^{\rm 32b}$,
atlas_authlist.tex:M.~Kuna$^{\rm 132a,132b}$,
atlas_authlist.tex:T.~Kunigo$^{\rm 68}$,
atlas_authlist.tex:A.~Kupco$^{\rm 127}$,
atlas_authlist.tex:H.~Kurashige$^{\rm 67}$,
atlas_authlist.tex:Y.A.~Kurochkin$^{\rm 92}$,
atlas_authlist.tex:V.~Kus$^{\rm 127}$,
atlas_authlist.tex:E.S.~Kuwertz$^{\rm 169}$,
atlas_authlist.tex:M.~Kuze$^{\rm 157}$,
atlas_authlist.tex:J.~Kvita$^{\rm 115}$,
atlas_authlist.tex:T.~Kwan$^{\rm 169}$,
atlas_authlist.tex:D.~Kyriazopoulos$^{\rm 139}$,
atlas_authlist.tex:A.~La~Rosa$^{\rm 137}$,
atlas_authlist.tex:J.L.~La~Rosa~Navarro$^{\rm 24d}$,
atlas_authlist.tex:L.~La~Rotonda$^{\rm 37a,37b}$,
atlas_authlist.tex:C.~Lacasta$^{\rm 167}$,
atlas_authlist.tex:F.~Lacava$^{\rm 132a,132b}$,
atlas_authlist.tex:J.~Lacey$^{\rm 29}$,
atlas_authlist.tex:H.~Lacker$^{\rm 16}$,
atlas_authlist.tex:D.~Lacour$^{\rm 80}$,
atlas_authlist.tex:V.R.~Lacuesta$^{\rm 167}$,
atlas_authlist.tex:E.~Ladygin$^{\rm 65}$,
atlas_authlist.tex:R.~Lafaye$^{\rm 5}$,
atlas_authlist.tex:B.~Laforge$^{\rm 80}$,
atlas_authlist.tex:T.~Lagouri$^{\rm 176}$,
atlas_authlist.tex:S.~Lai$^{\rm 54}$,
atlas_authlist.tex:L.~Lambourne$^{\rm 78}$,
atlas_authlist.tex:S.~Lammers$^{\rm 61}$,
atlas_authlist.tex:C.L.~Lampen$^{\rm 7}$,
atlas_authlist.tex:W.~Lampl$^{\rm 7}$,
atlas_authlist.tex:E.~Lan\c{c}on$^{\rm 136}$,
atlas_authlist.tex:U.~Landgraf$^{\rm 48}$,
atlas_authlist.tex:M.P.J.~Landon$^{\rm 76}$,
atlas_authlist.tex:V.S.~Lang$^{\rm 58a}$,
atlas_authlist.tex:J.C.~Lange$^{\rm 12}$,
atlas_authlist.tex:A.J.~Lankford$^{\rm 163}$,
atlas_authlist.tex:F.~Lanni$^{\rm 25}$,
atlas_authlist.tex:K.~Lantzsch$^{\rm 30}$,
atlas_authlist.tex:A.~Lanza$^{\rm 121a}$,
atlas_authlist.tex:S.~Laplace$^{\rm 80}$,
atlas_authlist.tex:C.~Lapoire$^{\rm 30}$,
atlas_authlist.tex:J.F.~Laporte$^{\rm 136}$,
atlas_authlist.tex:T.~Lari$^{\rm 91a}$,
atlas_authlist.tex:F.~Lasagni~Manghi$^{\rm 20a,20b}$,
atlas_authlist.tex:M.~Lassnig$^{\rm 30}$,
atlas_authlist.tex:P.~Laurelli$^{\rm 47}$,
atlas_authlist.tex:W.~Lavrijsen$^{\rm 15}$,
atlas_authlist.tex:A.T.~Law$^{\rm 137}$,
atlas_authlist.tex:P.~Laycock$^{\rm 74}$,
atlas_authlist.tex:T.~Lazovich$^{\rm 57}$,
atlas_authlist.tex:O.~Le~Dortz$^{\rm 80}$,
atlas_authlist.tex:E.~Le~Guirriec$^{\rm 85}$,
atlas_authlist.tex:E.~Le~Menedeu$^{\rm 12}$,
atlas_authlist.tex:M.~LeBlanc$^{\rm 169}$,
atlas_authlist.tex:T.~LeCompte$^{\rm 6}$,
atlas_authlist.tex:F.~Ledroit-Guillon$^{\rm 55}$,
atlas_authlist.tex:C.A.~Lee$^{\rm 145b}$,
atlas_authlist.tex:S.C.~Lee$^{\rm 151}$,
atlas_authlist.tex:L.~Lee$^{\rm 1}$,
atlas_authlist.tex:G.~Lefebvre$^{\rm 80}$,
atlas_authlist.tex:M.~Lefebvre$^{\rm 169}$,
atlas_authlist.tex:F.~Legger$^{\rm 100}$,
atlas_authlist.tex:C.~Leggett$^{\rm 15}$,
atlas_authlist.tex:A.~Lehan$^{\rm 74}$,
atlas_authlist.tex:G.~Lehmann~Miotto$^{\rm 30}$,
atlas_authlist.tex:X.~Lei$^{\rm 7}$,
atlas_authlist.tex:W.A.~Leight$^{\rm 29}$,
atlas_authlist.tex:A.~Leisos$^{\rm 154}$$^{,w}$,
atlas_authlist.tex:A.G.~Leister$^{\rm 176}$,
atlas_authlist.tex:M.A.L.~Leite$^{\rm 24d}$,
atlas_authlist.tex:R.~Leitner$^{\rm 129}$,
atlas_authlist.tex:D.~Lellouch$^{\rm 172}$,
atlas_authlist.tex:B.~Lemmer$^{\rm 54}$,
atlas_authlist.tex:K.J.C.~Leney$^{\rm 78}$,
atlas_authlist.tex:T.~Lenz$^{\rm 21}$,
atlas_authlist.tex:B.~Lenzi$^{\rm 30}$,
atlas_authlist.tex:R.~Leone$^{\rm 7}$,
atlas_authlist.tex:S.~Leone$^{\rm 124a,124b}$,
atlas_authlist.tex:C.~Leonidopoulos$^{\rm 46}$,
atlas_authlist.tex:S.~Leontsinis$^{\rm 10}$,
atlas_authlist.tex:G.~Lerner$^{\rm 149}$,
atlas_authlist.tex:C.~Leroy$^{\rm 95}$,
atlas_authlist.tex:C.G.~Lester$^{\rm 28}$,
atlas_authlist.tex:M.~Levchenko$^{\rm 123}$,
atlas_authlist.tex:J.~Lev\^eque$^{\rm 5}$,
atlas_authlist.tex:D.~Levin$^{\rm 89}$,
atlas_authlist.tex:L.J.~Levinson$^{\rm 172}$,
atlas_authlist.tex:M.~Levy$^{\rm 18}$,
atlas_authlist.tex:A.~Lewis$^{\rm 120}$,
atlas_authlist.tex:A.M.~Leyko$^{\rm 21}$,
atlas_authlist.tex:M.~Leyton$^{\rm 41}$,
atlas_authlist.tex:B.~Li$^{\rm 33b}$$^{,x}$,
atlas_authlist.tex:H.~Li$^{\rm 148}$,
atlas_authlist.tex:H.L.~Li$^{\rm 31}$,
atlas_authlist.tex:L.~Li$^{\rm 45}$,
atlas_authlist.tex:L.~Li$^{\rm 33e}$,
atlas_authlist.tex:S.~Li$^{\rm 45}$,
atlas_authlist.tex:Y.~Li$^{\rm 33c}$$^{,y}$,
atlas_authlist.tex:Z.~Liang$^{\rm 137}$,
atlas_authlist.tex:H.~Liao$^{\rm 34}$,
atlas_authlist.tex:B.~Liberti$^{\rm 133a}$,
atlas_authlist.tex:A.~Liblong$^{\rm 158}$,
atlas_authlist.tex:P.~Lichard$^{\rm 30}$,
atlas_authlist.tex:K.~Lie$^{\rm 165}$,
atlas_authlist.tex:J.~Liebal$^{\rm 21}$,
atlas_authlist.tex:W.~Liebig$^{\rm 14}$,
atlas_authlist.tex:C.~Limbach$^{\rm 21}$,
atlas_authlist.tex:A.~Limosani$^{\rm 150}$,
atlas_authlist.tex:S.C.~Lin$^{\rm 151}$$^{,z}$,
atlas_authlist.tex:T.H.~Lin$^{\rm 83}$,
atlas_authlist.tex:F.~Linde$^{\rm 107}$,
atlas_authlist.tex:B.E.~Lindquist$^{\rm 148}$,
atlas_authlist.tex:J.T.~Linnemann$^{\rm 90}$,
atlas_authlist.tex:E.~Lipeles$^{\rm 122}$,
atlas_authlist.tex:A.~Lipniacka$^{\rm 14}$,
atlas_authlist.tex:M.~Lisovyi$^{\rm 58b}$,
atlas_authlist.tex:T.M.~Liss$^{\rm 165}$,
atlas_authlist.tex:D.~Lissauer$^{\rm 25}$,
atlas_authlist.tex:A.~Lister$^{\rm 168}$,
atlas_authlist.tex:A.M.~Litke$^{\rm 137}$,
atlas_authlist.tex:B.~Liu$^{\rm 151}$$^{,aa}$,
atlas_authlist.tex:D.~Liu$^{\rm 151}$,
atlas_authlist.tex:H.~Liu$^{\rm 89}$,
atlas_authlist.tex:J.~Liu$^{\rm 85}$,
atlas_authlist.tex:J.B.~Liu$^{\rm 33b}$,
atlas_authlist.tex:K.~Liu$^{\rm 85}$,
atlas_authlist.tex:L.~Liu$^{\rm 165}$,
atlas_authlist.tex:M.~Liu$^{\rm 45}$,
atlas_authlist.tex:M.~Liu$^{\rm 33b}$,
atlas_authlist.tex:Y.~Liu$^{\rm 33b}$,
atlas_authlist.tex:M.~Livan$^{\rm 121a,121b}$,
atlas_authlist.tex:A.~Lleres$^{\rm 55}$,
atlas_authlist.tex:J.~Llorente~Merino$^{\rm 82}$,
atlas_authlist.tex:S.L.~Lloyd$^{\rm 76}$,
atlas_authlist.tex:F.~Lo~Sterzo$^{\rm 151}$,
atlas_authlist.tex:E.~Lobodzinska$^{\rm 42}$,
atlas_authlist.tex:P.~Loch$^{\rm 7}$,
atlas_authlist.tex:W.S.~Lockman$^{\rm 137}$,
atlas_authlist.tex:F.K.~Loebinger$^{\rm 84}$,
atlas_authlist.tex:A.E.~Loevschall-Jensen$^{\rm 36}$,
atlas_authlist.tex:A.~Loginov$^{\rm 176}$,
atlas_authlist.tex:T.~Lohse$^{\rm 16}$,
atlas_authlist.tex:K.~Lohwasser$^{\rm 42}$,
atlas_authlist.tex:M.~Lokajicek$^{\rm 127}$,
atlas_authlist.tex:B.A.~Long$^{\rm 22}$,
atlas_authlist.tex:J.D.~Long$^{\rm 89}$,
atlas_authlist.tex:R.E.~Long$^{\rm 72}$,
atlas_authlist.tex:K.A.~Looper$^{\rm 111}$,
atlas_authlist.tex:L.~Lopes$^{\rm 126a}$,
atlas_authlist.tex:D.~Lopez~Mateos$^{\rm 57}$,
atlas_authlist.tex:B.~Lopez~Paredes$^{\rm 139}$,
atlas_authlist.tex:I.~Lopez~Paz$^{\rm 12}$,
atlas_authlist.tex:J.~Lorenz$^{\rm 100}$,
atlas_authlist.tex:N.~Lorenzo~Martinez$^{\rm 61}$,
atlas_authlist.tex:M.~Losada$^{\rm 162}$,
atlas_authlist.tex:P.~Loscutoff$^{\rm 15}$,
atlas_authlist.tex:P.J.~L{\"o}sel$^{\rm 100}$,
atlas_authlist.tex:X.~Lou$^{\rm 33a}$,
atlas_authlist.tex:A.~Lounis$^{\rm 117}$,
atlas_authlist.tex:J.~Love$^{\rm 6}$,
atlas_authlist.tex:P.A.~Love$^{\rm 72}$,
atlas_authlist.tex:N.~Lu$^{\rm 89}$,
atlas_authlist.tex:H.J.~Lubatti$^{\rm 138}$,
atlas_authlist.tex:C.~Luci$^{\rm 132a,132b}$,
atlas_authlist.tex:A.~Lucotte$^{\rm 55}$,
atlas_authlist.tex:F.~Luehring$^{\rm 61}$,
atlas_authlist.tex:W.~Lukas$^{\rm 62}$,
atlas_authlist.tex:L.~Luminari$^{\rm 132a}$,
atlas_authlist.tex:O.~Lundberg$^{\rm 146a,146b}$,
atlas_authlist.tex:B.~Lund-Jensen$^{\rm 147}$,
atlas_authlist.tex:D.~Lynn$^{\rm 25}$,
atlas_authlist.tex:R.~Lysak$^{\rm 127}$,
atlas_authlist.tex:E.~Lytken$^{\rm 81}$,
atlas_authlist.tex:H.~Ma$^{\rm 25}$,
atlas_authlist.tex:L.L.~Ma$^{\rm 33d}$,
atlas_authlist.tex:G.~Maccarrone$^{\rm 47}$,
atlas_authlist.tex:A.~Macchiolo$^{\rm 101}$,
atlas_authlist.tex:C.M.~Macdonald$^{\rm 139}$,
atlas_authlist.tex:J.~Machado~Miguens$^{\rm 122,126b}$,
atlas_authlist.tex:D.~Macina$^{\rm 30}$,
atlas_authlist.tex:D.~Madaffari$^{\rm 85}$,
atlas_authlist.tex:R.~Madar$^{\rm 34}$,
atlas_authlist.tex:H.J.~Maddocks$^{\rm 72}$,
atlas_authlist.tex:W.F.~Mader$^{\rm 44}$,
atlas_authlist.tex:A.~Madsen$^{\rm 166}$,
atlas_authlist.tex:S.~Maeland$^{\rm 14}$,
atlas_authlist.tex:T.~Maeno$^{\rm 25}$,
atlas_authlist.tex:A.~Maevskiy$^{\rm 99}$,
atlas_authlist.tex:E.~Magradze$^{\rm 54}$,
atlas_authlist.tex:K.~Mahboubi$^{\rm 48}$,
atlas_authlist.tex:J.~Mahlstedt$^{\rm 107}$,
atlas_authlist.tex:C.~Maiani$^{\rm 136}$,
atlas_authlist.tex:C.~Maidantchik$^{\rm 24a}$,
atlas_authlist.tex:A.A.~Maier$^{\rm 101}$,
atlas_authlist.tex:T.~Maier$^{\rm 100}$,
atlas_authlist.tex:A.~Maio$^{\rm 126a,126b,126d}$,
atlas_authlist.tex:S.~Majewski$^{\rm 116}$,
atlas_authlist.tex:Y.~Makida$^{\rm 66}$,
atlas_authlist.tex:N.~Makovec$^{\rm 117}$,
atlas_authlist.tex:B.~Malaescu$^{\rm 80}$,
atlas_authlist.tex:Pa.~Malecki$^{\rm 39}$,
atlas_authlist.tex:V.P.~Maleev$^{\rm 123}$,
atlas_authlist.tex:F.~Malek$^{\rm 55}$,
atlas_authlist.tex:U.~Mallik$^{\rm 63}$,
atlas_authlist.tex:D.~Malon$^{\rm 6}$,
atlas_authlist.tex:C.~Malone$^{\rm 143}$,
atlas_authlist.tex:S.~Maltezos$^{\rm 10}$,
atlas_authlist.tex:V.M.~Malyshev$^{\rm 109}$,
atlas_authlist.tex:S.~Malyukov$^{\rm 30}$,
atlas_authlist.tex:J.~Mamuzic$^{\rm 42}$,
atlas_authlist.tex:G.~Mancini$^{\rm 47}$,
atlas_authlist.tex:B.~Mandelli$^{\rm 30}$,
atlas_authlist.tex:L.~Mandelli$^{\rm 91a}$,
atlas_authlist.tex:I.~Mandi\'{c}$^{\rm 75}$,
atlas_authlist.tex:R.~Mandrysch$^{\rm 63}$,
atlas_authlist.tex:J.~Maneira$^{\rm 126a,126b}$,
atlas_authlist.tex:A.~Manfredini$^{\rm 101}$,
atlas_authlist.tex:L.~Manhaes~de~Andrade~Filho$^{\rm 24b}$,
atlas_authlist.tex:J.~Manjarres~Ramos$^{\rm 159b}$,
atlas_authlist.tex:A.~Mann$^{\rm 100}$,
atlas_authlist.tex:P.M.~Manning$^{\rm 137}$,
atlas_authlist.tex:A.~Manousakis-Katsikakis$^{\rm 9}$,
atlas_authlist.tex:B.~Mansoulie$^{\rm 136}$,
atlas_authlist.tex:R.~Mantifel$^{\rm 87}$,
atlas_authlist.tex:M.~Mantoani$^{\rm 54}$,
atlas_authlist.tex:L.~Mapelli$^{\rm 30}$,
atlas_authlist.tex:L.~March$^{\rm 145c}$,
atlas_authlist.tex:G.~Marchiori$^{\rm 80}$,
atlas_authlist.tex:M.~Marcisovsky$^{\rm 127}$,
atlas_authlist.tex:C.P.~Marino$^{\rm 169}$,
atlas_authlist.tex:M.~Marjanovic$^{\rm 13}$,
atlas_authlist.tex:D.E.~Marley$^{\rm 89}$,
atlas_authlist.tex:F.~Marroquim$^{\rm 24a}$,
atlas_authlist.tex:S.P.~Marsden$^{\rm 84}$,
atlas_authlist.tex:Z.~Marshall$^{\rm 15}$,
atlas_authlist.tex:L.F.~Marti$^{\rm 17}$,
atlas_authlist.tex:S.~Marti-Garcia$^{\rm 167}$,
atlas_authlist.tex:B.~Martin$^{\rm 90}$,
atlas_authlist.tex:T.A.~Martin$^{\rm 170}$,
atlas_authlist.tex:V.J.~Martin$^{\rm 46}$,
atlas_authlist.tex:B.~Martin~dit~Latour$^{\rm 14}$,
atlas_authlist.tex:M.~Martinez$^{\rm 12}$$^{,o}$,
atlas_authlist.tex:S.~Martin-Haugh$^{\rm 131}$,
atlas_authlist.tex:V.S.~Martoiu$^{\rm 26a}$,
atlas_authlist.tex:A.C.~Martyniuk$^{\rm 78}$,
atlas_authlist.tex:M.~Marx$^{\rm 138}$,
atlas_authlist.tex:F.~Marzano$^{\rm 132a}$,
atlas_authlist.tex:A.~Marzin$^{\rm 30}$,
atlas_authlist.tex:L.~Masetti$^{\rm 83}$,
atlas_authlist.tex:T.~Mashimo$^{\rm 155}$,
atlas_authlist.tex:R.~Mashinistov$^{\rm 96}$,
atlas_authlist.tex:J.~Masik$^{\rm 84}$,
atlas_authlist.tex:A.L.~Maslennikov$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:I.~Massa$^{\rm 20a,20b}$,
atlas_authlist.tex:L.~Massa$^{\rm 20a,20b}$,
atlas_authlist.tex:N.~Massol$^{\rm 5}$,
atlas_authlist.tex:P.~Mastrandrea$^{\rm 148}$,
atlas_authlist.tex:A.~Mastroberardino$^{\rm 37a,37b}$,
atlas_authlist.tex:T.~Masubuchi$^{\rm 155}$,
atlas_authlist.tex:P.~M\"attig$^{\rm 175}$,
atlas_authlist.tex:J.~Mattmann$^{\rm 83}$,
atlas_authlist.tex:J.~Maurer$^{\rm 26a}$,
atlas_authlist.tex:S.J.~Maxfield$^{\rm 74}$,
atlas_authlist.tex:D.A.~Maximov$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:R.~Mazini$^{\rm 151}$,
atlas_authlist.tex:S.M.~Mazza$^{\rm 91a,91b}$,
atlas_authlist.tex:L.~Mazzaferro$^{\rm 133a,133b}$,
atlas_authlist.tex:G.~Mc~Goldrick$^{\rm 158}$,
atlas_authlist.tex:S.P.~Mc~Kee$^{\rm 89}$,
atlas_authlist.tex:A.~McCarn$^{\rm 89}$,
atlas_authlist.tex:R.L.~McCarthy$^{\rm 148}$,
atlas_authlist.tex:T.G.~McCarthy$^{\rm 29}$,
atlas_authlist.tex:N.A.~McCubbin$^{\rm 131}$,
atlas_authlist.tex:K.W.~McFarlane$^{\rm 56}$$^{,*}$,
atlas_authlist.tex:J.A.~Mcfayden$^{\rm 78}$,
atlas_authlist.tex:G.~Mchedlidze$^{\rm 54}$,
atlas_authlist.tex:S.J.~McMahon$^{\rm 131}$,
atlas_authlist.tex:R.A.~McPherson$^{\rm 169}$$^{,k}$,
atlas_authlist.tex:M.~Medinnis$^{\rm 42}$,
atlas_authlist.tex:S.~Meehan$^{\rm 145a}$,
atlas_authlist.tex:S.~Mehlhase$^{\rm 100}$,
atlas_authlist.tex:A.~Mehta$^{\rm 74}$,
atlas_authlist.tex:K.~Meier$^{\rm 58a}$,
atlas_authlist.tex:C.~Meineck$^{\rm 100}$,
atlas_authlist.tex:B.~Meirose$^{\rm 41}$,
atlas_authlist.tex:B.R.~Mellado~Garcia$^{\rm 145c}$,
atlas_authlist.tex:F.~Meloni$^{\rm 17}$,
atlas_authlist.tex:A.~Mengarelli$^{\rm 20a,20b}$,
atlas_authlist.tex:S.~Menke$^{\rm 101}$,
atlas_authlist.tex:E.~Meoni$^{\rm 161}$,
atlas_authlist.tex:K.M.~Mercurio$^{\rm 57}$,
atlas_authlist.tex:S.~Mergelmeyer$^{\rm 21}$,
atlas_authlist.tex:P.~Mermod$^{\rm 49}$,
atlas_authlist.tex:L.~Merola$^{\rm 104a,104b}$,
atlas_authlist.tex:C.~Meroni$^{\rm 91a}$,
atlas_authlist.tex:F.S.~Merritt$^{\rm 31}$,
atlas_authlist.tex:A.~Messina$^{\rm 132a,132b}$,
atlas_authlist.tex:J.~Metcalfe$^{\rm 25}$,
atlas_authlist.tex:A.S.~Mete$^{\rm 163}$,
atlas_authlist.tex:C.~Meyer$^{\rm 83}$,
atlas_authlist.tex:C.~Meyer$^{\rm 122}$,
atlas_authlist.tex:J-P.~Meyer$^{\rm 136}$,
atlas_authlist.tex:J.~Meyer$^{\rm 107}$,
atlas_authlist.tex:R.P.~Middleton$^{\rm 131}$,
atlas_authlist.tex:S.~Miglioranzi$^{\rm 164a,164c}$,
atlas_authlist.tex:L.~Mijovi\'{c}$^{\rm 21}$,
atlas_authlist.tex:G.~Mikenberg$^{\rm 172}$,
atlas_authlist.tex:M.~Mikestikova$^{\rm 127}$,
atlas_authlist.tex:M.~Miku\v{z}$^{\rm 75}$,
atlas_authlist.tex:M.~Milesi$^{\rm 88}$,
atlas_authlist.tex:A.~Milic$^{\rm 30}$,
atlas_authlist.tex:D.W.~Miller$^{\rm 31}$,
atlas_authlist.tex:C.~Mills$^{\rm 46}$,
atlas_authlist.tex:A.~Milov$^{\rm 172}$,
atlas_authlist.tex:D.A.~Milstead$^{\rm 146a,146b}$,
atlas_authlist.tex:A.A.~Minaenko$^{\rm 130}$,
atlas_authlist.tex:Y.~Minami$^{\rm 155}$,
atlas_authlist.tex:I.A.~Minashvili$^{\rm 65}$,
atlas_authlist.tex:A.I.~Mincer$^{\rm 110}$,
atlas_authlist.tex:B.~Mindur$^{\rm 38a}$,
atlas_authlist.tex:M.~Mineev$^{\rm 65}$,
atlas_authlist.tex:Y.~Ming$^{\rm 173}$,
atlas_authlist.tex:L.M.~Mir$^{\rm 12}$,
atlas_authlist.tex:T.~Mitani$^{\rm 171}$,
atlas_authlist.tex:J.~Mitrevski$^{\rm 100}$,
atlas_authlist.tex:V.A.~Mitsou$^{\rm 167}$,
atlas_authlist.tex:A.~Miucci$^{\rm 49}$,
atlas_authlist.tex:P.S.~Miyagawa$^{\rm 139}$,
atlas_authlist.tex:J.U.~Mj\"ornmark$^{\rm 81}$,
atlas_authlist.tex:T.~Moa$^{\rm 146a,146b}$,
atlas_authlist.tex:K.~Mochizuki$^{\rm 85}$,
atlas_authlist.tex:S.~Mohapatra$^{\rm 35}$,
atlas_authlist.tex:W.~Mohr$^{\rm 48}$,
atlas_authlist.tex:S.~Molander$^{\rm 146a,146b}$,
atlas_authlist.tex:R.~Moles-Valls$^{\rm 21}$,
atlas_authlist.tex:K.~M\"onig$^{\rm 42}$,
atlas_authlist.tex:C.~Monini$^{\rm 55}$,
atlas_authlist.tex:J.~Monk$^{\rm 36}$,
atlas_authlist.tex:E.~Monnier$^{\rm 85}$,
atlas_authlist.tex:J.~Montejo~Berlingen$^{\rm 12}$,
atlas_authlist.tex:F.~Monticelli$^{\rm 71}$,
atlas_authlist.tex:S.~Monzani$^{\rm 132a,132b}$,
atlas_authlist.tex:R.W.~Moore$^{\rm 3}$,
atlas_authlist.tex:N.~Morange$^{\rm 117}$,
atlas_authlist.tex:D.~Moreno$^{\rm 162}$,
atlas_authlist.tex:M.~Moreno~Ll\'acer$^{\rm 54}$,
atlas_authlist.tex:P.~Morettini$^{\rm 50a}$,
atlas_authlist.tex:M.~Morgenstern$^{\rm 44}$,
atlas_authlist.tex:D.~Mori$^{\rm 142}$,
atlas_authlist.tex:M.~Morii$^{\rm 57}$,
atlas_authlist.tex:M.~Morinaga$^{\rm 155}$,
atlas_authlist.tex:V.~Morisbak$^{\rm 119}$,
atlas_authlist.tex:S.~Moritz$^{\rm 83}$,
atlas_authlist.tex:A.K.~Morley$^{\rm 150}$,
atlas_authlist.tex:G.~Mornacchi$^{\rm 30}$,
atlas_authlist.tex:J.D.~Morris$^{\rm 76}$,
atlas_authlist.tex:S.S.~Mortensen$^{\rm 36}$,
atlas_authlist.tex:A.~Morton$^{\rm 53}$,
atlas_authlist.tex:L.~Morvaj$^{\rm 103}$,
atlas_authlist.tex:M.~Mosidze$^{\rm 51b}$,
atlas_authlist.tex:J.~Moss$^{\rm 111}$,
atlas_authlist.tex:K.~Motohashi$^{\rm 157}$,
atlas_authlist.tex:R.~Mount$^{\rm 143}$,
atlas_authlist.tex:E.~Mountricha$^{\rm 25}$,
atlas_authlist.tex:S.V.~Mouraviev$^{\rm 96}$$^{,*}$,
atlas_authlist.tex:E.J.W.~Moyse$^{\rm 86}$,
atlas_authlist.tex:S.~Muanza$^{\rm 85}$,
atlas_authlist.tex:R.D.~Mudd$^{\rm 18}$,
atlas_authlist.tex:F.~Mueller$^{\rm 101}$,
atlas_authlist.tex:J.~Mueller$^{\rm 125}$,
atlas_authlist.tex:R.S.P.~Mueller$^{\rm 100}$,
atlas_authlist.tex:T.~Mueller$^{\rm 28}$,
atlas_authlist.tex:D.~Muenstermann$^{\rm 49}$,
atlas_authlist.tex:P.~Mullen$^{\rm 53}$,
atlas_authlist.tex:G.A.~Mullier$^{\rm 17}$,
atlas_authlist.tex:J.A.~Murillo~Quijada$^{\rm 18}$,
atlas_authlist.tex:W.J.~Murray$^{\rm 170,131}$,
atlas_authlist.tex:H.~Musheghyan$^{\rm 54}$,
atlas_authlist.tex:E.~Musto$^{\rm 152}$,
atlas_authlist.tex:A.G.~Myagkov$^{\rm 130}$$^{,ab}$,
atlas_authlist.tex:M.~Myska$^{\rm 128}$,
atlas_authlist.tex:B.P.~Nachman$^{\rm 143}$,
atlas_authlist.tex:O.~Nackenhorst$^{\rm 54}$,
atlas_authlist.tex:J.~Nadal$^{\rm 54}$,
atlas_authlist.tex:K.~Nagai$^{\rm 120}$,
atlas_authlist.tex:R.~Nagai$^{\rm 157}$,
atlas_authlist.tex:Y.~Nagai$^{\rm 85}$,
atlas_authlist.tex:K.~Nagano$^{\rm 66}$,
atlas_authlist.tex:A.~Nagarkar$^{\rm 111}$,
atlas_authlist.tex:Y.~Nagasaka$^{\rm 59}$,
atlas_authlist.tex:K.~Nagata$^{\rm 160}$,
atlas_authlist.tex:M.~Nagel$^{\rm 101}$,
atlas_authlist.tex:E.~Nagy$^{\rm 85}$,
atlas_authlist.tex:A.M.~Nairz$^{\rm 30}$,
atlas_authlist.tex:Y.~Nakahama$^{\rm 30}$,
atlas_authlist.tex:K.~Nakamura$^{\rm 66}$,
atlas_authlist.tex:T.~Nakamura$^{\rm 155}$,
atlas_authlist.tex:I.~Nakano$^{\rm 112}$,
atlas_authlist.tex:H.~Namasivayam$^{\rm 41}$,
atlas_authlist.tex:R.F.~Naranjo~Garcia$^{\rm 42}$,
atlas_authlist.tex:R.~Narayan$^{\rm 31}$,
atlas_authlist.tex:T.~Naumann$^{\rm 42}$,
atlas_authlist.tex:G.~Navarro$^{\rm 162}$,
atlas_authlist.tex:R.~Nayyar$^{\rm 7}$,
atlas_authlist.tex:H.A.~Neal$^{\rm 89}$,
atlas_authlist.tex:P.Yu.~Nechaeva$^{\rm 96}$,
atlas_authlist.tex:T.J.~Neep$^{\rm 84}$,
atlas_authlist.tex:P.D.~Nef$^{\rm 143}$,
atlas_authlist.tex:A.~Negri$^{\rm 121a,121b}$,
atlas_authlist.tex:M.~Negrini$^{\rm 20a}$,
atlas_authlist.tex:S.~Nektarijevic$^{\rm 106}$,
atlas_authlist.tex:C.~Nellist$^{\rm 117}$,
atlas_authlist.tex:A.~Nelson$^{\rm 163}$,
atlas_authlist.tex:S.~Nemecek$^{\rm 127}$,
atlas_authlist.tex:P.~Nemethy$^{\rm 110}$,
atlas_authlist.tex:A.A.~Nepomuceno$^{\rm 24a}$,
atlas_authlist.tex:M.~Nessi$^{\rm 30}$$^{,ac}$,
atlas_authlist.tex:M.S.~Neubauer$^{\rm 165}$,
atlas_authlist.tex:M.~Neumann$^{\rm 175}$,
atlas_authlist.tex:R.M.~Neves$^{\rm 110}$,
atlas_authlist.tex:P.~Nevski$^{\rm 25}$,
atlas_authlist.tex:P.R.~Newman$^{\rm 18}$,
atlas_authlist.tex:D.H.~Nguyen$^{\rm 6}$,
atlas_authlist.tex:R.B.~Nickerson$^{\rm 120}$,
atlas_authlist.tex:R.~Nicolaidou$^{\rm 136}$,
atlas_authlist.tex:B.~Nicquevert$^{\rm 30}$,
atlas_authlist.tex:J.~Nielsen$^{\rm 137}$,
atlas_authlist.tex:N.~Nikiforou$^{\rm 35}$,
atlas_authlist.tex:A.~Nikiforov$^{\rm 16}$,
atlas_authlist.tex:V.~Nikolaenko$^{\rm 130}$$^{,ab}$,
atlas_authlist.tex:I.~Nikolic-Audit$^{\rm 80}$,
atlas_authlist.tex:K.~Nikolopoulos$^{\rm 18}$,
atlas_authlist.tex:J.K.~Nilsen$^{\rm 119}$,
atlas_authlist.tex:P.~Nilsson$^{\rm 25}$,
atlas_authlist.tex:Y.~Ninomiya$^{\rm 155}$,
atlas_authlist.tex:A.~Nisati$^{\rm 132a}$,
atlas_authlist.tex:R.~Nisius$^{\rm 101}$,
atlas_authlist.tex:T.~Nobe$^{\rm 155}$,
atlas_authlist.tex:M.~Nomachi$^{\rm 118}$,
atlas_authlist.tex:I.~Nomidis$^{\rm 29}$,
atlas_authlist.tex:T.~Nooney$^{\rm 76}$,
atlas_authlist.tex:S.~Norberg$^{\rm 113}$,
atlas_authlist.tex:M.~Nordberg$^{\rm 30}$,
atlas_authlist.tex:O.~Novgorodova$^{\rm 44}$,
atlas_authlist.tex:S.~Nowak$^{\rm 101}$,
atlas_authlist.tex:M.~Nozaki$^{\rm 66}$,
atlas_authlist.tex:L.~Nozka$^{\rm 115}$,
atlas_authlist.tex:K.~Ntekas$^{\rm 10}$,
atlas_authlist.tex:G.~Nunes~Hanninger$^{\rm 88}$,
atlas_authlist.tex:T.~Nunnemann$^{\rm 100}$,
atlas_authlist.tex:E.~Nurse$^{\rm 78}$,
atlas_authlist.tex:F.~Nuti$^{\rm 88}$,
atlas_authlist.tex:B.J.~O'Brien$^{\rm 46}$,
atlas_authlist.tex:F.~O'grady$^{\rm 7}$,
atlas_authlist.tex:D.C.~O'Neil$^{\rm 142}$,
atlas_authlist.tex:V.~O'Shea$^{\rm 53}$,
atlas_authlist.tex:F.G.~Oakham$^{\rm 29}$$^{,d}$,
atlas_authlist.tex:H.~Oberlack$^{\rm 101}$,
atlas_authlist.tex:T.~Obermann$^{\rm 21}$,
atlas_authlist.tex:J.~Ocariz$^{\rm 80}$,
atlas_authlist.tex:A.~Ochi$^{\rm 67}$,
atlas_authlist.tex:I.~Ochoa$^{\rm 78}$,
atlas_authlist.tex:J.P.~Ochoa-Ricoux$^{\rm 32a}$,
atlas_authlist.tex:S.~Oda$^{\rm 70}$,
atlas_authlist.tex:S.~Odaka$^{\rm 66}$,
atlas_authlist.tex:H.~Ogren$^{\rm 61}$,
atlas_authlist.tex:A.~Oh$^{\rm 84}$,
atlas_authlist.tex:S.H.~Oh$^{\rm 45}$,
atlas_authlist.tex:C.C.~Ohm$^{\rm 15}$,
atlas_authlist.tex:H.~Ohman$^{\rm 166}$,
atlas_authlist.tex:H.~Oide$^{\rm 30}$,
atlas_authlist.tex:W.~Okamura$^{\rm 118}$,
atlas_authlist.tex:H.~Okawa$^{\rm 160}$,
atlas_authlist.tex:Y.~Okumura$^{\rm 31}$,
atlas_authlist.tex:T.~Okuyama$^{\rm 66}$,
atlas_authlist.tex:A.~Olariu$^{\rm 26a}$,
atlas_authlist.tex:S.A.~Olivares~Pino$^{\rm 46}$,
atlas_authlist.tex:D.~Oliveira~Damazio$^{\rm 25}$,
atlas_authlist.tex:E.~Oliver~Garcia$^{\rm 167}$,
atlas_authlist.tex:A.~Olszewski$^{\rm 39}$,
atlas_authlist.tex:J.~Olszowska$^{\rm 39}$,
atlas_authlist.tex:A.~Onofre$^{\rm 126a,126e}$,
atlas_authlist.tex:P.U.E.~Onyisi$^{\rm 31}$$^{,r}$,
atlas_authlist.tex:C.J.~Oram$^{\rm 159a}$,
atlas_authlist.tex:M.J.~Oreglia$^{\rm 31}$,
atlas_authlist.tex:Y.~Oren$^{\rm 153}$,
atlas_authlist.tex:D.~Orestano$^{\rm 134a,134b}$,
atlas_authlist.tex:N.~Orlando$^{\rm 154}$,
atlas_authlist.tex:C.~Oropeza~Barrera$^{\rm 53}$,
atlas_authlist.tex:R.S.~Orr$^{\rm 158}$,
atlas_authlist.tex:B.~Osculati$^{\rm 50a,50b}$,
atlas_authlist.tex:R.~Ospanov$^{\rm 84}$,
atlas_authlist.tex:G.~Otero~y~Garzon$^{\rm 27}$,
atlas_authlist.tex:H.~Otono$^{\rm 70}$,
atlas_authlist.tex:M.~Ouchrif$^{\rm 135d}$,
atlas_authlist.tex:E.A.~Ouellette$^{\rm 169}$,
atlas_authlist.tex:F.~Ould-Saada$^{\rm 119}$,
atlas_authlist.tex:A.~Ouraou$^{\rm 136}$,
atlas_authlist.tex:K.P.~Oussoren$^{\rm 107}$,
atlas_authlist.tex:Q.~Ouyang$^{\rm 33a}$,
atlas_authlist.tex:A.~Ovcharova$^{\rm 15}$,
atlas_authlist.tex:M.~Owen$^{\rm 53}$,
atlas_authlist.tex:R.E.~Owen$^{\rm 18}$,
atlas_authlist.tex:V.E.~Ozcan$^{\rm 19a}$,
atlas_authlist.tex:N.~Ozturk$^{\rm 8}$,
atlas_authlist.tex:K.~Pachal$^{\rm 142}$,
atlas_authlist.tex:A.~Pacheco~Pages$^{\rm 12}$,
atlas_authlist.tex:C.~Padilla~Aranda$^{\rm 12}$,
atlas_authlist.tex:M.~Pag\'{a}\v{c}ov\'{a}$^{\rm 48}$,
atlas_authlist.tex:S.~Pagan~Griso$^{\rm 15}$,
atlas_authlist.tex:E.~Paganis$^{\rm 139}$,
atlas_authlist.tex:F.~Paige$^{\rm 25}$,
atlas_authlist.tex:P.~Pais$^{\rm 86}$,
atlas_authlist.tex:K.~Pajchel$^{\rm 119}$,
atlas_authlist.tex:G.~Palacino$^{\rm 159b}$,
atlas_authlist.tex:S.~Palestini$^{\rm 30}$,
atlas_authlist.tex:M.~Palka$^{\rm 38b}$,
atlas_authlist.tex:D.~Pallin$^{\rm 34}$,
atlas_authlist.tex:A.~Palma$^{\rm 126a,126b}$,
atlas_authlist.tex:Y.B.~Pan$^{\rm 173}$,
atlas_authlist.tex:E.~Panagiotopoulou$^{\rm 10}$,
atlas_authlist.tex:C.E.~Pandini$^{\rm 80}$,
atlas_authlist.tex:J.G.~Panduro~Vazquez$^{\rm 77}$,
atlas_authlist.tex:P.~Pani$^{\rm 146a,146b}$,
atlas_authlist.tex:S.~Panitkin$^{\rm 25}$,
atlas_authlist.tex:D.~Pantea$^{\rm 26a}$,
atlas_authlist.tex:L.~Paolozzi$^{\rm 49}$,
atlas_authlist.tex:Th.D.~Papadopoulou$^{\rm 10}$,
atlas_authlist.tex:K.~Papageorgiou$^{\rm 154}$,
atlas_authlist.tex:A.~Paramonov$^{\rm 6}$,
atlas_authlist.tex:D.~Paredes~Hernandez$^{\rm 154}$,
atlas_authlist.tex:M.A.~Parker$^{\rm 28}$,
atlas_authlist.tex:K.A.~Parker$^{\rm 139}$,
atlas_authlist.tex:F.~Parodi$^{\rm 50a,50b}$,
atlas_authlist.tex:J.A.~Parsons$^{\rm 35}$,
atlas_authlist.tex:U.~Parzefall$^{\rm 48}$,
atlas_authlist.tex:E.~Pasqualucci$^{\rm 132a}$,
atlas_authlist.tex:S.~Passaggio$^{\rm 50a}$,
atlas_authlist.tex:F.~Pastore$^{\rm 134a,134b}$$^{,*}$,
atlas_authlist.tex:Fr.~Pastore$^{\rm 77}$,
atlas_authlist.tex:G.~P\'asztor$^{\rm 29}$,
atlas_authlist.tex:S.~Pataraia$^{\rm 175}$,
atlas_authlist.tex:N.D.~Patel$^{\rm 150}$,
atlas_authlist.tex:J.R.~Pater$^{\rm 84}$,
atlas_authlist.tex:T.~Pauly$^{\rm 30}$,
atlas_authlist.tex:J.~Pearce$^{\rm 169}$,
atlas_authlist.tex:B.~Pearson$^{\rm 113}$,
atlas_authlist.tex:L.E.~Pedersen$^{\rm 36}$,
atlas_authlist.tex:M.~Pedersen$^{\rm 119}$,
atlas_authlist.tex:S.~Pedraza~Lopez$^{\rm 167}$,
atlas_authlist.tex:R.~Pedro$^{\rm 126a,126b}$,
atlas_authlist.tex:S.V.~Peleganchuk$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:D.~Pelikan$^{\rm 166}$,
atlas_authlist.tex:O.~Penc$^{\rm 127}$,
atlas_authlist.tex:C.~Peng$^{\rm 33a}$,
atlas_authlist.tex:H.~Peng$^{\rm 33b}$,
atlas_authlist.tex:B.~Penning$^{\rm 31}$,
atlas_authlist.tex:J.~Penwell$^{\rm 61}$,
atlas_authlist.tex:D.V.~Perepelitsa$^{\rm 25}$,
atlas_authlist.tex:E.~Perez~Codina$^{\rm 159a}$,
atlas_authlist.tex:M.T.~P\'erez~Garc\'ia-Esta\~n$^{\rm 167}$,
atlas_authlist.tex:L.~Perini$^{\rm 91a,91b}$,
atlas_authlist.tex:H.~Pernegger$^{\rm 30}$,
atlas_authlist.tex:S.~Perrella$^{\rm 104a,104b}$,
atlas_authlist.tex:R.~Peschke$^{\rm 42}$,
atlas_authlist.tex:V.D.~Peshekhonov$^{\rm 65}$,
atlas_authlist.tex:K.~Peters$^{\rm 30}$,
atlas_authlist.tex:R.F.Y.~Peters$^{\rm 84}$,
atlas_authlist.tex:B.A.~Petersen$^{\rm 30}$,
atlas_authlist.tex:T.C.~Petersen$^{\rm 36}$,
atlas_authlist.tex:E.~Petit$^{\rm 42}$,
atlas_authlist.tex:A.~Petridis$^{\rm 146a,146b}$,
atlas_authlist.tex:C.~Petridou$^{\rm 154}$,
atlas_authlist.tex:P.~Petroff$^{\rm 117}$,
atlas_authlist.tex:E.~Petrolo$^{\rm 132a}$,
atlas_authlist.tex:F.~Petrucci$^{\rm 134a,134b}$,
atlas_authlist.tex:N.E.~Pettersson$^{\rm 157}$,
atlas_authlist.tex:R.~Pezoa$^{\rm 32b}$,
atlas_authlist.tex:P.W.~Phillips$^{\rm 131}$,
atlas_authlist.tex:G.~Piacquadio$^{\rm 143}$,
atlas_authlist.tex:E.~Pianori$^{\rm 170}$,
atlas_authlist.tex:A.~Picazio$^{\rm 49}$,
atlas_authlist.tex:E.~Piccaro$^{\rm 76}$,
atlas_authlist.tex:M.~Piccinini$^{\rm 20a,20b}$,
atlas_authlist.tex:M.A.~Pickering$^{\rm 120}$,
atlas_authlist.tex:R.~Piegaia$^{\rm 27}$,
atlas_authlist.tex:D.T.~Pignotti$^{\rm 111}$,
atlas_authlist.tex:J.E.~Pilcher$^{\rm 31}$,
atlas_authlist.tex:A.D.~Pilkington$^{\rm 84}$,
atlas_authlist.tex:J.~Pina$^{\rm 126a,126b,126d}$,
atlas_authlist.tex:M.~Pinamonti$^{\rm 164a,164c}$$^{,ad}$,
atlas_authlist.tex:J.L.~Pinfold$^{\rm 3}$,
atlas_authlist.tex:A.~Pingel$^{\rm 36}$,
atlas_authlist.tex:B.~Pinto$^{\rm 126a}$,
atlas_authlist.tex:S.~Pires$^{\rm 80}$,
atlas_authlist.tex:H.~Pirumov$^{\rm 42}$,
atlas_authlist.tex:M.~Pitt$^{\rm 172}$,
atlas_authlist.tex:C.~Pizio$^{\rm 91a,91b}$,
atlas_authlist.tex:L.~Plazak$^{\rm 144a}$,
atlas_authlist.tex:M.-A.~Pleier$^{\rm 25}$,
atlas_authlist.tex:V.~Pleskot$^{\rm 129}$,
atlas_authlist.tex:E.~Plotnikova$^{\rm 65}$,
atlas_authlist.tex:P.~Plucinski$^{\rm 146a,146b}$,
atlas_authlist.tex:D.~Pluth$^{\rm 64}$,
atlas_authlist.tex:R.~Poettgen$^{\rm 146a,146b}$,
atlas_authlist.tex:L.~Poggioli$^{\rm 117}$,
atlas_authlist.tex:D.~Pohl$^{\rm 21}$,
atlas_authlist.tex:G.~Polesello$^{\rm 121a}$,
atlas_authlist.tex:A.~Poley$^{\rm 42}$,
atlas_authlist.tex:A.~Policicchio$^{\rm 37a,37b}$,
atlas_authlist.tex:R.~Polifka$^{\rm 158}$,
atlas_authlist.tex:A.~Polini$^{\rm 20a}$,
atlas_authlist.tex:C.S.~Pollard$^{\rm 53}$,
atlas_authlist.tex:V.~Polychronakos$^{\rm 25}$,
atlas_authlist.tex:K.~Pomm\`es$^{\rm 30}$,
atlas_authlist.tex:L.~Pontecorvo$^{\rm 132a}$,
atlas_authlist.tex:B.G.~Pope$^{\rm 90}$,
atlas_authlist.tex:G.A.~Popeneciu$^{\rm 26b}$,
atlas_authlist.tex:D.S.~Popovic$^{\rm 13}$,
atlas_authlist.tex:A.~Poppleton$^{\rm 30}$,
atlas_authlist.tex:S.~Pospisil$^{\rm 128}$,
atlas_authlist.tex:K.~Potamianos$^{\rm 15}$,
atlas_authlist.tex:I.N.~Potrap$^{\rm 65}$,
atlas_authlist.tex:C.J.~Potter$^{\rm 149}$,
atlas_authlist.tex:C.T.~Potter$^{\rm 116}$,
atlas_authlist.tex:G.~Poulard$^{\rm 30}$,
atlas_authlist.tex:J.~Poveda$^{\rm 30}$,
atlas_authlist.tex:V.~Pozdnyakov$^{\rm 65}$,
atlas_authlist.tex:P.~Pralavorio$^{\rm 85}$,
atlas_authlist.tex:A.~Pranko$^{\rm 15}$,
atlas_authlist.tex:S.~Prasad$^{\rm 30}$,
atlas_authlist.tex:S.~Prell$^{\rm 64}$,
atlas_authlist.tex:D.~Price$^{\rm 84}$,
atlas_authlist.tex:L.E.~Price$^{\rm 6}$,
atlas_authlist.tex:M.~Primavera$^{\rm 73a}$,
atlas_authlist.tex:S.~Prince$^{\rm 87}$,
atlas_authlist.tex:M.~Proissl$^{\rm 46}$,
atlas_authlist.tex:K.~Prokofiev$^{\rm 60c}$,
atlas_authlist.tex:F.~Prokoshin$^{\rm 32b}$,
atlas_authlist.tex:E.~Protopapadaki$^{\rm 136}$,
atlas_authlist.tex:S.~Protopopescu$^{\rm 25}$,
atlas_authlist.tex:J.~Proudfoot$^{\rm 6}$,
atlas_authlist.tex:M.~Przybycien$^{\rm 38a}$,
atlas_authlist.tex:E.~Ptacek$^{\rm 116}$,
atlas_authlist.tex:D.~Puddu$^{\rm 134a,134b}$,
atlas_authlist.tex:E.~Pueschel$^{\rm 86}$,
atlas_authlist.tex:D.~Puldon$^{\rm 148}$,
atlas_authlist.tex:M.~Purohit$^{\rm 25}$$^{,ae}$,
atlas_authlist.tex:P.~Puzo$^{\rm 117}$,
atlas_authlist.tex:J.~Qian$^{\rm 89}$,
atlas_authlist.tex:G.~Qin$^{\rm 53}$,
atlas_authlist.tex:Y.~Qin$^{\rm 84}$,
atlas_authlist.tex:A.~Quadt$^{\rm 54}$,
atlas_authlist.tex:D.R.~Quarrie$^{\rm 15}$,
atlas_authlist.tex:W.B.~Quayle$^{\rm 164a,164b}$,
atlas_authlist.tex:M.~Queitsch-Maitland$^{\rm 84}$,
atlas_authlist.tex:D.~Quilty$^{\rm 53}$,
atlas_authlist.tex:S.~Raddum$^{\rm 119}$,
atlas_authlist.tex:V.~Radeka$^{\rm 25}$,
atlas_authlist.tex:V.~Radescu$^{\rm 42}$,
atlas_authlist.tex:S.K.~Radhakrishnan$^{\rm 148}$,
atlas_authlist.tex:P.~Radloff$^{\rm 116}$,
atlas_authlist.tex:P.~Rados$^{\rm 88}$,
atlas_authlist.tex:F.~Ragusa$^{\rm 91a,91b}$,
atlas_authlist.tex:G.~Rahal$^{\rm 178}$,
atlas_authlist.tex:S.~Rajagopalan$^{\rm 25}$,
atlas_authlist.tex:M.~Rammensee$^{\rm 30}$,
atlas_authlist.tex:C.~Rangel-Smith$^{\rm 166}$,
atlas_authlist.tex:F.~Rauscher$^{\rm 100}$,
atlas_authlist.tex:S.~Rave$^{\rm 83}$,
atlas_authlist.tex:T.~Ravenscroft$^{\rm 53}$,
atlas_authlist.tex:M.~Raymond$^{\rm 30}$,
atlas_authlist.tex:A.L.~Read$^{\rm 119}$,
atlas_authlist.tex:N.P.~Readioff$^{\rm 74}$,
atlas_authlist.tex:D.M.~Rebuzzi$^{\rm 121a,121b}$,
atlas_authlist.tex:A.~Redelbach$^{\rm 174}$,
atlas_authlist.tex:G.~Redlinger$^{\rm 25}$,
atlas_authlist.tex:R.~Reece$^{\rm 137}$,
atlas_authlist.tex:K.~Reeves$^{\rm 41}$,
atlas_authlist.tex:L.~Rehnisch$^{\rm 16}$,
atlas_authlist.tex:J.~Reichert$^{\rm 122}$,
atlas_authlist.tex:H.~Reisin$^{\rm 27}$,
atlas_authlist.tex:M.~Relich$^{\rm 163}$,
atlas_authlist.tex:C.~Rembser$^{\rm 30}$,
atlas_authlist.tex:H.~Ren$^{\rm 33a}$,
atlas_authlist.tex:A.~Renaud$^{\rm 117}$,
atlas_authlist.tex:M.~Rescigno$^{\rm 132a}$,
atlas_authlist.tex:S.~Resconi$^{\rm 91a}$,
atlas_authlist.tex:O.L.~Rezanova$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:P.~Reznicek$^{\rm 129}$,
atlas_authlist.tex:R.~Rezvani$^{\rm 95}$,
atlas_authlist.tex:R.~Richter$^{\rm 101}$,
atlas_authlist.tex:S.~Richter$^{\rm 78}$,
atlas_authlist.tex:E.~Richter-Was$^{\rm 38b}$,
atlas_authlist.tex:O.~Ricken$^{\rm 21}$,
atlas_authlist.tex:M.~Ridel$^{\rm 80}$,
atlas_authlist.tex:P.~Rieck$^{\rm 16}$,
atlas_authlist.tex:C.J.~Riegel$^{\rm 175}$,
atlas_authlist.tex:J.~Rieger$^{\rm 54}$,
atlas_authlist.tex:M.~Rijssenbeek$^{\rm 148}$,
atlas_authlist.tex:A.~Rimoldi$^{\rm 121a,121b}$,
atlas_authlist.tex:L.~Rinaldi$^{\rm 20a}$,
atlas_authlist.tex:B.~Risti\'{c}$^{\rm 49}$,
atlas_authlist.tex:E.~Ritsch$^{\rm 30}$,
atlas_authlist.tex:I.~Riu$^{\rm 12}$,
atlas_authlist.tex:F.~Rizatdinova$^{\rm 114}$,
atlas_authlist.tex:E.~Rizvi$^{\rm 76}$,
atlas_authlist.tex:S.H.~Robertson$^{\rm 87}$$^{,k}$,
atlas_authlist.tex:A.~Robichaud-Veronneau$^{\rm 87}$,
atlas_authlist.tex:D.~Robinson$^{\rm 28}$,
atlas_authlist.tex:J.E.M.~Robinson$^{\rm 42}$,
atlas_authlist.tex:A.~Robson$^{\rm 53}$,
atlas_authlist.tex:C.~Roda$^{\rm 124a,124b}$,
atlas_authlist.tex:S.~Roe$^{\rm 30}$,
atlas_authlist.tex:O.~R{\o}hne$^{\rm 119}$,
atlas_authlist.tex:S.~Rolli$^{\rm 161}$,
atlas_authlist.tex:A.~Romaniouk$^{\rm 98}$,
atlas_authlist.tex:M.~Romano$^{\rm 20a,20b}$,
atlas_authlist.tex:S.M.~Romano~Saez$^{\rm 34}$,
atlas_authlist.tex:E.~Romero~Adam$^{\rm 167}$,
atlas_authlist.tex:N.~Rompotis$^{\rm 138}$,
atlas_authlist.tex:M.~Ronzani$^{\rm 48}$,
atlas_authlist.tex:L.~Roos$^{\rm 80}$,
atlas_authlist.tex:E.~Ros$^{\rm 167}$,
atlas_authlist.tex:S.~Rosati$^{\rm 132a}$,
atlas_authlist.tex:K.~Rosbach$^{\rm 48}$,
atlas_authlist.tex:P.~Rose$^{\rm 137}$,
atlas_authlist.tex:P.L.~Rosendahl$^{\rm 14}$,
atlas_authlist.tex:O.~Rosenthal$^{\rm 141}$,
atlas_authlist.tex:V.~Rossetti$^{\rm 146a,146b}$,
atlas_authlist.tex:E.~Rossi$^{\rm 104a,104b}$,
atlas_authlist.tex:L.P.~Rossi$^{\rm 50a}$,
atlas_authlist.tex:R.~Rosten$^{\rm 138}$,
atlas_authlist.tex:M.~Rotaru$^{\rm 26a}$,
atlas_authlist.tex:I.~Roth$^{\rm 172}$,
atlas_authlist.tex:J.~Rothberg$^{\rm 138}$,
atlas_authlist.tex:D.~Rousseau$^{\rm 117}$,
atlas_authlist.tex:C.R.~Royon$^{\rm 136}$,
atlas_authlist.tex:A.~Rozanov$^{\rm 85}$,
atlas_authlist.tex:Y.~Rozen$^{\rm 152}$,
atlas_authlist.tex:X.~Ruan$^{\rm 145c}$,
atlas_authlist.tex:F.~Rubbo$^{\rm 143}$,
atlas_authlist.tex:I.~Rubinskiy$^{\rm 42}$,
atlas_authlist.tex:V.I.~Rud$^{\rm 99}$,
atlas_authlist.tex:C.~Rudolph$^{\rm 44}$,
atlas_authlist.tex:M.S.~Rudolph$^{\rm 158}$,
atlas_authlist.tex:F.~R\"uhr$^{\rm 48}$,
atlas_authlist.tex:A.~Ruiz-Martinez$^{\rm 30}$,
atlas_authlist.tex:Z.~Rurikova$^{\rm 48}$,
atlas_authlist.tex:N.A.~Rusakovich$^{\rm 65}$,
atlas_authlist.tex:A.~Ruschke$^{\rm 100}$,
atlas_authlist.tex:H.L.~Russell$^{\rm 138}$,
atlas_authlist.tex:J.P.~Rutherfoord$^{\rm 7}$,
atlas_authlist.tex:N.~Ruthmann$^{\rm 48}$,
atlas_authlist.tex:Y.F.~Ryabov$^{\rm 123}$,
atlas_authlist.tex:M.~Rybar$^{\rm 165}$,
atlas_authlist.tex:G.~Rybkin$^{\rm 117}$,
atlas_authlist.tex:N.C.~Ryder$^{\rm 120}$,
atlas_authlist.tex:A.F.~Saavedra$^{\rm 150}$,
atlas_authlist.tex:G.~Sabato$^{\rm 107}$,
atlas_authlist.tex:S.~Sacerdoti$^{\rm 27}$,
atlas_authlist.tex:A.~Saddique$^{\rm 3}$,
atlas_authlist.tex:H.F-W.~Sadrozinski$^{\rm 137}$,
atlas_authlist.tex:R.~Sadykov$^{\rm 65}$,
atlas_authlist.tex:F.~Safai~Tehrani$^{\rm 132a}$,
atlas_authlist.tex:M.~Saimpert$^{\rm 136}$,
atlas_authlist.tex:T.~Saito$^{\rm 155}$,
atlas_authlist.tex:H.~Sakamoto$^{\rm 155}$,
atlas_authlist.tex:Y.~Sakurai$^{\rm 171}$,
atlas_authlist.tex:G.~Salamanna$^{\rm 134a,134b}$,
atlas_authlist.tex:A.~Salamon$^{\rm 133a}$,
atlas_authlist.tex:M.~Saleem$^{\rm 113}$,
atlas_authlist.tex:D.~Salek$^{\rm 107}$,
atlas_authlist.tex:P.H.~Sales~De~Bruin$^{\rm 138}$,
atlas_authlist.tex:D.~Salihagic$^{\rm 101}$,
atlas_authlist.tex:A.~Salnikov$^{\rm 143}$,
atlas_authlist.tex:J.~Salt$^{\rm 167}$,
atlas_authlist.tex:D.~Salvatore$^{\rm 37a,37b}$,
atlas_authlist.tex:F.~Salvatore$^{\rm 149}$,
atlas_authlist.tex:A.~Salvucci$^{\rm 106}$,
atlas_authlist.tex:A.~Salzburger$^{\rm 30}$,
atlas_authlist.tex:D.~Sammel$^{\rm 48}$,
atlas_authlist.tex:D.~Sampsonidis$^{\rm 154}$,
atlas_authlist.tex:A.~Sanchez$^{\rm 104a,104b}$,
atlas_authlist.tex:J.~S\'anchez$^{\rm 167}$,
atlas_authlist.tex:V.~Sanchez~Martinez$^{\rm 167}$,
atlas_authlist.tex:H.~Sandaker$^{\rm 119}$,
atlas_authlist.tex:R.L.~Sandbach$^{\rm 76}$,
atlas_authlist.tex:H.G.~Sander$^{\rm 83}$,
atlas_authlist.tex:M.P.~Sanders$^{\rm 100}$,
atlas_authlist.tex:M.~Sandhoff$^{\rm 175}$,
atlas_authlist.tex:C.~Sandoval$^{\rm 162}$,
atlas_authlist.tex:R.~Sandstroem$^{\rm 101}$,
atlas_authlist.tex:D.P.C.~Sankey$^{\rm 131}$,
atlas_authlist.tex:M.~Sannino$^{\rm 50a,50b}$,
atlas_authlist.tex:A.~Sansoni$^{\rm 47}$,
atlas_authlist.tex:C.~Santoni$^{\rm 34}$,
atlas_authlist.tex:R.~Santonico$^{\rm 133a,133b}$,
atlas_authlist.tex:H.~Santos$^{\rm 126a}$,
atlas_authlist.tex:I.~Santoyo~Castillo$^{\rm 149}$,
atlas_authlist.tex:K.~Sapp$^{\rm 125}$,
atlas_authlist.tex:A.~Sapronov$^{\rm 65}$,
atlas_authlist.tex:J.G.~Saraiva$^{\rm 126a,126d}$,
atlas_authlist.tex:B.~Sarrazin$^{\rm 21}$,
atlas_authlist.tex:O.~Sasaki$^{\rm 66}$,
atlas_authlist.tex:Y.~Sasaki$^{\rm 155}$,
atlas_authlist.tex:K.~Sato$^{\rm 160}$,
atlas_authlist.tex:G.~Sauvage$^{\rm 5}$$^{,*}$,
atlas_authlist.tex:E.~Sauvan$^{\rm 5}$,
atlas_authlist.tex:G.~Savage$^{\rm 77}$,
atlas_authlist.tex:P.~Savard$^{\rm 158}$$^{,d}$,
atlas_authlist.tex:C.~Sawyer$^{\rm 131}$,
atlas_authlist.tex:L.~Sawyer$^{\rm 79}$$^{,n}$,
atlas_authlist.tex:J.~Saxon$^{\rm 31}$,
atlas_authlist.tex:C.~Sbarra$^{\rm 20a}$,
atlas_authlist.tex:A.~Sbrizzi$^{\rm 20a,20b}$,
atlas_authlist.tex:T.~Scanlon$^{\rm 78}$,
atlas_authlist.tex:D.A.~Scannicchio$^{\rm 163}$,
atlas_authlist.tex:M.~Scarcella$^{\rm 150}$,
atlas_authlist.tex:V.~Scarfone$^{\rm 37a,37b}$,
atlas_authlist.tex:J.~Schaarschmidt$^{\rm 172}$,
atlas_authlist.tex:P.~Schacht$^{\rm 101}$,
atlas_authlist.tex:D.~Schaefer$^{\rm 30}$,
atlas_authlist.tex:R.~Schaefer$^{\rm 42}$,
atlas_authlist.tex:J.~Schaeffer$^{\rm 83}$,
atlas_authlist.tex:S.~Schaepe$^{\rm 21}$,
atlas_authlist.tex:S.~Schaetzel$^{\rm 58b}$,
atlas_authlist.tex:U.~Sch\"afer$^{\rm 83}$,
atlas_authlist.tex:A.C.~Schaffer$^{\rm 117}$,
atlas_authlist.tex:D.~Schaile$^{\rm 100}$,
atlas_authlist.tex:R.D.~Schamberger$^{\rm 148}$,
atlas_authlist.tex:V.~Scharf$^{\rm 58a}$,
atlas_authlist.tex:V.A.~Schegelsky$^{\rm 123}$,
atlas_authlist.tex:D.~Scheirich$^{\rm 129}$,
atlas_authlist.tex:M.~Schernau$^{\rm 163}$,
atlas_authlist.tex:C.~Schiavi$^{\rm 50a,50b}$,
atlas_authlist.tex:C.~Schillo$^{\rm 48}$,
atlas_authlist.tex:M.~Schioppa$^{\rm 37a,37b}$,
atlas_authlist.tex:S.~Schlenker$^{\rm 30}$,
atlas_authlist.tex:E.~Schmidt$^{\rm 48}$,
atlas_authlist.tex:K.~Schmieden$^{\rm 30}$,
atlas_authlist.tex:C.~Schmitt$^{\rm 83}$,
atlas_authlist.tex:S.~Schmitt$^{\rm 58b}$,
atlas_authlist.tex:S.~Schmitt$^{\rm 42}$,
atlas_authlist.tex:B.~Schneider$^{\rm 159a}$,
atlas_authlist.tex:Y.J.~Schnellbach$^{\rm 74}$,
atlas_authlist.tex:U.~Schnoor$^{\rm 44}$,
atlas_authlist.tex:L.~Schoeffel$^{\rm 136}$,
atlas_authlist.tex:A.~Schoening$^{\rm 58b}$,
atlas_authlist.tex:B.D.~Schoenrock$^{\rm 90}$,
atlas_authlist.tex:E.~Schopf$^{\rm 21}$,
atlas_authlist.tex:A.L.S.~Schorlemmer$^{\rm 54}$,
atlas_authlist.tex:M.~Schott$^{\rm 83}$,
atlas_authlist.tex:D.~Schouten$^{\rm 159a}$,
atlas_authlist.tex:J.~Schovancova$^{\rm 8}$,
atlas_authlist.tex:S.~Schramm$^{\rm 49}$,
atlas_authlist.tex:M.~Schreyer$^{\rm 174}$,
atlas_authlist.tex:C.~Schroeder$^{\rm 83}$,
atlas_authlist.tex:N.~Schuh$^{\rm 83}$,
atlas_authlist.tex:M.J.~Schultens$^{\rm 21}$,
atlas_authlist.tex:H.-C.~Schultz-Coulon$^{\rm 58a}$,
atlas_authlist.tex:H.~Schulz$^{\rm 16}$,
atlas_authlist.tex:M.~Schumacher$^{\rm 48}$,
atlas_authlist.tex:B.A.~Schumm$^{\rm 137}$,
atlas_authlist.tex:Ph.~Schune$^{\rm 136}$,
atlas_authlist.tex:C.~Schwanenberger$^{\rm 84}$,
atlas_authlist.tex:A.~Schwartzman$^{\rm 143}$,
atlas_authlist.tex:T.A.~Schwarz$^{\rm 89}$,
atlas_authlist.tex:Ph.~Schwegler$^{\rm 101}$,
atlas_authlist.tex:H.~Schweiger$^{\rm 84}$,
atlas_authlist.tex:Ph.~Schwemling$^{\rm 136}$,
atlas_authlist.tex:R.~Schwienhorst$^{\rm 90}$,
atlas_authlist.tex:J.~Schwindling$^{\rm 136}$,
atlas_authlist.tex:T.~Schwindt$^{\rm 21}$,
atlas_authlist.tex:F.G.~Sciacca$^{\rm 17}$,
atlas_authlist.tex:E.~Scifo$^{\rm 117}$,
atlas_authlist.tex:G.~Sciolla$^{\rm 23}$,
atlas_authlist.tex:F.~Scuri$^{\rm 124a,124b}$,
atlas_authlist.tex:F.~Scutti$^{\rm 21}$,
atlas_authlist.tex:J.~Searcy$^{\rm 89}$,
atlas_authlist.tex:G.~Sedov$^{\rm 42}$,
atlas_authlist.tex:E.~Sedykh$^{\rm 123}$,
atlas_authlist.tex:P.~Seema$^{\rm 21}$,
atlas_authlist.tex:S.C.~Seidel$^{\rm 105}$,
atlas_authlist.tex:A.~Seiden$^{\rm 137}$,
atlas_authlist.tex:F.~Seifert$^{\rm 128}$,
atlas_authlist.tex:J.M.~Seixas$^{\rm 24a}$,
atlas_authlist.tex:G.~Sekhniaidze$^{\rm 104a}$,
atlas_authlist.tex:K.~Sekhon$^{\rm 89}$,
atlas_authlist.tex:S.J.~Sekula$^{\rm 40}$,
atlas_authlist.tex:D.M.~Seliverstov$^{\rm 123}$$^{,*}$,
atlas_authlist.tex:N.~Semprini-Cesari$^{\rm 20a,20b}$,
atlas_authlist.tex:C.~Serfon$^{\rm 30}$,
atlas_authlist.tex:L.~Serin$^{\rm 117}$,
atlas_authlist.tex:L.~Serkin$^{\rm 164a,164b}$,
atlas_authlist.tex:T.~Serre$^{\rm 85}$,
atlas_authlist.tex:M.~Sessa$^{\rm 134a,134b}$,
atlas_authlist.tex:R.~Seuster$^{\rm 159a}$,
atlas_authlist.tex:H.~Severini$^{\rm 113}$,
atlas_authlist.tex:T.~Sfiligoj$^{\rm 75}$,
atlas_authlist.tex:F.~Sforza$^{\rm 30}$,
atlas_authlist.tex:A.~Sfyrla$^{\rm 30}$,
atlas_authlist.tex:E.~Shabalina$^{\rm 54}$,
atlas_authlist.tex:M.~Shamim$^{\rm 116}$,
atlas_authlist.tex:L.Y.~Shan$^{\rm 33a}$,
atlas_authlist.tex:R.~Shang$^{\rm 165}$,
atlas_authlist.tex:J.T.~Shank$^{\rm 22}$,
atlas_authlist.tex:M.~Shapiro$^{\rm 15}$,
atlas_authlist.tex:P.B.~Shatalov$^{\rm 97}$,
atlas_authlist.tex:K.~Shaw$^{\rm 164a,164b}$,
atlas_authlist.tex:S.M.~Shaw$^{\rm 84}$,
atlas_authlist.tex:A.~Shcherbakova$^{\rm 146a,146b}$,
atlas_authlist.tex:C.Y.~Shehu$^{\rm 149}$,
atlas_authlist.tex:P.~Sherwood$^{\rm 78}$,
atlas_authlist.tex:L.~Shi$^{\rm 151}$$^{,af}$,
atlas_authlist.tex:S.~Shimizu$^{\rm 67}$,
atlas_authlist.tex:C.O.~Shimmin$^{\rm 163}$,
atlas_authlist.tex:M.~Shimojima$^{\rm 102}$,
atlas_authlist.tex:M.~Shiyakova$^{\rm 65}$,
atlas_authlist.tex:A.~Shmeleva$^{\rm 96}$,
atlas_authlist.tex:D.~Shoaleh~Saadi$^{\rm 95}$,
atlas_authlist.tex:M.J.~Shochet$^{\rm 31}$,
atlas_authlist.tex:S.~Shojaii$^{\rm 91a,91b}$,
atlas_authlist.tex:S.~Shrestha$^{\rm 111}$,
atlas_authlist.tex:E.~Shulga$^{\rm 98}$,
atlas_authlist.tex:M.A.~Shupe$^{\rm 7}$,
atlas_authlist.tex:S.~Shushkevich$^{\rm 42}$,
atlas_authlist.tex:P.~Sicho$^{\rm 127}$,
atlas_authlist.tex:P.E.~Sidebo$^{\rm 147}$,
atlas_authlist.tex:O.~Sidiropoulou$^{\rm 174}$,
atlas_authlist.tex:D.~Sidorov$^{\rm 114}$,
atlas_authlist.tex:A.~Sidoti$^{\rm 20a,20b}$,
atlas_authlist.tex:F.~Siegert$^{\rm 44}$,
atlas_authlist.tex:Dj.~Sijacki$^{\rm 13}$,
atlas_authlist.tex:J.~Silva$^{\rm 126a,126d}$,
atlas_authlist.tex:Y.~Silver$^{\rm 153}$,
atlas_authlist.tex:S.B.~Silverstein$^{\rm 146a}$,
atlas_authlist.tex:V.~Simak$^{\rm 128}$,
atlas_authlist.tex:O.~Simard$^{\rm 5}$,
atlas_authlist.tex:Lj.~Simic$^{\rm 13}$,
atlas_authlist.tex:S.~Simion$^{\rm 117}$,
atlas_authlist.tex:E.~Simioni$^{\rm 83}$,
atlas_authlist.tex:B.~Simmons$^{\rm 78}$,
atlas_authlist.tex:D.~Simon$^{\rm 34}$,
atlas_authlist.tex:R.~Simoniello$^{\rm 91a,91b}$,
atlas_authlist.tex:P.~Sinervo$^{\rm 158}$,
atlas_authlist.tex:N.B.~Sinev$^{\rm 116}$,
atlas_authlist.tex:M.~Sioli$^{\rm 20a,20b}$,
atlas_authlist.tex:G.~Siragusa$^{\rm 174}$,
atlas_authlist.tex:A.N.~Sisakyan$^{\rm 65}$$^{,*}$,
atlas_authlist.tex:S.Yu.~Sivoklokov$^{\rm 99}$,
atlas_authlist.tex:J.~Sj\"{o}lin$^{\rm 146a,146b}$,
atlas_authlist.tex:T.B.~Sjursen$^{\rm 14}$,
atlas_authlist.tex:M.B.~Skinner$^{\rm 72}$,
atlas_authlist.tex:H.P.~Skottowe$^{\rm 57}$,
atlas_authlist.tex:P.~Skubic$^{\rm 113}$,
atlas_authlist.tex:M.~Slater$^{\rm 18}$,
atlas_authlist.tex:T.~Slavicek$^{\rm 128}$,
atlas_authlist.tex:M.~Slawinska$^{\rm 107}$,
atlas_authlist.tex:K.~Sliwa$^{\rm 161}$,
atlas_authlist.tex:V.~Smakhtin$^{\rm 172}$,
atlas_authlist.tex:B.H.~Smart$^{\rm 46}$,
atlas_authlist.tex:L.~Smestad$^{\rm 14}$,
atlas_authlist.tex:S.Yu.~Smirnov$^{\rm 98}$,
atlas_authlist.tex:Y.~Smirnov$^{\rm 98}$,
atlas_authlist.tex:L.N.~Smirnova$^{\rm 99}$$^{,ag}$,
atlas_authlist.tex:O.~Smirnova$^{\rm 81}$,
atlas_authlist.tex:M.N.K.~Smith$^{\rm 35}$,
atlas_authlist.tex:R.W.~Smith$^{\rm 35}$,
atlas_authlist.tex:M.~Smizanska$^{\rm 72}$,
atlas_authlist.tex:K.~Smolek$^{\rm 128}$,
atlas_authlist.tex:A.A.~Snesarev$^{\rm 96}$,
atlas_authlist.tex:G.~Snidero$^{\rm 76}$,
atlas_authlist.tex:S.~Snyder$^{\rm 25}$,
atlas_authlist.tex:R.~Sobie$^{\rm 169}$$^{,k}$,
atlas_authlist.tex:F.~Socher$^{\rm 44}$,
atlas_authlist.tex:A.~Soffer$^{\rm 153}$,
atlas_authlist.tex:D.A.~Soh$^{\rm 151}$$^{,af}$,
atlas_authlist.tex:C.A.~Solans$^{\rm 30}$,
atlas_authlist.tex:M.~Solar$^{\rm 128}$,
atlas_authlist.tex:J.~Solc$^{\rm 128}$,
atlas_authlist.tex:E.Yu.~Soldatov$^{\rm 98}$,
atlas_authlist.tex:U.~Soldevila$^{\rm 167}$,
atlas_authlist.tex:A.A.~Solodkov$^{\rm 130}$,
atlas_authlist.tex:A.~Soloshenko$^{\rm 65}$,
atlas_authlist.tex:O.V.~Solovyanov$^{\rm 130}$,
atlas_authlist.tex:V.~Solovyev$^{\rm 123}$,
atlas_authlist.tex:P.~Sommer$^{\rm 48}$,
atlas_authlist.tex:H.Y.~Song$^{\rm 33b}$,
atlas_authlist.tex:N.~Soni$^{\rm 1}$,
atlas_authlist.tex:A.~Sood$^{\rm 15}$,
atlas_authlist.tex:A.~Sopczak$^{\rm 128}$,
atlas_authlist.tex:B.~Sopko$^{\rm 128}$,
atlas_authlist.tex:V.~Sopko$^{\rm 128}$,
atlas_authlist.tex:V.~Sorin$^{\rm 12}$,
atlas_authlist.tex:D.~Sosa$^{\rm 58b}$,
atlas_authlist.tex:M.~Sosebee$^{\rm 8}$,
atlas_authlist.tex:C.L.~Sotiropoulou$^{\rm 124a,124b}$,
atlas_authlist.tex:R.~Soualah$^{\rm 164a,164c}$,
atlas_authlist.tex:A.M.~Soukharev$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:D.~South$^{\rm 42}$,
atlas_authlist.tex:B.C.~Sowden$^{\rm 77}$,
atlas_authlist.tex:S.~Spagnolo$^{\rm 73a,73b}$,
atlas_authlist.tex:M.~Spalla$^{\rm 124a,124b}$,
atlas_authlist.tex:F.~Span\`o$^{\rm 77}$,
atlas_authlist.tex:W.R.~Spearman$^{\rm 57}$,
atlas_authlist.tex:D.~Sperlich$^{\rm 16}$,
atlas_authlist.tex:F.~Spettel$^{\rm 101}$,
atlas_authlist.tex:R.~Spighi$^{\rm 20a}$,
atlas_authlist.tex:G.~Spigo$^{\rm 30}$,
atlas_authlist.tex:L.A.~Spiller$^{\rm 88}$,
atlas_authlist.tex:M.~Spousta$^{\rm 129}$,
atlas_authlist.tex:T.~Spreitzer$^{\rm 158}$,
atlas_authlist.tex:R.D.~St.~Denis$^{\rm 53}$$^{,*}$,
atlas_authlist.tex:S.~Staerz$^{\rm 44}$,
atlas_authlist.tex:J.~Stahlman$^{\rm 122}$,
atlas_authlist.tex:R.~Stamen$^{\rm 58a}$,
atlas_authlist.tex:S.~Stamm$^{\rm 16}$,
atlas_authlist.tex:E.~Stanecka$^{\rm 39}$,
atlas_authlist.tex:C.~Stanescu$^{\rm 134a}$,
atlas_authlist.tex:M.~Stanescu-Bellu$^{\rm 42}$,
atlas_authlist.tex:M.M.~Stanitzki$^{\rm 42}$,
atlas_authlist.tex:S.~Stapnes$^{\rm 119}$,
atlas_authlist.tex:E.A.~Starchenko$^{\rm 130}$,
atlas_authlist.tex:J.~Stark$^{\rm 55}$,
atlas_authlist.tex:P.~Staroba$^{\rm 127}$,
atlas_authlist.tex:P.~Starovoitov$^{\rm 42}$,
atlas_authlist.tex:R.~Staszewski$^{\rm 39}$,
atlas_authlist.tex:P.~Stavina$^{\rm 144a}$$^{,*}$,
atlas_authlist.tex:P.~Steinberg$^{\rm 25}$,
atlas_authlist.tex:B.~Stelzer$^{\rm 142}$,
atlas_authlist.tex:H.J.~Stelzer$^{\rm 30}$,
atlas_authlist.tex:O.~Stelzer-Chilton$^{\rm 159a}$,
atlas_authlist.tex:H.~Stenzel$^{\rm 52}$,
atlas_authlist.tex:G.A.~Stewart$^{\rm 53}$,
atlas_authlist.tex:J.A.~Stillings$^{\rm 21}$,
atlas_authlist.tex:M.C.~Stockton$^{\rm 87}$,
atlas_authlist.tex:M.~Stoebe$^{\rm 87}$,
atlas_authlist.tex:G.~Stoicea$^{\rm 26a}$,
atlas_authlist.tex:P.~Stolte$^{\rm 54}$,
atlas_authlist.tex:S.~Stonjek$^{\rm 101}$,
atlas_authlist.tex:A.R.~Stradling$^{\rm 8}$,
atlas_authlist.tex:A.~Straessner$^{\rm 44}$,
atlas_authlist.tex:M.E.~Stramaglia$^{\rm 17}$,
atlas_authlist.tex:J.~Strandberg$^{\rm 147}$,
atlas_authlist.tex:S.~Strandberg$^{\rm 146a,146b}$,
atlas_authlist.tex:A.~Strandlie$^{\rm 119}$,
atlas_authlist.tex:E.~Strauss$^{\rm 143}$,
atlas_authlist.tex:M.~Strauss$^{\rm 113}$,
atlas_authlist.tex:P.~Strizenec$^{\rm 144b}$,
atlas_authlist.tex:R.~Str\"ohmer$^{\rm 174}$,
atlas_authlist.tex:D.M.~Strom$^{\rm 116}$,
atlas_authlist.tex:R.~Stroynowski$^{\rm 40}$,
atlas_authlist.tex:A.~Strubig$^{\rm 106}$,
atlas_authlist.tex:S.A.~Stucci$^{\rm 17}$,
atlas_authlist.tex:B.~Stugu$^{\rm 14}$,
atlas_authlist.tex:N.A.~Styles$^{\rm 42}$,
atlas_authlist.tex:D.~Su$^{\rm 143}$,
atlas_authlist.tex:J.~Su$^{\rm 125}$,
atlas_authlist.tex:R.~Subramaniam$^{\rm 79}$,
atlas_authlist.tex:A.~Succurro$^{\rm 12}$,
atlas_authlist.tex:Y.~Sugaya$^{\rm 118}$,
atlas_authlist.tex:C.~Suhr$^{\rm 108}$,
atlas_authlist.tex:M.~Suk$^{\rm 128}$,
atlas_authlist.tex:V.V.~Sulin$^{\rm 96}$,
atlas_authlist.tex:S.~Sultansoy$^{\rm 4c}$,
atlas_authlist.tex:T.~Sumida$^{\rm 68}$,
atlas_authlist.tex:S.~Sun$^{\rm 57}$,
atlas_authlist.tex:X.~Sun$^{\rm 33a}$,
atlas_authlist.tex:J.E.~Sundermann$^{\rm 48}$,
atlas_authlist.tex:K.~Suruliz$^{\rm 149}$,
atlas_authlist.tex:G.~Susinno$^{\rm 37a,37b}$,
atlas_authlist.tex:M.R.~Sutton$^{\rm 149}$,
atlas_authlist.tex:S.~Suzuki$^{\rm 66}$,
atlas_authlist.tex:M.~Svatos$^{\rm 127}$,
atlas_authlist.tex:S.~Swedish$^{\rm 168}$,
atlas_authlist.tex:M.~Swiatlowski$^{\rm 143}$,
atlas_authlist.tex:I.~Sykora$^{\rm 144a}$,
atlas_authlist.tex:T.~Sykora$^{\rm 129}$,
atlas_authlist.tex:D.~Ta$^{\rm 90}$,
atlas_authlist.tex:C.~Taccini$^{\rm 134a,134b}$,
atlas_authlist.tex:K.~Tackmann$^{\rm 42}$,
atlas_authlist.tex:J.~Taenzer$^{\rm 158}$,
atlas_authlist.tex:A.~Taffard$^{\rm 163}$,
atlas_authlist.tex:R.~Tafirout$^{\rm 159a}$,
atlas_authlist.tex:N.~Taiblum$^{\rm 153}$,
atlas_authlist.tex:H.~Takai$^{\rm 25}$,
atlas_authlist.tex:R.~Takashima$^{\rm 69}$,
atlas_authlist.tex:H.~Takeda$^{\rm 67}$,
atlas_authlist.tex:T.~Takeshita$^{\rm 140}$,
atlas_authlist.tex:Y.~Takubo$^{\rm 66}$,
atlas_authlist.tex:M.~Talby$^{\rm 85}$,
atlas_authlist.tex:A.A.~Talyshev$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:J.Y.C.~Tam$^{\rm 174}$,
atlas_authlist.tex:K.G.~Tan$^{\rm 88}$,
atlas_authlist.tex:J.~Tanaka$^{\rm 155}$,
atlas_authlist.tex:R.~Tanaka$^{\rm 117}$,
atlas_authlist.tex:S.~Tanaka$^{\rm 66}$,
atlas_authlist.tex:B.B.~Tannenwald$^{\rm 111}$,
atlas_authlist.tex:N.~Tannoury$^{\rm 21}$,
atlas_authlist.tex:S.~Tapprogge$^{\rm 83}$,
atlas_authlist.tex:S.~Tarem$^{\rm 152}$,
atlas_authlist.tex:F.~Tarrade$^{\rm 29}$,
atlas_authlist.tex:G.F.~Tartarelli$^{\rm 91a}$,
atlas_authlist.tex:P.~Tas$^{\rm 129}$,
atlas_authlist.tex:M.~Tasevsky$^{\rm 127}$,
atlas_authlist.tex:T.~Tashiro$^{\rm 68}$,
atlas_authlist.tex:E.~Tassi$^{\rm 37a,37b}$,
atlas_authlist.tex:A.~Tavares~Delgado$^{\rm 126a,126b}$,
atlas_authlist.tex:Y.~Tayalati$^{\rm 135d}$,
atlas_authlist.tex:F.E.~Taylor$^{\rm 94}$,
atlas_authlist.tex:G.N.~Taylor$^{\rm 88}$,
atlas_authlist.tex:W.~Taylor$^{\rm 159b}$,
atlas_authlist.tex:F.A.~Teischinger$^{\rm 30}$,
atlas_authlist.tex:M.~Teixeira~Dias~Castanheira$^{\rm 76}$,
atlas_authlist.tex:P.~Teixeira-Dias$^{\rm 77}$,
atlas_authlist.tex:K.K.~Temming$^{\rm 48}$,
atlas_authlist.tex:H.~Ten~Kate$^{\rm 30}$,
atlas_authlist.tex:P.K.~Teng$^{\rm 151}$,
atlas_authlist.tex:J.J.~Teoh$^{\rm 118}$,
atlas_authlist.tex:F.~Tepel$^{\rm 175}$,
atlas_authlist.tex:S.~Terada$^{\rm 66}$,
atlas_authlist.tex:K.~Terashi$^{\rm 155}$,
atlas_authlist.tex:J.~Terron$^{\rm 82}$,
atlas_authlist.tex:S.~Terzo$^{\rm 101}$,
atlas_authlist.tex:M.~Testa$^{\rm 47}$,
atlas_authlist.tex:R.J.~Teuscher$^{\rm 158}$$^{,k}$,
atlas_authlist.tex:T.~Theveneaux-Pelzer$^{\rm 34}$,
atlas_authlist.tex:J.P.~Thomas$^{\rm 18}$,
atlas_authlist.tex:J.~Thomas-Wilsker$^{\rm 77}$,
atlas_authlist.tex:E.N.~Thompson$^{\rm 35}$,
atlas_authlist.tex:P.D.~Thompson$^{\rm 18}$,
atlas_authlist.tex:R.J.~Thompson$^{\rm 84}$,
atlas_authlist.tex:A.S.~Thompson$^{\rm 53}$,
atlas_authlist.tex:L.A.~Thomsen$^{\rm 176}$,
atlas_authlist.tex:E.~Thomson$^{\rm 122}$,
atlas_authlist.tex:M.~Thomson$^{\rm 28}$,
atlas_authlist.tex:R.P.~Thun$^{\rm 89}$$^{,*}$,
atlas_authlist.tex:M.J.~Tibbetts$^{\rm 15}$,
atlas_authlist.tex:R.E.~Ticse~Torres$^{\rm 85}$,
atlas_authlist.tex:V.O.~Tikhomirov$^{\rm 96}$$^{,ah}$,
atlas_authlist.tex:Yu.A.~Tikhonov$^{\rm 109}$$^{,c}$,
atlas_authlist.tex:S.~Timoshenko$^{\rm 98}$,
atlas_authlist.tex:E.~Tiouchichine$^{\rm 85}$,
atlas_authlist.tex:P.~Tipton$^{\rm 176}$,
atlas_authlist.tex:S.~Tisserant$^{\rm 85}$,
atlas_authlist.tex:K.~Todome$^{\rm 157}$,
atlas_authlist.tex:T.~Todorov$^{\rm 5}$$^{,*}$,
atlas_authlist.tex:S.~Todorova-Nova$^{\rm 129}$,
atlas_authlist.tex:J.~Tojo$^{\rm 70}$,
atlas_authlist.tex:S.~Tok\'ar$^{\rm 144a}$,
atlas_authlist.tex:K.~Tokushuku$^{\rm 66}$,
atlas_authlist.tex:K.~Tollefson$^{\rm 90}$,
atlas_authlist.tex:E.~Tolley$^{\rm 57}$,
atlas_authlist.tex:L.~Tomlinson$^{\rm 84}$,
atlas_authlist.tex:M.~Tomoto$^{\rm 103}$,
atlas_authlist.tex:L.~Tompkins$^{\rm 143}$$^{,ai}$,
atlas_authlist.tex:K.~Toms$^{\rm 105}$,
atlas_authlist.tex:E.~Torrence$^{\rm 116}$,
atlas_authlist.tex:H.~Torres$^{\rm 142}$,
atlas_authlist.tex:E.~Torr\'o~Pastor$^{\rm 167}$,
atlas_authlist.tex:J.~Toth$^{\rm 85}$$^{,aj}$,
atlas_authlist.tex:F.~Touchard$^{\rm 85}$,
atlas_authlist.tex:D.R.~Tovey$^{\rm 139}$,
atlas_authlist.tex:T.~Trefzger$^{\rm 174}$,
atlas_authlist.tex:L.~Tremblet$^{\rm 30}$,
atlas_authlist.tex:A.~Tricoli$^{\rm 30}$,
atlas_authlist.tex:I.M.~Trigger$^{\rm 159a}$,
atlas_authlist.tex:S.~Trincaz-Duvoid$^{\rm 80}$,
atlas_authlist.tex:M.F.~Tripiana$^{\rm 12}$,
atlas_authlist.tex:W.~Trischuk$^{\rm 158}$,
atlas_authlist.tex:B.~Trocm\'e$^{\rm 55}$,
atlas_authlist.tex:C.~Troncon$^{\rm 91a}$,
atlas_authlist.tex:M.~Trottier-McDonald$^{\rm 15}$,
atlas_authlist.tex:M.~Trovatelli$^{\rm 169}$,
atlas_authlist.tex:P.~True$^{\rm 90}$,
atlas_authlist.tex:L.~Truong$^{\rm 164a,164c}$,
atlas_authlist.tex:M.~Trzebinski$^{\rm 39}$,
atlas_authlist.tex:A.~Trzupek$^{\rm 39}$,
atlas_authlist.tex:C.~Tsarouchas$^{\rm 30}$,
atlas_authlist.tex:J.C-L.~Tseng$^{\rm 120}$,
atlas_authlist.tex:P.V.~Tsiareshka$^{\rm 92}$,
atlas_authlist.tex:D.~Tsionou$^{\rm 154}$,
atlas_authlist.tex:G.~Tsipolitis$^{\rm 10}$,
atlas_authlist.tex:N.~Tsirintanis$^{\rm 9}$,
atlas_authlist.tex:S.~Tsiskaridze$^{\rm 12}$,
atlas_authlist.tex:V.~Tsiskaridze$^{\rm 48}$,
atlas_authlist.tex:E.G.~Tskhadadze$^{\rm 51a}$,
atlas_authlist.tex:I.I.~Tsukerman$^{\rm 97}$,
atlas_authlist.tex:V.~Tsulaia$^{\rm 15}$,
atlas_authlist.tex:S.~Tsuno$^{\rm 66}$,
atlas_authlist.tex:D.~Tsybychev$^{\rm 148}$,
atlas_authlist.tex:A.~Tudorache$^{\rm 26a}$,
atlas_authlist.tex:V.~Tudorache$^{\rm 26a}$,
atlas_authlist.tex:A.N.~Tuna$^{\rm 122}$,
atlas_authlist.tex:S.A.~Tupputi$^{\rm 20a,20b}$,
atlas_authlist.tex:S.~Turchikhin$^{\rm 99}$$^{,ag}$,
atlas_authlist.tex:D.~Turecek$^{\rm 128}$,
atlas_authlist.tex:R.~Turra$^{\rm 91a,91b}$,
atlas_authlist.tex:A.J.~Turvey$^{\rm 40}$,
atlas_authlist.tex:P.M.~Tuts$^{\rm 35}$,
atlas_authlist.tex:A.~Tykhonov$^{\rm 49}$,
atlas_authlist.tex:M.~Tylmad$^{\rm 146a,146b}$,
atlas_authlist.tex:M.~Tyndel$^{\rm 131}$,
atlas_authlist.tex:I.~Ueda$^{\rm 155}$,
atlas_authlist.tex:R.~Ueno$^{\rm 29}$,
atlas_authlist.tex:M.~Ughetto$^{\rm 146a,146b}$,
atlas_authlist.tex:M.~Ugland$^{\rm 14}$,
atlas_authlist.tex:M.~Uhlenbrock$^{\rm 21}$,
atlas_authlist.tex:F.~Ukegawa$^{\rm 160}$,
atlas_authlist.tex:G.~Unal$^{\rm 30}$,
atlas_authlist.tex:A.~Undrus$^{\rm 25}$,
atlas_authlist.tex:G.~Unel$^{\rm 163}$,
atlas_authlist.tex:F.C.~Ungaro$^{\rm 48}$,
atlas_authlist.tex:Y.~Unno$^{\rm 66}$,
atlas_authlist.tex:C.~Unverdorben$^{\rm 100}$,
atlas_authlist.tex:J.~Urban$^{\rm 144b}$,
atlas_authlist.tex:P.~Urquijo$^{\rm 88}$,
atlas_authlist.tex:P.~Urrejola$^{\rm 83}$,
atlas_authlist.tex:G.~Usai$^{\rm 8}$,
atlas_authlist.tex:A.~Usanova$^{\rm 62}$,
atlas_authlist.tex:L.~Vacavant$^{\rm 85}$,
atlas_authlist.tex:V.~Vacek$^{\rm 128}$,
atlas_authlist.tex:B.~Vachon$^{\rm 87}$,
atlas_authlist.tex:C.~Valderanis$^{\rm 83}$,
atlas_authlist.tex:N.~Valencic$^{\rm 107}$,
atlas_authlist.tex:S.~Valentinetti$^{\rm 20a,20b}$,
atlas_authlist.tex:A.~Valero$^{\rm 167}$,
atlas_authlist.tex:L.~Valery$^{\rm 12}$,
atlas_authlist.tex:S.~Valkar$^{\rm 129}$,
atlas_authlist.tex:E.~Valladolid~Gallego$^{\rm 167}$,
atlas_authlist.tex:S.~Vallecorsa$^{\rm 49}$,
atlas_authlist.tex:J.A.~Valls~Ferrer$^{\rm 167}$,
atlas_authlist.tex:W.~Van~Den~Wollenberg$^{\rm 107}$,
atlas_authlist.tex:P.C.~Van~Der~Deijl$^{\rm 107}$,
atlas_authlist.tex:R.~van~der~Geer$^{\rm 107}$,
atlas_authlist.tex:H.~van~der~Graaf$^{\rm 107}$,
atlas_authlist.tex:R.~Van~Der~Leeuw$^{\rm 107}$,
atlas_authlist.tex:N.~van~Eldik$^{\rm 152}$,
atlas_authlist.tex:P.~van~Gemmeren$^{\rm 6}$,
atlas_authlist.tex:J.~Van~Nieuwkoop$^{\rm 142}$,
atlas_authlist.tex:I.~van~Vulpen$^{\rm 107}$,
atlas_authlist.tex:M.C.~van~Woerden$^{\rm 30}$,
atlas_authlist.tex:M.~Vanadia$^{\rm 132a,132b}$,
atlas_authlist.tex:W.~Vandelli$^{\rm 30}$,
atlas_authlist.tex:R.~Vanguri$^{\rm 122}$,
atlas_authlist.tex:A.~Vaniachine$^{\rm 6}$,
atlas_authlist.tex:F.~Vannucci$^{\rm 80}$,
atlas_authlist.tex:G.~Vardanyan$^{\rm 177}$,
atlas_authlist.tex:R.~Vari$^{\rm 132a}$,
atlas_authlist.tex:E.W.~Varnes$^{\rm 7}$,
atlas_authlist.tex:T.~Varol$^{\rm 40}$,
atlas_authlist.tex:D.~Varouchas$^{\rm 80}$,
atlas_authlist.tex:A.~Vartapetian$^{\rm 8}$,
atlas_authlist.tex:K.E.~Varvell$^{\rm 150}$,
atlas_authlist.tex:F.~Vazeille$^{\rm 34}$,
atlas_authlist.tex:T.~Vazquez~Schroeder$^{\rm 87}$,
atlas_authlist.tex:J.~Veatch$^{\rm 7}$,
atlas_authlist.tex:L.M.~Veloce$^{\rm 158}$,
atlas_authlist.tex:F.~Veloso$^{\rm 126a,126c}$,
atlas_authlist.tex:T.~Velz$^{\rm 21}$,
atlas_authlist.tex:S.~Veneziano$^{\rm 132a}$,
atlas_authlist.tex:A.~Ventura$^{\rm 73a,73b}$,
atlas_authlist.tex:D.~Ventura$^{\rm 86}$,
atlas_authlist.tex:M.~Venturi$^{\rm 169}$,
atlas_authlist.tex:N.~Venturi$^{\rm 158}$,
atlas_authlist.tex:A.~Venturini$^{\rm 23}$,
atlas_authlist.tex:V.~Vercesi$^{\rm 121a}$,
atlas_authlist.tex:M.~Verducci$^{\rm 132a,132b}$,
atlas_authlist.tex:W.~Verkerke$^{\rm 107}$,
atlas_authlist.tex:J.C.~Vermeulen$^{\rm 107}$,
atlas_authlist.tex:A.~Vest$^{\rm 44}$,
atlas_authlist.tex:M.C.~Vetterli$^{\rm 142}$$^{,d}$,
atlas_authlist.tex:O.~Viazlo$^{\rm 81}$,
atlas_authlist.tex:I.~Vichou$^{\rm 165}$,
atlas_authlist.tex:T.~Vickey$^{\rm 139}$,
atlas_authlist.tex:O.E.~Vickey~Boeriu$^{\rm 139}$,
atlas_authlist.tex:G.H.A.~Viehhauser$^{\rm 120}$,
atlas_authlist.tex:S.~Viel$^{\rm 15}$,
atlas_authlist.tex:R.~Vigne$^{\rm 62}$,
atlas_authlist.tex:M.~Villa$^{\rm 20a,20b}$,
atlas_authlist.tex:M.~Villaplana~Perez$^{\rm 91a,91b}$,
atlas_authlist.tex:E.~Vilucchi$^{\rm 47}$,
atlas_authlist.tex:M.G.~Vincter$^{\rm 29}$,
atlas_authlist.tex:V.B.~Vinogradov$^{\rm 65}$,
atlas_authlist.tex:I.~Vivarelli$^{\rm 149}$,
atlas_authlist.tex:F.~Vives~Vaque$^{\rm 3}$,
atlas_authlist.tex:S.~Vlachos$^{\rm 10}$,
atlas_authlist.tex:D.~Vladoiu$^{\rm 100}$,
atlas_authlist.tex:M.~Vlasak$^{\rm 128}$,
atlas_authlist.tex:M.~Vogel$^{\rm 32a}$,
atlas_authlist.tex:P.~Vokac$^{\rm 128}$,
atlas_authlist.tex:G.~Volpi$^{\rm 124a,124b}$,
atlas_authlist.tex:M.~Volpi$^{\rm 88}$,
atlas_authlist.tex:H.~von~der~Schmitt$^{\rm 101}$,
atlas_authlist.tex:H.~von~Radziewski$^{\rm 48}$,
atlas_authlist.tex:E.~von~Toerne$^{\rm 21}$,
atlas_authlist.tex:V.~Vorobel$^{\rm 129}$,
atlas_authlist.tex:K.~Vorobev$^{\rm 98}$,
atlas_authlist.tex:M.~Vos$^{\rm 167}$,
atlas_authlist.tex:R.~Voss$^{\rm 30}$,
atlas_authlist.tex:J.H.~Vossebeld$^{\rm 74}$,
atlas_authlist.tex:N.~Vranjes$^{\rm 13}$,
atlas_authlist.tex:M.~Vranjes~Milosavljevic$^{\rm 13}$,
atlas_authlist.tex:V.~Vrba$^{\rm 127}$,
atlas_authlist.tex:M.~Vreeswijk$^{\rm 107}$,
atlas_authlist.tex:R.~Vuillermet$^{\rm 30}$,
atlas_authlist.tex:I.~Vukotic$^{\rm 31}$,
atlas_authlist.tex:Z.~Vykydal$^{\rm 128}$,
atlas_authlist.tex:P.~Wagner$^{\rm 21}$,
atlas_authlist.tex:W.~Wagner$^{\rm 175}$,
atlas_authlist.tex:H.~Wahlberg$^{\rm 71}$,
atlas_authlist.tex:S.~Wahrmund$^{\rm 44}$,
atlas_authlist.tex:J.~Wakabayashi$^{\rm 103}$,
atlas_authlist.tex:J.~Walder$^{\rm 72}$,
atlas_authlist.tex:R.~Walker$^{\rm 100}$,
atlas_authlist.tex:W.~Walkowiak$^{\rm 141}$,
atlas_authlist.tex:C.~Wang$^{\rm 151}$,
atlas_authlist.tex:F.~Wang$^{\rm 173}$,
atlas_authlist.tex:H.~Wang$^{\rm 15}$,
atlas_authlist.tex:H.~Wang$^{\rm 40}$,
atlas_authlist.tex:J.~Wang$^{\rm 42}$,
atlas_authlist.tex:J.~Wang$^{\rm 33a}$,
atlas_authlist.tex:K.~Wang$^{\rm 87}$,
atlas_authlist.tex:R.~Wang$^{\rm 6}$,
atlas_authlist.tex:S.M.~Wang$^{\rm 151}$,
atlas_authlist.tex:T.~Wang$^{\rm 21}$,
atlas_authlist.tex:T.~Wang$^{\rm 35}$,
atlas_authlist.tex:X.~Wang$^{\rm 176}$,
atlas_authlist.tex:C.~Wanotayaroj$^{\rm 116}$,
atlas_authlist.tex:A.~Warburton$^{\rm 87}$,
atlas_authlist.tex:C.P.~Ward$^{\rm 28}$,
atlas_authlist.tex:D.R.~Wardrope$^{\rm 78}$,
atlas_authlist.tex:M.~Warsinsky$^{\rm 48}$,
atlas_authlist.tex:A.~Washbrook$^{\rm 46}$,
atlas_authlist.tex:C.~Wasicki$^{\rm 42}$,
atlas_authlist.tex:P.M.~Watkins$^{\rm 18}$,
atlas_authlist.tex:A.T.~Watson$^{\rm 18}$,
atlas_authlist.tex:I.J.~Watson$^{\rm 150}$,
atlas_authlist.tex:M.F.~Watson$^{\rm 18}$,
atlas_authlist.tex:G.~Watts$^{\rm 138}$,
atlas_authlist.tex:S.~Watts$^{\rm 84}$,
atlas_authlist.tex:B.M.~Waugh$^{\rm 78}$,
atlas_authlist.tex:S.~Webb$^{\rm 84}$,
atlas_authlist.tex:M.S.~Weber$^{\rm 17}$,
atlas_authlist.tex:S.W.~Weber$^{\rm 174}$,
atlas_authlist.tex:J.S.~Webster$^{\rm 31}$,
atlas_authlist.tex:A.R.~Weidberg$^{\rm 120}$,
atlas_authlist.tex:B.~Weinert$^{\rm 61}$,
atlas_authlist.tex:J.~Weingarten$^{\rm 54}$,
atlas_authlist.tex:C.~Weiser$^{\rm 48}$,
atlas_authlist.tex:H.~Weits$^{\rm 107}$,
atlas_authlist.tex:P.S.~Wells$^{\rm 30}$,
atlas_authlist.tex:T.~Wenaus$^{\rm 25}$,
atlas_authlist.tex:T.~Wengler$^{\rm 30}$,
atlas_authlist.tex:S.~Wenig$^{\rm 30}$,
atlas_authlist.tex:N.~Wermes$^{\rm 21}$,
atlas_authlist.tex:M.~Werner$^{\rm 48}$,
atlas_authlist.tex:P.~Werner$^{\rm 30}$,
atlas_authlist.tex:M.~Wessels$^{\rm 58a}$,
atlas_authlist.tex:J.~Wetter$^{\rm 161}$,
atlas_authlist.tex:K.~Whalen$^{\rm 116}$,
atlas_authlist.tex:A.M.~Wharton$^{\rm 72}$,
atlas_authlist.tex:A.~White$^{\rm 8}$,
atlas_authlist.tex:M.J.~White$^{\rm 1}$,
atlas_authlist.tex:R.~White$^{\rm 32b}$,
atlas_authlist.tex:S.~White$^{\rm 124a,124b}$,
atlas_authlist.tex:D.~Whiteson$^{\rm 163}$,
atlas_authlist.tex:F.J.~Wickens$^{\rm 131}$,
atlas_authlist.tex:W.~Wiedenmann$^{\rm 173}$,
atlas_authlist.tex:M.~Wielers$^{\rm 131}$,
atlas_authlist.tex:P.~Wienemann$^{\rm 21}$,
atlas_authlist.tex:C.~Wiglesworth$^{\rm 36}$,
atlas_authlist.tex:L.A.M.~Wiik-Fuchs$^{\rm 21}$,
atlas_authlist.tex:A.~Wildauer$^{\rm 101}$,
atlas_authlist.tex:H.G.~Wilkens$^{\rm 30}$,
atlas_authlist.tex:H.H.~Williams$^{\rm 122}$,
atlas_authlist.tex:S.~Williams$^{\rm 107}$,
atlas_authlist.tex:C.~Willis$^{\rm 90}$,
atlas_authlist.tex:S.~Willocq$^{\rm 86}$,
atlas_authlist.tex:A.~Wilson$^{\rm 89}$,
atlas_authlist.tex:J.A.~Wilson$^{\rm 18}$,
atlas_authlist.tex:I.~Wingerter-Seez$^{\rm 5}$,
atlas_authlist.tex:F.~Winklmeier$^{\rm 116}$,
atlas_authlist.tex:B.T.~Winter$^{\rm 21}$,
atlas_authlist.tex:M.~Wittgen$^{\rm 143}$,
atlas_authlist.tex:J.~Wittkowski$^{\rm 100}$,
atlas_authlist.tex:S.J.~Wollstadt$^{\rm 83}$,
atlas_authlist.tex:M.W.~Wolter$^{\rm 39}$,
atlas_authlist.tex:H.~Wolters$^{\rm 126a,126c}$,
atlas_authlist.tex:B.K.~Wosiek$^{\rm 39}$,
atlas_authlist.tex:J.~Wotschack$^{\rm 30}$,
atlas_authlist.tex:M.J.~Woudstra$^{\rm 84}$,
atlas_authlist.tex:K.W.~Wozniak$^{\rm 39}$,
atlas_authlist.tex:M.~Wu$^{\rm 55}$,
atlas_authlist.tex:M.~Wu$^{\rm 31}$,
atlas_authlist.tex:S.L.~Wu$^{\rm 173}$,
atlas_authlist.tex:X.~Wu$^{\rm 49}$,
atlas_authlist.tex:Y.~Wu$^{\rm 89}$,
atlas_authlist.tex:T.R.~Wyatt$^{\rm 84}$,
atlas_authlist.tex:B.M.~Wynne$^{\rm 46}$,
atlas_authlist.tex:S.~Xella$^{\rm 36}$,
atlas_authlist.tex:D.~Xu$^{\rm 33a}$,
atlas_authlist.tex:L.~Xu$^{\rm 33b}$$^{,ak}$,
atlas_authlist.tex:B.~Yabsley$^{\rm 150}$,
atlas_authlist.tex:S.~Yacoob$^{\rm 145a}$,
atlas_authlist.tex:R.~Yakabe$^{\rm 67}$,
atlas_authlist.tex:M.~Yamada$^{\rm 66}$,
atlas_authlist.tex:Y.~Yamaguchi$^{\rm 118}$,
atlas_authlist.tex:A.~Yamamoto$^{\rm 66}$,
atlas_authlist.tex:S.~Yamamoto$^{\rm 155}$,
atlas_authlist.tex:T.~Yamanaka$^{\rm 155}$,
atlas_authlist.tex:K.~Yamauchi$^{\rm 103}$,
atlas_authlist.tex:Y.~Yamazaki$^{\rm 67}$,
atlas_authlist.tex:Z.~Yan$^{\rm 22}$,
atlas_authlist.tex:H.~Yang$^{\rm 33e}$,
atlas_authlist.tex:H.~Yang$^{\rm 173}$,
atlas_authlist.tex:Y.~Yang$^{\rm 151}$,
atlas_authlist.tex:W-M.~Yao$^{\rm 15}$,
atlas_authlist.tex:Y.~Yasu$^{\rm 66}$,
atlas_authlist.tex:E.~Yatsenko$^{\rm 5}$,
atlas_authlist.tex:K.H.~Yau~Wong$^{\rm 21}$,
atlas_authlist.tex:J.~Ye$^{\rm 40}$,
atlas_authlist.tex:S.~Ye$^{\rm 25}$,
atlas_authlist.tex:I.~Yeletskikh$^{\rm 65}$,
atlas_authlist.tex:A.L.~Yen$^{\rm 57}$,
atlas_authlist.tex:E.~Yildirim$^{\rm 42}$,
atlas_authlist.tex:K.~Yorita$^{\rm 171}$,
atlas_authlist.tex:R.~Yoshida$^{\rm 6}$,
atlas_authlist.tex:K.~Yoshihara$^{\rm 122}$,
atlas_authlist.tex:C.~Young$^{\rm 143}$,
atlas_authlist.tex:C.J.S.~Young$^{\rm 30}$,
atlas_authlist.tex:S.~Youssef$^{\rm 22}$,
atlas_authlist.tex:D.R.~Yu$^{\rm 15}$,
atlas_authlist.tex:J.~Yu$^{\rm 8}$,
atlas_authlist.tex:J.M.~Yu$^{\rm 89}$,
atlas_authlist.tex:J.~Yu$^{\rm 114}$,
atlas_authlist.tex:L.~Yuan$^{\rm 67}$,
atlas_authlist.tex:S.P.Y.~Yuen$^{\rm 21}$,
atlas_authlist.tex:A.~Yurkewicz$^{\rm 108}$,
atlas_authlist.tex:I.~Yusuff$^{\rm 28}$$^{,al}$,
atlas_authlist.tex:B.~Zabinski$^{\rm 39}$,
atlas_authlist.tex:R.~Zaidan$^{\rm 63}$,
atlas_authlist.tex:A.M.~Zaitsev$^{\rm 130}$$^{,ab}$,
atlas_authlist.tex:J.~Zalieckas$^{\rm 14}$,
atlas_authlist.tex:A.~Zaman$^{\rm 148}$,
atlas_authlist.tex:S.~Zambito$^{\rm 57}$,
atlas_authlist.tex:L.~Zanello$^{\rm 132a,132b}$,
atlas_authlist.tex:D.~Zanzi$^{\rm 88}$,
atlas_authlist.tex:C.~Zeitnitz$^{\rm 175}$,
atlas_authlist.tex:M.~Zeman$^{\rm 128}$,
atlas_authlist.tex:A.~Zemla$^{\rm 38a}$,
atlas_authlist.tex:K.~Zengel$^{\rm 23}$,
atlas_authlist.tex:O.~Zenin$^{\rm 130}$,
atlas_authlist.tex:T.~\v{Z}eni\v{s}$^{\rm 144a}$,
atlas_authlist.tex:D.~Zerwas$^{\rm 117}$,
atlas_authlist.tex:D.~Zhang$^{\rm 89}$,
atlas_authlist.tex:F.~Zhang$^{\rm 173}$,
atlas_authlist.tex:H.~Zhang$^{\rm 33c}$,
atlas_authlist.tex:J.~Zhang$^{\rm 6}$,
atlas_authlist.tex:L.~Zhang$^{\rm 48}$,
atlas_authlist.tex:R.~Zhang$^{\rm 33b}$,
atlas_authlist.tex:X.~Zhang$^{\rm 33d}$,
atlas_authlist.tex:Z.~Zhang$^{\rm 117}$,
atlas_authlist.tex:X.~Zhao$^{\rm 40}$,
atlas_authlist.tex:Y.~Zhao$^{\rm 33d,117}$,
atlas_authlist.tex:Z.~Zhao$^{\rm 33b}$,
atlas_authlist.tex:A.~Zhemchugov$^{\rm 65}$,
atlas_authlist.tex:J.~Zhong$^{\rm 120}$,
atlas_authlist.tex:B.~Zhou$^{\rm 89}$,
atlas_authlist.tex:C.~Zhou$^{\rm 45}$,
atlas_authlist.tex:L.~Zhou$^{\rm 35}$,
atlas_authlist.tex:L.~Zhou$^{\rm 40}$,
atlas_authlist.tex:N.~Zhou$^{\rm 163}$,
atlas_authlist.tex:C.G.~Zhu$^{\rm 33d}$,
atlas_authlist.tex:H.~Zhu$^{\rm 33a}$,
atlas_authlist.tex:J.~Zhu$^{\rm 89}$,
atlas_authlist.tex:Y.~Zhu$^{\rm 33b}$,
atlas_authlist.tex:X.~Zhuang$^{\rm 33a}$,
atlas_authlist.tex:K.~Zhukov$^{\rm 96}$,
atlas_authlist.tex:A.~Zibell$^{\rm 174}$,
atlas_authlist.tex:D.~Zieminska$^{\rm 61}$,
atlas_authlist.tex:N.I.~Zimine$^{\rm 65}$,
atlas_authlist.tex:C.~Zimmermann$^{\rm 83}$,
atlas_authlist.tex:S.~Zimmermann$^{\rm 48}$,
atlas_authlist.tex:Z.~Zinonos$^{\rm 54}$,
atlas_authlist.tex:M.~Zinser$^{\rm 83}$,
atlas_authlist.tex:M.~Ziolkowski$^{\rm 141}$,
atlas_authlist.tex:L.~\v{Z}ivkovi\'{c}$^{\rm 13}$,
atlas_authlist.tex:G.~Zobernig$^{\rm 173}$,
atlas_authlist.tex:A.~Zoccoli$^{\rm 20a,20b}$,
atlas_authlist.tex:M.~zur~Nedden$^{\rm 16}$,
atlas_authlist.tex:G.~Zurzolo$^{\rm 104a,104b}$,
atlas_authlist.tex:L.~Zwalinski$^{\rm 30}$.
atlas_authlist.tex:$^{16}$ Department of Physics, Humboldt University, Berlin, Germany\\
atlas_authlist.tex:$^{18}$ School of Physics and Astronomy, University of Birmingham, Birmingham, United Kingdom\\
atlas_authlist.tex:$^{21}$ Physikalisches Institut, University of Bonn, Bonn, Germany\\
atlas_authlist.tex:$^{31}$ Enrico Fermi Institute, University of Chicago, Chicago IL, United States of America\\
atlas_authlist.tex:$^{34}$ Laboratoire de Physique Corpusculaire, Clermont Universit{\'e} and Universit{\'e} Blaise Pascal and CNRS/IN2P3, Clermont-Ferrand, France\\
atlas_authlist.tex:$^{42}$ DESY, Hamburg and Zeuthen, Germany\\
atlas_authlist.tex:$^{43}$ Institut f{\"u}r Experimentelle Physik IV, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
atlas_authlist.tex:$^{44}$ Institut f{\"u}r Kern-{~}und Teilchenphysik, Technische Universit{\"a}t Dresden, Dresden, Germany\\
atlas_authlist.tex:$^{48}$ Fakult{\"a}t f{\"u}r Mathematik und Physik, Albert-Ludwigs-Universit{\"a}t, Freiburg, Germany\\
atlas_authlist.tex:$^{52}$ II Physikalisches Institut, Justus-Liebig-Universit{\"a}t Giessen, Giessen, Germany\\
atlas_authlist.tex:$^{54}$ II Physikalisches Institut, Georg-August-Universit{\"a}t, G{\"o}ttingen, Germany\\
atlas_authlist.tex:$^{58}$ $^{(a)}$ Kirchhoff-Institut f{\"u}r Physik, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg; $^{(b)}$ Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg; $^{(c)}$ ZITI Institut f{\"u}r technische Informatik, Ruprecht-Karls-Universit{\"a}t Heidelberg, Mannheim, Germany\\
atlas_authlist.tex:$^{59}$ Faculty of Applied Information Science, Hiroshima Institute of Technology, Hiroshima, Japan\\
atlas_authlist.tex:$^{83}$ Institut f{\"u}r Physik, Universit{\"a}t Mainz, Mainz, Germany\\
atlas_authlist.tex:$^{100}$ Fakult{\"a}t f{\"u}r Physik, Ludwig-Maximilians-Universit{\"a}t M{\"u}nchen, M{\"u}nchen, Germany\\
atlas_authlist.tex:$^{101}$ Max-Planck-Institut f{\"u}r Physik (Werner-Heisenberg-Institut), M{\"u}nchen, Germany\\
atlas_authlist.tex:$^{113}$ Homer L. Dodge Department of Physics and Astronomy, University of Oklahoma, Norman OK, United States of America\\
atlas_authlist.tex:$^{124}$ $^{(a)}$ INFN Sezione di Pisa; $^{(b)}$ Dipartimento di Fisica E. Fermi, Universit{\`a} di Pisa, Pisa, Italy\\
atlas_authlist.tex:$^{141}$ Fachbereich Physik, Universit{\"a}t Siegen, Siegen, Germany\\
atlas_authlist.tex:$^{144}$ $^{(a)}$ Faculty of Mathematics, Physics {\&} Informatics, Comenius University, Bratislava; $^{(b)}$ Department of Subnuclear Physics, Institute of Experimental Physics of the Slovak Academy of Sciences, Kosice, Slovak Republic\\
atlas_authlist.tex:$^{174}$ Fakult{\"a}t f{\"u}r Physik und Astronomie, Julius-Maximilians-Universit{\"a}t, W{\"u}rzburg, Germany\\
atlas_authlist.tex:$^{175}$ Fachbereich C Physik, Bergische Universit{\"a}t Wuppertal, Wuppertal, Germany\\
atlas_authlist.tex:$^{177}$ Yerevan Physics Institute, Yerevan, Armenia\\
bChi_diagrams.tex:%\put(15,230){$\dmCN = 5, 20\ \mathrm{GeV}$}
bChi_diagrams.tex:%\put(15,230){$\Delta m \left(\tone, \chipm \right) = 10\ \mathrm{GeV}$}
bChi_diagrams.tex:\caption{Scenarios considered for the $\tone \rightarrow b \chipm$ decay: (a) $\dmCN = 5, 20\ \mathrm{GeV}$; (b) Fixed chargino mass; (c) $m_{\chipm} = 2 m_{\neut}$; (d) $\Delta m \left(\tone, \chipm \right) = 10\ \mathrm{GeV}$. A thicker red line indicates that the particle mass is kept fixed in the corresponding model}
charm.tex:If the difference in mass between the stop and the neutralino is smaller than the $W$ boson mass, then the only possible decay channels are $\stop \rightarrow \neut c$ or $\stop \rightarrow W^* b$, where the decay products of the off-shell $W^*$ would,  in general, be soft. This analysis~\cite{Aad:2014nra} has defined two sets of signal regions, both optimised for the $\stop \rightarrow \neut c$ decay. A common preselection requires the presence of a high-\pt\ jet, large \etmiss and applies a lepton veto. The first set of signal regions named \stopCharm-M, targets scenarios with the stop mass almost degenerate with the neutralino mass, and applies a selection that exploits a monojet-like signature arising from the presence of an ISR jet. Three different signal regions have been designed, characterised by increasing thresholds on the leading jet \pt\ and \etmiss. The second set of signal regions, named \stopCharm-C, targets less compressed scenarios, and exploits the presence of jets originating from the fragmentation of $c$-quarks in the final state. A dedicated $c$-tagging algorithm was  used to reject the dominant SM background processes arising mostly from \ttbar\  and $Z\rightarrow \nu \bar{\nu}$ (produced in association with heavy-flavour jets) production. As in the case of the \stopCharm-M signal regions, different thresholds on the leading jet \pt\ and on \etmiss are used to identify a looser and a tighter \stopCharm-C region.  
detector.tex:beam pipe. The pseudorapidity is defined in terms of the polar angle $\theta$ as $\eta=-\ln\tan(\theta/2)$. The
detector.tex:distance~$\mathrm{\Delta} R$ in the $\eta$--$\phi$ space is defined as
detector.tex:$\mathrm{\Delta} R = \sqrt{(\mathrm{\Delta}\eta)^2+(\mathrm{\Delta}\phi)^2}$.} range $|\eta| < 2.5$.
exp_sig.tex:Final states from compressed stop & \multirow{2}{*}{\stopCharm} & M1-3  & $\tone/\bone \rightarrow \mathrm{anything}$ with $m_{\tone} \sim m_{\neut}$\\
exp_sig.tex:at intermediate \mtTwoll~\ref{sec:WWlike} & &  & $\tone \rightarrow b \ell \nu \neut$ (three- and four-body decays) \\
general.tex:For each SR, multiple control regions (CR) are defined: they are used to constrain the normalisation of the most relevant SM production processes and to validate the MC predictions of the shapes of distributions of the kinematic variables used in the analysis. The event selection of the CRs is mutually exclusive with that of the SRs. It is, however, chosen to be as close as possible to that of the signal region while keeping the signal contamination small, and such that the event yield is dominated by one specific background process. 
general.tex:A likelihood function is built as the product of Poisson probability functions, describing the observed and expected number of events in the control and signal regions. The observed numbers of events in the various CRs and SRs are used in a combined profile likelihood fit~\cite{Cowan:2010js} to determine the expected SM background yields for each of the SRs. Systematic uncertainties are treated as nuisance parameters in the fit and are constrained with Gaussian functions with standard deviation equal to their value. The fit procedure takes into account correlations in the yield predictions between different regions due to common background normalisation parameters and systematic uncertainties, as well as  contamination from SUSY signal events, when a particular model is considered for exclusion.
interpretations.tex:Several analyses have sensitivity in this region of the $m_{\tone} - m_{\neut}$ plane. The monojet-like signal regions (\stopCharm-M1-3) dominate the sensitivity in the region with $\DMstopN \gtrsim m_b$, regardless of the decay of the stop pair, which goes undetected: their selection is based on the presence of an initial-state radiation (ISR) jet recoiling against the stop-pair system, which is assumed to be invisible.  At larger values of $\DMstopN$, signal regions requiring the presence of a $c$-tagged jet (\stopCharm-C1-2) complement the monojet-like signal regions by targeting the $\tone\rightarrow c \neut$ decay. Limits on four-body decays can be set using signal regions which include low transverse momentum electrons and muons (\stopOneLep-bCa\_low and \WWlike).
interpretations.tex:\input{stop_4body_charm}
interpretations.tex:In this case, the neutralinos are produced with low $\pt$, and the kinematic properties of the signal are similar to those of SM $\ttbar$ production. Exclusion limits in this region were obtained by two analyses performing precision SM measurements. The first one is the measurement of the \ttbar\ inclusive production cross section $\sigma_{\ttbar}$. Limits on $\tone$ pair production were already set in Ref.~\cite{Aad:2014kva}, which measured $\sigma_{\ttbar}$ in the different-flavour, opposite-sign channel $e\mu$. They were derived assuming a $\tone$ decay into an on-shell top quark, $\tone \rightarrow t \neut$. An extension of the limits into the three-body stop decay is discussed in Appendix~\ref{sec:published_SR}. For a massless neutralino, the analysis excludes stop masses from about 150 GeV to about $\mtop$. The limit deteriorates for higher neutralino masses, mainly because of the softer \bjet\ spectrum and the consequent  loss in acceptance. 
interpretations.tex:The second analysis considered is that of the top quark spin correlation (\spinCorr) which considers SM $\ttbar$ production with decays to final states containing two leptons (electrons or muons). The shape and normalisation of the distribution of the azimuthal angle between the two leptons is sensitive to the spin of the produced particles, hence it allows the analysis to differentiate between stop pair and $\ttbar$ production. The limit obtained is shown in the bottom middle (dark orange) of the inset of Figure~\ref{fig:tNsummary}.  A small region of $\DMstopN \approx 180$~GeV is excluded with this measurement assuming a small neutralino mass.
interpretations.tex:    \caption{Summary of the ATLAS Run 1 searches for direct stop pair production in models where the decay mode $\tone \rightarrow b \chipm$ with $\chipm\rightarrow W^{*} \neut$ is assumed with a branching ratio of 100\%. Various hypotheses on the $\tone$, $\chipm$, and $\neut$ mass hierarchy are used. Exclusion limits at 95\% CL are shown in the $\tone-\neut$ mass plane. The dashed and solid lines show the expected and observed limits, respectively, including all uncertainties except the theoretical signal cross-section uncertainty (PDF and scale). Wherever not superseded by any $\sqrt{s}=8$ TeV analysis, results obtained by analyses using 4.7 \ifb\ of proton--proton collision data taken at $\sqrt{s} = 7$ TeV are also shown, with the corresponding reference. The four plots correspond to interpretations of (a) the \sbottom\ and \stopOneLep\ soft-lepton analyses in two scenarios ($\dmCN = 5\ \GeV$ in light green and  $\dmCN = 20\ \mathrm{GeV}$ in dark green), for a total of four limits; (b) the \sbottom, \stopOneLep\ and \stopTwoLep\ analyses in scenarios with a fixed chargino mass $m_{\chipm} = 106$~GeV (dark green) and  $m_{\chipm} = 150$ GeV (light green); (c) the \stopOneLep\ and \stopTwoLep\ analyses in scenarios with $m_{\chipm} = 2 m_{\neut}$; (d) interpretations of the \stopOneLep, \stopTwoLep\ and \WWlike\ analyses in senarios with $\Delta m \left(\tone, \chipm \right) = 10\ \mathrm{GeV}$. }
interpretations.tex:If additional particles beside the stop and the lightest neutralino take part in the stop decay, the stop phenomenology quickly becomes complex. Even if the chargino is the only other relevant SUSY particle, the stop phenomenology depends on the chargino mass, on the stop left-right mixing, and on the composition of the neutralino and chargino in terms of bino, wino and higgsino states.
interpretations.tex:\paragraph{$\dmCN =  5, 20$ GeV.} This scenario assumes that the difference in mass between the lightest chargino and the neutralino is small (Figure~\ref{fig:bCsummary_dmCN}). {\color{red}{This is a rather common feature of models where, for example, the LSP has a large wino or higgsino component}}. Two hypotheses have been considered, with $\dmCN =  5$ GeV and $\dmCN = 20$ GeV. For both, the complete decay chain is $\tone \rightarrow b \chipm \rightarrow b f f' \neut$, where the transverse momenta of the fermions $f$ and $f'$ depend on $\dmCN$ and on the stop mass, given the dependency on the chargino boost. If $\dmCN = 5$ GeV, the fermions have  momenta too low to be efficiently reconstructed. The observed final state then consists of two \bjets and $\met$. This final state is the direct target of the \sbottom\ signal regions. For $\dmCN = 20$ GeV, the signal efficiencies of the \sbottom\ signal regions decrease because of the lepton and jet veto applied. The \stopOneLep\ signal regions with soft leptons, instead, gain in sensitivity, profiting from the higher transverse momentum of the fermions from the off-shell $W$ decay produced in the chargino decay.
interpretations.tex:\paragraph{$m_{\chipm} = 2 m_{\neut}$.} Inspired by gauge-universality considerations, the third scenario (Figure~\ref{fig:bCsummary_univ}) is characterised by a relatively large $\dmCN$. The \stopTwoLep\ signal regions dominate the sensitivity for $m_{\tone} \sim m_{\chipm}$. The sensitivity of the dedicated \stopOneLep-bC is dominant in a large region of the plane, and determines the exclusion reach for moderate to large values of $\DMstopN$.
introduction.tex:In a theory with broken supersymmetry (SUSY)~\cite{Miyazawa:1966,Ramond:1971gb,Golfand:1971iw,Neveu:1971rx,Neveu:1971iv,Gervais:1971ji,Volkov:1973ix,Wess:1973kz,Wess:1974tw}, the mass scale of the supersymmetric particles is undetermined. However, for SUSY to provide a solution to the hierarchy problem~\cite{Weinberg:1975gm,Gildener:1976ai,Weinberg:1979bn,Susskind:1978ms} some of the new SUSY particles masses are typically required to be below about one TeV~\cite{Barbieri:1987fn,deCarlos:1993yy}, hence they could be within the reach of the LHC. 
introduction.tex: The $\tright$ and $\tleft$ components mix to form the mass eigenstates $\tone$ and $\ttwo$, $\tone$ being defined as the lighter of the two. The scalar superpartner of the left-handed chiral component of the bottom quark ($\bleft$) belongs to the same weak isospin doublet as the $\tleft$, hence they usually share the same supersymmetry-breaking mass parameter: a light stop can therefore imply the existence of a light scalar bottom. The lightest sbottom mass eigenstate is referred to as $\bone$. 
introduction.tex:during Run 1 of the LHC.\footnote{The analysis exploiting the measurement of the \ttbar\  cross section discussed in this paper also uses 4.7 \ifb\ of proton-proton collisions at $\sqrt{s} = 7$ TeV.} The third-generation squarks are assumed to decay to the stable lightest supersymmetric particle (LSP) directly or through one or more intermediate stages. The analyses considered are those previously published by the ATLAS collaboration on the topic, together with new ones designed to increase the sensitivity to scenarios not optimally covered so far. A wide range of SUSY scenarios are studied by combining different analyses to improve the global sensitivity. 
introduction.tex:For the sake of brevity, the body of the paper provides no details of the ATLAS detector and object reconstruction, of the analyses used in the limit derivation, or of how the signal Monte Carlo simulation samples were generated. However, a comprehensive set of appendices is provided to supply additional information to the interested reader. Appendix~\ref{sec:detector} briefly summarises the layout of the ATLAS detector and the general principles used in the reconstruction of electrons, muons, jets, jets containing $b$-hadrons (\bjets), and the missing transverse momentum vector $\bf{p}_{\mathrm{T}}^{\mathrm{miss}}$ (whose magnitude is referred to as $\etmiss$). Appendix~\ref{sec:SRs} discusses the analyses used to derive the exclusion limits presented in Sections~\ref{sec:interpretations} and \ref{sec:pMSSM}. The analyses that have already been published are only briefly reviewed, while those presented for the first time in this paper are discussed in detail. Appendix~\ref{sec:01lepCombine} provides further details of a combination of analyses which is performed for the first time in this paper. Finally, Appendix~\ref{sec:signal_generation} provides details about the generation and simulation of the signal Monte Carlo samples used to derive the limits presented.
newSR.tex:\subsubsection{Final states with two leptons at intermediate values of \mtTwoll (\WWlike)}
objecteventsel.tex:information~\cite{ATLAS-CONF-2012-043}; this algorithm is based on a
pMSSM.tex:\item[-] No flavour-changing neutral currents. This is implemented by requiring that the matrices for the sfermion masses and trilinear couplings are diagonal.   
pMSSM.tex:{\color{red}{A full assessment of the ATLAS sensitivity to a scan of the 19-parameters space has been performed in Ref.~\cite{Aad:2015baa}. Here, a set of additional hypotheses are made, to focus on the sensitivity to a specific, well-motivated set of models with enhanced third generation squark production:}} 
pMSSM.tex:\item[-] The common masses of the first- and second-generation squarks have been set to a multi-TeV scale, making these quarks irrelevant for the processes studied at the energies investigated in this paper. This choice is motivated by the absence of any signal from squark or gluino production in dedicated SUSY searches performed by the ATLAS~\cite{Aad:2014wea,Aad:2015mia,Aad:2013wta,Aad:2014pda,Aad:2014lra,Aad:2015gna} and CMS~\cite{Khachatryan:2015vra,Chatrchyan:2013fea,Khachatryan:2015pwa,CMS:2014dpa,Chatrchyan:2014lfa,Chatrchyan:2013iqa,Chatrchyan:2013wxa,Chatrchyan:2013lya} collaborations. 
pMSSM.tex:These assumptions reduce the number of additional free parameters of the model to the mass parameters of the electroweak sector ($\mu, M_1, M_2$) and two of the three third-generation squark mass parameters ($\mqlthree, \mtR, \mbR$). All the assumptions made either have a solid experimental basis, or are intended to simplify the interpretation in terms of direct production of stops and sbottoms (as, for example, the assumption on the slepton mass parameters).  
pMSSM.tex:Three types of models have been chosen, that, by implementing in different ways  constraints arising from naturalness arguments and the dark-matter relic density measurement, further reduce the number of parameters to be scanned over. They are described below, and summarised in Table~\ref{tab:pMSSM_models} together with additional information on the most relevant production and decay channels.
pMSSM.tex:\paragraph{Naturalness-inspired pMSSM:}The model is inspired by naturalness criteria, which require a value of $\mu$ in the range of a few hundred GeV, favour stop masses below one TeV, place weak constraints on the gluino mass and give no constraints on the mass of other SUSY particles~\cite{Papucci:2011wy}. The exclusion limits are determined as a  function of the higgsino mass parameter $\mu$ and the left-handed squark mass parameter $\mqlthree$. {\color{red}{The parameter $\mqlthree$ is scanned in the range $350 \ \GeV < \mqlthree < 900\ \GeV$. The parameter $\mu$ is scanned in the range $100 \ \GeV < \mu < \mqlthree -150\ \GeV$, the lower bound being determined by limits on the chargino mass arising from LEP~\cite{lep2, Heister:2003zk, Abdallah:2003xe, Acciarri:1999km, Abbiendi:2003sc}.}} The right-handed stop mass parameter $\mtR$ and the stop mixing parameter $X_t$ are determined by choosing the maximal mixing scenario $X_t/M_S = \sqrt{6}$ and by the requirement of having a Higgs boson mass of about 125 GeV. The other squark and slepton masses, as well as the bino mass parameter $M_1$, are set to 3 TeV. The wino mass parameter $M_2$ is set such that $M_2 = 3\mu$. The gluino mass parameter $M_3$ is set to 1.7 TeV.
pMSSM.tex: \paragraph{Well-tempered neutralino pMSSM:} The models are designed to loosely satisfy dark-matter thermal-relic density constraints ($0.09 < \Omega_{\mathrm{c}} h^2 < 0.15$, where $h$ is the Hubble constant), while keeping fine tuning (defined as in Ref.~\cite{CahillRowley:2012rv}) to less than 1\%. The exclusion limits are determined as a function of $M_1$ and $\mqlthree$, or $M_1$ and $\mtR$, with $\mu \sim- M_1$ in both cases to satisfy the dark-matter constraints through the presence of well-tempered neutralinos~\cite{ArkaniHamed:2006mb}. The constraints on the Higgs boson mass are satisfied in a way similar to the naturalness-inspired pMSSM model above. All other parameters are the same as in the naturalness-inspired pMSSM model. These models tend to have three neutralinos and two charginos with masses lower than $\tone$ or $\bone$, giving rise to a diverse phenomenology. 
pMSSM.tex:ensures that direct gluino production is highly suppressed compared to third-generation squark production. Two sets of models have been defined: in the first one, $\mu$ and the right-handed sbottom mass parameter $\mbR$ are scanned while keeping $M_2 = \mu$, $\mqlthree = 1.2$ TeV, $\mtR = 1.6$ TeV; in the second one, $\mu$ and $\mqlthree$ are scanned while keeping $M_2 = 1$ TeV, $\mbR = 3$ TeV, $\mtR = 2$ TeV. The former is dominated by sbottom pair production, while both sbottom and stop pair production are relevant for the latter. Stop mixing parameters are chosen with maximal mixing to satisfy Higgs boson mass constraints. 
pMSSM.tex:Exclusion limits for these pMSSM models are determined by combining many of the SRs defined for the searches discussed in this paper (\stopZeroLep, \stopOneLep, \TBM,\footnote{The \TBM\ signal region, discussed in detail in Appendix~\ref{sec:tbmet}, implement a one-lepton selection, designed to be sensitive to final states containing a top quark, a $b$-quark and $\etmiss$. It complements the selections of the $\stopZeroLep$ and $\stopOneLep$ signal regions targeting $tt\etmiss$ final states.} \stopTwo, \threeb, \stopCharm). For each set of parameters the individual 95\% CL expected limit is evaluated. The combined exclusion contour is determined by choosing, for each model point, the signal region having the smallest expected \cls\ value of the test statistic for the signal-plus-background hypothesis.
pMSSM.tex: The signal regions that dominate the sensitivity are the \TBM, \stopZeroLep-SRC1 and  \stopOneLep-bCd\_bulk at low values of $\mqlthree$,  and \TBM, \stopZeroLep-SRA1, \stopZeroLep-SRA2 and \stopOneLep-tNbC\_mix at intermediate and high values of $\mqlthree$. The excluded region for models with $\mqlthree \sim 900$ GeV and $\mu \sim 150$ GeV is due to the saturation of $m_{\tone}$ at high $\mqlthree$ values: to satisfy the Higgs boson mass constraint requires $M_S \sim 800$ GeV, hence $m_{\tone}$ at  $\mqlthree \sim 900$ \GeV\ is smaller than that at $\mqlthree \sim 800$ \GeV. {\color{red}{The large fluctuations of the observed limit with respect to the expected one are due to transitions between different signal regions providing the best expected exclusion in different regions of the plane.}}
pMSSM.tex:Figures~\ref{fig:DM_mql3} and \ref{fig:DM_mtR} show the exclusion limit obtained for the set of pMSSM models with well-tempered neutralinos as a function of $\mqlthree$ and $\mtR$, respectively. {\color{red}{In both cases, the exclusion is largely dominated by the \stopZeroLep\ analysis. For Figure~\ref{fig:DM_mql3}, the signal region dominating the sensitivity at low $\mqlthree$ is \stopZeroLep-SRC1, while at higher  $\mqlthree$ values \stopZeroLep-SRA1 and \stopZeroLep-SRA2 dominate the sensitivity. The drop in sensitivity at $\mqlthree = 410\ \GeV$, $M_1 = 260\ \GeV$ is due to the opening of the $\tone \rightarrow t \neuttwo$ and $\tone \rightarrow t \neutthree$ transition, kinematically suppressed for smaller values of  the difference $\mqlthree - M_1$. Such decays introduce more intermediate states in the decay, effectively reducing the transverse momenta of the final state objects. The large fluctuations of the observed limit are again due to transitions between different signal regions. For Figure~\ref{fig:DM_mtR}, the sensitivity is entirely dominated by the various \stopZeroLep-SRC.  The difference in sensitivity between these two scenarios is due to the presence of both a  stop and a sbottom for small $\mqlthree$, while only a stop is present for low values of $\mtR$}}. 
phenomenology.tex: The cross section for direct stop pair production in proton--proton collisions at $\sqrt{s} = 8$ TeV as a function of the stop mass as calculated with \prospino~\cite{prospino,Kramer:2012bx} is shown in Figure~\ref{fig:stopcrosssec}. It is calculated to next-to-leading order accuracy in the strong coupling constant, adding the resummation of soft gluon emission at next-to-leading-logarithmic accuracy (NLO+NLL)~\cite{Beenakker:1997ut,Beenakker:2010nq,Beenakker:2011fu}. In this paper, the nominal cross section and its uncertainty are taken from an envelope of cross-section predictions using different parton distribution function (PDF) sets and factorisation and renormalisation scales described in Ref.~\cite{Kramer:2012bx}. The difference in cross section between the sbottom and stop pair production is known to be small~\cite{Beenakker:2010nq}, hence the values of Figure~\ref{fig:stopcrosssec} are used for both.
phenomenology.tex:\draw [->] (0,0) -- (6.5,0) node [below left]  {\small $\mathrm{m}(\tone)$ [GeV]};
phenomenology.tex:\draw [->] (0,0) -- (0,4) node [above,rotate = 90] {\small $\mathrm{m}(\neut)$ [GeV]};	
phenomenology.tex: A significantly more complex phenomenology has to be considered for the stop, depending on its mass and on the $\neut$ mass. Figure~\ref{fig:stop_pheno} shows the three main regions in the $m_{\tone}$--$m_{\neut}$ plane that are taken into account. They are identified by different values of $\DMstopN = m_{\tone}$-$m_{\neut}$. In the region where $\DMstopN > \mtop$, the favoured decay is $\tone \rightarrow t \neut$ (Figure~\ref{fig:tN1tN1}). The region where $m_W + m_b < \DMstopN <  \mtop$ is characterised by the three-body decay\footnote{In scenarios that depart from the minimal flavour violation assumption, flavour-changing decays like $\tone \rightarrow c \neut$ or $\tone \rightarrow u \neut$ could have a significant branching ratio up to $\DMstopN \sim 100$ GeV \cite{Grober:2015fia}.} ($\tone \rightarrow Wb \neut$ through an off-shell top quark, Figure~\ref{fig:threebody}). The region where the value of $\DMstopN$ drops below $m_W + m_b$, sees the four-body decay $\tone \rightarrow b f f' \neut$, (where $f$ and $f'$ indicate generic fermions coming from the decay of an off-shell $W$ boson, Figure~\ref{fig:fourbody}) competing with the flavour-changing decay\footnote{The decay $\tone \rightarrow u \neut$, in the assumption of minimal flavour violation~\cite{D'Ambrosio:2002ex}, is further suppressed with respect to $\tone \rightarrow c \neut$ by corresponding factors of the CKM matrix.}  $\tone \rightarrow c \neut$ of Figure~\ref{fig:cN1cN1}; the dominant decay depends on the details of the supersymmetric model chosen~\cite{Grober:2014aha}.
phenomenology.tex:Two types of SUSY models are used to interpret  the results in terms of exclusion limits. The simplified model approach assumes that either a stop or a sbottom pair is produced and that they decay into well-defined final states, involving one or two decay channels. 
phenomenology.tex:More complete phenomenological minimal supersymmetric extensions of the Standard Model (pMSSM in the following~\cite{Djouadi:1998di}) are also considered, to assess the performance of the analyses in scenarios where the stop and sbottom typically have many allowed decay channels with competing branching ratios. Three different sets of pMSSM models are considered, which take into account experimental constraints from LHC direct searches, satisfying the Higgs boson mass and dark-matter relic density constraints, or additional constraints arising from considerations of naturalness. The sensitivity to these models is discussed in Section~\ref{sec:pMSSM}.
published_SR.tex:\paragraph{Final states from  compressed stop decays (\stopCharm)}
published_SR.tex:\input{charm}
sbottom.tex:Under the assumption that no supersymmetric particle takes part in the sbottom decay apart from the lightest neutralino, the sbottom decays as $\bone \rightarrow b \neut$ with a branching ratio of 100\% (Figure~\ref{fig:bN1bN1}). The final state arising from sbottom pair production hence contains two \bjets\ and \etmiss. The \sbottom\ signal regions were explicitly optimised to be sensitive to this scenario. In case of a mass degeneracy between the sbottom and the neutralino, the general consideration that the monojet-like \stopCharm-M selection is almost insensitive to the details of the decay of the produced particles still holds:
sbottom.tex:the \stopCharm-M signal regions offer the best sensitivity for scenarios where $m_{\bone} \sim m_{\neut}$.  
sbottom.tex:	\caption{Observed (solid lines) and expected (dashed lines) 95\% CL limits on sbottom pair production where the sbottom is assumed to decay as $\bone \rightarrow b \neut$ with a branching ratio of 100\%. The purple lines refer to the limit of the \stopCharm\ analysis, while the blue lines refer to the \sbottom\ analysis.}
sbottom.tex:Figure~\ref{fig:sbottom_bneut} shows the limits of the \stopCharm\ and \sbottom\ analyses on the $m_{\bone} - m_{\neut}$ plane. The monojet-like (\stopCharm-M) SRs  exclude models up to a value of $m_{\bone} \sim m_{\neut} \sim 280\ \GeV$. Sbottom masses are excluded up to about 600 GeV for neutralino masses below about 250 GeV. 
sbottom.tex:If other supersymmetric particles enter into the decay chain, then multiple decay channels would be allowed. Similarly to the stop, the case in which other neutralinos or charginos have a mass below the sbottom is well motivated. The branching ratios of the sbottom to the different decay channels depend on the supersymmetric particle mass hierarchy, on the mixing of the left-right components of the sbottom, and on the composition of the charginos and neutralinos in terms of bino, wino, and higgsino states.
signal_generation.tex:Several SUSY models are considered throughout this paper. This section provides the details of how these signal models are generated. For all SUSY models discussed below, the detector response is simulated by passing the generated events  through a detector simulation~\cite{atlassimulation} based on \geant~\cite{geant4} or through a fast simulation using a parametric response to the showers in the electromagnetic and hadronic calorimeters~\cite{ATL-PHYS-PUB-2010-013} and \geant-based simulation elsewhere. All samples are produced with a varying number of simulated minimum-bias interactions overlaid on the hard-scattering event to account for multiple $pp$ interactions in the same or nearby bunch crossings (pileup). The simulation is reweighted to match the number of minimum bias interactions in data, which varies between approximately 10 and 30 interactions in each bunch crossing. Corrections are applied to the simulated samples to account for differences between data and simulation for the trigger and reconstruction efficiencies, momentum scale and resolution of the final-state objects, including the efficiency of identifying jets originating from the fragmentation of \bquarks, together with the probability for mis-tagging light-flavour and charm quarks.
signal_generation.tex:The three-body stop decay samples are generated with \herwigpp, which performs the matrix element calculation of the three-body decay. The four-body stop decay samples are generated with \madgraph.
spin_correlation.tex:If the mass of the $\tone$ is such that $m_{\tone} \sim m_{\neut} + \mtop$, the final-state kinematics are similar to that of Standard Model \ttbar\ production. One possible approach is to derive exclusion limits on the stop mass by performing SM precision measurements. This analysis has measured the azimuthal angle difference between the two leptons arising from the dileptonic \ttbar\ decay~\cite{Aad:2014mfk}. The events are required to contain, beside the two leptons, at least two additional jets, one of which is required to be \btagged. In events containing two leptons of the same flavour, the $Z$ production background is suppressed by applying a selection on the dilepton invariant mass. The distribution of the azimuthal angle between the two leptons is sensitive to the spin correlations of the $\ttbar$ system: it is hence used to extract limits on possible contaminations from direct scalar top production events. 
ss3l.tex:Final states containing many leptons or same-sign (SS) leptons can arise from the pair production of gluinos and squarks, when the produced particles decay to the LSP through multiple intermediate stages, or when several top quarks appear as part of the decay chain. The analysis was developed for the gluino-mediated stop production process $\gluino \gluino \rightarrow \tone \tone t t$ followed by $\tone \rightarrow t \neut$,  which can yield final states containing up to four leptons, including SS pairs. Similar final states arise from the sbottom decay $\bone \rightarrow t \chipm$, which are studied in this paper.
stop2.tex:Although the pair production of $\tone$ has a cross section larger than that of $\ttwo$, and although the decay patterns of the two particles can be similar, it can be convenient to search for the latter in regions where the sensitivity to the former is limited. This is the case, for example, in the region where $\DMstopN \sim \mtop$ of Figure~\ref{fig:tNsummary}, where the separation of $\tone$ pair production from SM top quark pair production is difficult. The \stopTwo\ and \ttH\ analyses are designed to detect $\ttwo$ pair production in this region of the $m_{\tone}-m_{\neut}$ plane, followed by the decays $\ttwo \rightarrow \tone Z$ and $\ttwo \rightarrow \tone h$. The Higgs boson $h$ is assumed to have a mass of 125 GeV and SM branching ratios.
stop2.tex:    \caption{Exclusion limits at 95\% CL in the scenario where $\ttwo$ pair production is assumed, followed by the decay  $\ttwo \rightarrow Z \tone$ (blue) or  $\ttwo \rightarrow \tone \higgs$ (red) and then by $\tone \rightarrow t \neut$ with a branching ratio  of 100\%, as a function of the $\ttwo$ and $\neut$ mass. The $\tone$ mass is determined by the relation $m_{\tone} - m_{\neut} = 180$ GeV. The dashed lines indicate the expected limit and the solid lines indicate the observed limit.}
stop2_app.tex:This analysis~\cite{Aad:2014mha} defines five different signal regions divided into two sets. The first set, named \stopTwo-SR2, requires two same-flavour leptons whose invariant mass is consistent with that of a $Z$ boson, $m_Z$, and at least one $b$-tagged jet. The three signal regions are characterised by the different selection thresholds applied to the \etmiss , to the transverse momentum of the dilepton system \ptll and to the jet multiplicity. The second set of signal regions, named \stopTwo-SR3, requires three leptons, two of which must form an opposite-sign same-flavour pair whose invariant mass is consistent with $m_Z$. Both signal regions require at least five jets, among which at least one has to be $b$-tagged. The two signal regions are characterised by the different selection thresholds applied to \ptll and to the leading lepton \pt. 
stopBC.tex:The final scenario considered is one where the stop mass is fixed at 300 GeV, and the exclusion limits are expressed in the $m_{\chipm}$--$m_{\neut}$ plane. In the case of the compressed scenario, corresponding to a small mass difference \dmCN, the fermions from the $W^{(\ast)}$ decay can escape detection and only the two \bjets and \etmiss would be identified in the final state. Thus, the \sbottom\ signal regions are expected to have a large sensitivity in this case, while for larger values of \dmCN, the lepton can be observed, yielding a final-state signature investigated by the \stopOneLep\ 
stopBC.tex:soft-lepton signal region. A combination of the \sbottom\ and \stopOneLep\ signal regions is performed by choosing, for each point of the plane, the SR giving the lowest \cls\ for expected exclusion. The
stop_4body_charm.tex:Two different scenarios, with $\DMstopN=10, 80$ \GeV, are considered. The first compressed scenario is characterised by low-\pt stop decay products, and the set of signal regions which have sensitivity is  the \stopCharm-M, independently of the decay of the stop. In the second scenario, the phase space available for the  \tone\ decay is larger, and  the full set of \stopCharm-M, \stopCharm-C,  \stopOneLep-bCa\_low, \stopOneLep-bCa\_med and \WWlike-SR selections have different sensitivity, depending on BR($\tone \rightarrow c \neut$). 
stop_4body_charm.tex:The limits quoted are taken from the best performing, based on expected exclusion \cls, signal regions from the \stopCharm-M, \stopCharm-C,  \stopOneLep-bCa\_low and \WWlike\ analyses at each mass point. The blue line and corresponding hashed band correspond to the mean value and uncertainty on the production cross section of the stop as a function of its mass. The pink lines, whose darkness indicate the value of BR($\stop \rightarrow c\neut$) according to the legend, indicate the observed limit on the production cross section.}
stop_4body_charm.tex:Figure~\ref{fig:cNeut_bffneut_combination} shows the result of these combinations. For $\DMstopN = 10$ GeV, the sensitivity is completely dominated by the \stopCharm-M 
stop_4body_charm.tex:the sensitivity is dominated by the \stopCharm-C signal regions at high values of BR($\stop \rightarrow c\neut$). For lower values of BR($\stop \rightarrow c\neut$), the ``soft-lepton'' and \WWlike\ signal regions both become competitive, the latter yielding a higher sensitivity at smaller values of the stop mass. The maximum excluded stop mass ranges from about 180 GeV for BR$(\stop \rightarrow c\neut)=50\%$ to about 270 GeV for BR$(\stop \rightarrow c\neut) = 100\%$.
stopsbottom_summary-metadata.tex:\AtlasCoverSupportingNote{Stop in  two leptons at intermediate mT2}{https://cds.cern.ch/record/1712507}
stopsbottom_summary-metadata.tex:\AtlasCoverAnalysisTeam{J.~Abdallah, S.~Amoroso, J.~Anders, J.-F.~Arguin, M.~Barisonzi, M.I.~Besana, M.~Bianco, J.~Boyd, S.~Brazzale, P.~Butti, R.~Caminal, A.~Cortes, D.~Costanzo~(*), D.~Cot\'e, J.~Da~Costa, C.~Deluca, P.~Dondero, M.~D'Onofrio, O.A.~Ducu, T.~Eifert, P.~Favareto, M. Fiascaris, L.~Gauthier, G.~Gaudio, V.~Giangiobbe, T.~Gilliam, M.P.~Giordani,  C.~Giuliani, T.~Golling, E.~Gorini, P.~Grenier, D.~Guest, R.~Hawkings, A.~Henrichs, G.~Herten, M.~Hohlfeld, W.~Hopkins, M.~Hurwitz, A.~Juste, M.~Kruse, J.~K\"uchler, T.~Lari, M.~LeBlanc, G.~Lerner, C.~Macdonald, S.~Majewski, M.~Martinez, A.~Martyniuk, P.~M\"attig, J.~Maurer, J.~McFayden, F.~Meloni, E. Le Menedeu, J.~Montejo, T.~M\"uller, B.~Nachman, Y.~Nakahama, M. Owen, M.~Pagacova, F.~Paige, P.~Pani, A.~Paramonov, S.~Pataraia, J.~Pilcher, G.~Polesello, J.~Poveda, R.~Povey, P.~Pralavorio, M.~Primavera, T.~Rave, G.~Redlinger, K.~Rosbach, F.~Rubbo, J.~Sh\"affer, C. Schwanenberg, J.-E.~Sundermann, K.~Suruliz, C.~Troncon, V.~Tsiskaridze, A.~Tudorache, F.~Ungaro, G.~Usai, A.~Ventura, I.~Vivarelli~(*), C.~Wanatayaroj, X.~Wang, T.~Yamanaka, C.~Zhou}
tbmet.tex:stop (or the sbottom), allow for the $\tone \rightarrow t \neut$, $\tone \rightarrow b\chipm$ and $\bone \rightarrow b \neut$, $\bone \rightarrow t \chipm$ decay channels to be open with competing branching ratios. Naturalness arguments require the higgsino mass parameter $\mu$ to be smaller than a few hundred GeV, while they impose virtually no constraint on the bino and wino mass parameters $M_1$ and $M_2$. If $\mu \ll M_1, M_2$, then the lightest chargino and neutralino masses are both of the order of $\mu$ and hence \dmCN\ is small. Therefore, pair production of stops can lead to $\tone\tone \rightarrow t\neut b\chipm \rightarrow t b \neut \neut ff'$, where $f$ and $f'$ represents low-\pt\ fermions emitted through $\chipm \rightarrow ff'  \neut$. Assuming both $f$ and $f'$ are too soft to be detected, the final state is characterised by the presence of a top quark, a bottom quark, and neutralinos escaping the detector. Similarly, $\bone$ pair production can lead to the same final state. Dedicated SRs are defined that target this topology, which is not well covered by the \stopZeroLep\  and \stopOneLep\ signal regions aimed at final states containing $t\bar{t}\etmiss$ and the \sbottom\ signal regions targeting $b\bar{b}\etmiss$ final states. 
tbmet.tex:has a veto requirement on the number of jets ($N_{\mathrm{xjets}}$) 
tbmet.tex:with \pt$>$50~GeV  in addition to the two leading \btagged jets. The final SR optimisation is performed
tbmet.tex:\item[-] $\metsig$: The ratio of the $\met$ to the square root of $H_{{\rm T}}$, which is the scalar sum of the $\pt$ of the two $b$-jets plus one light jet with $\pt > 25$ GeV and $|\eta| < 2.8$.
tbmet.tex:    \amtTwo^{2} ( \chi ) = \underset{ {\bf \not{q}}_{\rm T}^{(1)}   +   {\bf {\not q}}_{\rm T}^{(2)} =  {\bf \not{p}}_{\rm T}    }{min} \left [ max \left
tbmet.tex: \{  \mt^{2} ( {\bf p}_{\rm T}(v_{1}) , \xspace {\centernot{\bf{q}}_{\rm T}}^{(1)} ; \chi) , \mt^{2} ( {\bf p}_{\rm T}(v_{2}) , {\bf\centernot{q}}_{\rm
tbmet.tex:  \noindent where ${\bf p}_{\rm T}(v_{i})$ are reconstructed transverse momentum vectors, %or the top?.
tbmet.tex:  ${\bf\centernot{q}}_{\rm T}^{(i)}$ represent the missing transverse momenta from the two decays, with a total missing transverse momentum, ${\bf
tbmet.tex:\centernot{p}}_{\rm T} $, and $\chi$ is a free parameter representing the unknown neutralino mass, which is assumed to be zero in the calculation.
tbmet.tex:  The \amtTwo\ variable is calculated with different choices for $ {\bf p}_{\rm T}(v_{1})$ and ${\bf p}_{\rm T}(v_{2})$, depending on the value of \mlb$(n)$ ($n = 1,2$), the invariant mass of the $n^{\mathrm{th}}$ \btagged jet $b_n$ and the lepton: 
tbmet.tex:$N_{\mathrm{xjets}}$ & -- & -- & -- & $<$2  \\
tbmet.tex:points to SRs with no requirement on the $N_{\mathrm{xjets}}$ variable (\TBM-SRIn). In the case of the simplified models, additional 
tbmet.tex:jets come only from initial- or final-state radiation, and as a consequence a strict selection on $N_{\mathrm{xjets}}$ is applied as in the selection \TBM-SREx1.
tbmet.tex:production. The MC cross section is used to normalise the single-top background and all the other minor SM backgrounds, such as 
tbmet.tex:The normalisation factors of the \ttbar\ and \Wjets\ backgrounds are determined by a combined profile-likelihood fit. 
tbmet.tex:Specific control regions, whose event yield is expected to be dominated by each of these production processes, are defined and included in the fit to constrain the normalisation parameters. 
tbmet.tex:The \Wjets\ control regions (CRW) are defined by requiring $\mt<$120~GeV. For the control regions corresponding to the \TBM-SRIn, events with one \btagged\ jet are included in the CRW. Top quark pair production dominates the CRWs, with a \Wjets\ purity of 30\% or better. The normalisation factors $\mu_W$ and $\mu_{\ttbar}$ are presented
tbmet.tex:Norm. Factor & SRinA & SRinB & SRinC & SRexA \\
tbmet.tex:$\sigma_{\mathrm{vis}} = \sigma \times \epsilon \times \mathcal{A}$, where $\sigma$ is the cross section for non-SM 
tbmet.tex:together with the 95\% CL upper limits on the observed and expected number of signal events ($S_{\rm obs}^{95}$ 
tbmet.tex:and $S_{\rm exp}^{95}$ respectively), and on the visible cross section ($\langle\epsilon{\rm \sigma}\rangle_{\rm obs}^{95}$).
tbmet.tex:{\bf Signal channel}                        & Obs & Exp &  $S_{\rm obs}^{95}$  & $S_{\rm exp}^{95}$ &  $\langle\epsilon{\rm \sigma}\rangle_{\rm obs}^{95}$[fb]  \\
tbmet.tex:values of \dmCN=5, 20 GeV. Furthermore, by using a weighted combination of these simplified models with models corresponding
ttH.tex:The modelling of the production of \ttbar\ pairs in association with heavy flavour ($\ttbar$+HF) is of key relevance in this analysis. A detailed categorisation of $\ttbar$+HF is made for the purpose of comparisons with different generators and of the propagation of systematic uncertainties on the different heavy-flavour components. The categorisation is also used to reweight the different flavour components of the $\ttbar$+jets background to obtain a better modelling. These categorisation and reweighting procedures are discussed in detail in Ref.~\cite{Aad:2015gra}. In particular, the $\ttbar+\bbbar$ component, which is simulated with \powheg, is reweighted to a full NLO calculation \cite{Cascioli:2013era} performed in \sherpa 1.4.1+\verb+OpenLoops+\cite{Gleisberg:2008ta,Cascioli:2011va}. The reweighting is done at generator level using a number of kinematic variables such as the top quark \pt, \ttbar\ system \pt, $\Delta R$ and \pt of the dijet system not coming from the top-quark decay.  A different reweighting is applied to the $\ttbar + \ccbar$ and $\ttbar$+ light-jets components, which is based on the ratio of the differential cross sections at $\sqrt{s} = 7$ TeV obtained in data and simulation as a function of the top quark \pt and \ttbar\ system \pt~\cite{Aad:2014zka}. 
ttH.tex:The final discriminating variable used is \htnolep, defined as the scalar sum of \etmiss\ and the transverse momenta of all selected jets. The signal is searched for by performing a binned likelihood fit to the \htnolep\ distribution simultaneously in the six channels defined (low/high-\mt\ for three bins in \btagged\ jet multiplicity). The binning used for the \htnolep\ distributions is that used in Figure~\ref{fig:ttH_htnolep}, where the background estimate both before and after the fit is compared to the data  in the high-\mt\ region. The dominant post-fit uncertainties are  those on the absolute normalisation of the $\ttbar+\bbbar$ and $\ttbar+\ccbar$ processes. 
xsec.tex:N_1 = L \sigma_{\ttbar} \epsilon_{e\mu} 2\epsilon_b (1 - C_b \epsilon_b) + N_1^{\mathrm{bkg}} \label{eq:N1} \\
xsec.tex:N_2 = L \sigma_{\ttbar} \epsilon_{e\mu} C_b \epsilon_b^2 + N_2^{\mathrm{bkg}} \label{eq:N2}
xsec.tex:\noindent where $N_1$ and $N_2$ are the number of events with two different flavour leptons having exactly one or two \btagged\ jets, respectively,  $L$ is the integrated luminosity,  $\epsilon_{e\mu}$ the efficiency for a $\ttbar$ event to pass the lepton selection, $\epsilon_b$ is the probability of having a \bjet within acceptance and for it to be  tagged, $C_b$ is a correlation coefficient which is close to unity, and $N_1^{\mathrm{bkg}}$ and $ N_2^{\mathrm{bkg}}$ are the number of events with one or two \btagged\ jets  from SM events different from $\ttbar$ production. The values of $\sigma_{\ttbar}$ and $\epsilon_b$ are extracted from the data by solving the two simultaneous equations~(\ref{eq:N1}) and (\ref{eq:N2}), avoiding the need to estimate $\epsilon_b$ from simulation.
xsec.tex:The sensitivity of the $\ttbar$ cross-section measurement to $\tone$ pair production assuming  a branching ratio of 100\% into $\tone \rightarrow b \chipm$, followed by $\chipm \rightarrow W^{(*)} \neut$ with $m_{\chipm} = 2 m_{\neut}$ was also investigated. The presence of the intermediate chargino state tends to lower the \pt\ of the leptons and of the \bjets\ significantly, hence decreasing both  $\epsilon_{e\mu}$ and $\epsilon_b$. No exclusion limit can be derived for this scenario.  

